On P vs. NP, Geometric Complexity Theory, Explicit Proofs and the Complexity Barrier

Geometric complexity theory (GCT) is an approach to the P vs. NP and related problems. This article gives its complexity theoretic overview without assuming any background in algebraic geometry or representation theory.

==> GCT6_1.tex <==
\section{C: On crossing of the feasibility barrier in  characteristic zero}
\label{sgct6}
We now proceed to describe the main result of GCT for the general
complexity-theoretic
permanent vs. determinant problem in characteristic zero in the context
of  Goal~\ref{gobs} and the crossing of the  feasibility barrier. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of copies of 
the Weyl module $V_{k\lambda}(G)$ that live on $X_{\#P}(n,m)$. 
Let $G_{\lambda,m}(k)$ denote the  dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$. Here
by an invariant we mean a fix point of $G_{\det}$. i.e., a point that
does not move under its action.

Given a polytope $Q$, we let $f_Q(k)$ denote the number of 
integer points in the dilated polytope $k Q$. 
More generally, given a parametrized  polytope $P(k)$
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $s \times t$ matrix, $x$ a variable $t$-vector, and 
$b$ and $c$ some constant $s$-vectors, let 
$f_P(k)$ denote the number of integer points in $P(k)$. 



\begin{hypo} {\bf (PH1) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   an explicit  parametrized  polytope $P(k)=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is.
By explicit we mean 
it is given by 
a separation oracle \cite{lovasz} that, given any point $x$,
decides if $x \in P(k)$ and gives a separating hyperplane if it does not
in $\poly(n,\bitlength{m},\bitlength{x},\bitlength{k})$
time, where $\bitlength\langle \ \rangle$ denotes the bitlength of
description.

\noindent (b) For every $m$, there exist an  explicit 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is as long as
the length of $\lambda$ is $\poly(n)$ (as it will be in our applications).
Explicitness is defined similarly.
\end{hypo} 

See [GCT6,GCT7,GCT8] and \cite{GCTexplicit} for mathematical results, evidence
and justification for this hypothesis.


\begin{theorem} (GCT6) \label{tgct6}
The feasibility barrier for verification for the 
$\#P$ vs. $NC$ problem in characteriztic zero is crossed 
assuming  PH1. 

Specifically, there exists a explicit family $\{O_n\}$ of  obstructions 
for this problem 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

The feasibility barrier for discovery is also crossed assumming a
stronger positivity hypothesis PH4 that we do not specify here.

Analogous results holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

For mathematical evidence and justification for why OH should hold
see [GCT2,6,7,8]. 

The proof of Theorem~\ref{tgct6}, or rather the various results 
needed to justify its statement, is based on
the classical work of Hilbert in invariant theory \cite{mumford},
the fundamental work
on the resolutions of singularities in characteristic zero
\cite{hironaka} and the 
cohomological works \cite{boutot,flenner} 
based on this resolution; cf. \cite{GCTexplicit,GCT6} for other references.

Here OH is a {\em complexity theoretic} hypothesis in the sense
that $m$ has to be small in comparison with $n$ for it to hold,
as in the original IOH in this problem (which is similar to the
one in $P$ vs. $NP$ problem that we discussed before). 
In contrast, PH1 is a {\em mathematical} hypothesis in the sense
that there is no such restriction, and though there is a complexity 
theoretic component to it, it does not seem ``hard'' like the original 
$P \not = NP$ conjecture, because the dimensions of the various polytopes 
are already guaranteed to be $\poly(n)$, regardless of what $m$ is,
if they exist, and the complexity theoretic component is  basically 
linear programming on these small dimensional polytopes, which is 
generally regarded as  theoretically ``easy''.

Once the mathematical hypotheses PH1 and PH4 are proved, the feasibility
barrier is crossed and OH  becomes theoretically
feasible. Though, as we have already pointed out, actually proving OH
can be a mathematical challenge. 
Thus, in effect, this theorem has exchanged hard 
complexity theory (IOH) with hard mathematics (PH1+PH4+OH). What is
gained in this exchange is that the $P\not = NP$ conjecture 
should not stand in the way of this hard mathematics as it seemed to 
in the way of the original theoretically infeasible IOH.
The two concrete lower bounds of GCT that we discussed before 
illustrate that this exchange works in nontrivial instances.





As for as proving OH is concerned, there is nothing that we can
say at this point since it depends on the explicit forms of the polytopes 
in PH1/PH4.  So the next question is how to prove PH1. 
GCT6,7,and 8 suggest  an approach for this  via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
 lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for implementation of the
flip, i.e., for explicit construction of obstructions, based on
Theorem~\ref{tgct6}
seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to need   more. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.



==> GCT6_2.tex <==
\section{C: On crossing of the feasibility barrier in  characteristic zero}
\label{sgct6}
We now proceed to describe the main result of GCT for the general
complexity-theoretic
permanent vs. determinant problem in characteristic zero in the context
of  Goal~\ref{gobs} and the crossing of the  feasibility barrier. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of copies of 
the Weyl module $V_{k\lambda}(G)$ that live on $X_{\#P}(n,m)$. 
Let $G_{\lambda,m}(k)$ denote the  dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$. Here
by an invariant we mean a fix point of $G_{\det}$. i.e., a point that
does not move under its action.

Given a polytope $Q$, we let $f_Q(k)$ denote the number of 
integer points in the dilated polytope $k Q$. 
More generally, given a parametrized  polytope $P(k)$
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $s \times t$ matrix, $x$ a variable $t$-vector, and 
$b$ and $c$ some constant $s$-vectors, let 
$f_P(k)$ denote the number of integer points in $P(k)$. 



\begin{hypo} {\bf (PH1) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   an explicit  parametrized  polytope $P(k)=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is.
By explicit we mean 
it is given by 
a separation oracle \cite{lovasz} that, given any point $x$,
decides if $x \in P(k)$ and gives a separating hyperplane if it does not
in $\poly(n,\bitlength{m},\bitlength{x},\bitlength{k})$
time, where $\bitlength\langle \ \rangle$ denotes the bitlength of
description.

\noindent (b) For every $m$, there exist an  explicit 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is as long as
the length of $\lambda$ is $\poly(n)$ (as it will be in our applications).
Explicitness is defined similarly.
\end{hypo} 

See [GCT6,GCT7,GCT8] and \cite{GCTexplicit} for mathematical results, evidence
and justification for this hypothesis.


\begin{theorem} (GCT6) \label{tgct6}
The feasibility barrier for verification for the 
$\#P$ vs. $NC$ problem in characteriztic zero is crossed 
assuming  PH1. 

Specifically, there exists a explicit family $\{O_n\}$ of  obstructions 
for this problem 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

The feasibility barrier for discovery is also crossed assumming a
stronger positivity hypothesis PH4 that we do not specify here.

Analogous results holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

For mathematical evidence and justification for why OH should hold
see [GCT2,6,7,8]. 

The proof of Theorem~\ref{tgct6}, or rather the various results 
needed to justify its statement, is based on
the classical work of Hilbert in invariant theory \cite{mumford},
the fundamental work
on the resolutions of singularities in characteristic zero
\cite{hironaka} and the 
cohomological works \cite{boutot,flenner} 
based on this resolution; cf. \cite{GCTexplicit,GCT6} for other references.

Here OH is a {\em complexity theoretic} hypothesis in the sense
that $m$ has to be small in comparison with $n$ for it to hold,
as in the original IOH in this problem (which is similar to the
one in $P$ vs. $NP$ problem that we discussed before). 
In contrast, PH1 is a {\em mathematical} hypothesis in the sense
that there is no such restriction, and though there is a complexity 
theoretic component to it, it does not seem ``hard'' like the original 
$P \not = NP$ conjecture, because the dimensions of the various polytopes 
are already guaranteed to be $\poly(n)$, regardless of what $m$ is,
if they exist, and the complexity theoretic component is  basically 
linear programming on these small dimensional polytopes, which is 
generally regarded as  theoretically ``easy''.

Once the mathematical hypotheses PH1 and PH4 are proved, the feasibility
barrier is crossed and OH  becomes theoretically
feasible. Though, as we have already pointed out, actually proving OH
can be a mathematical challenge. 
Thus, in effect, this theorem has exchanged hard 
complexity theory (IOH) with hard mathematics (PH1+PH4+OH). What is
gained in this exchange is that the $P\not = NP$ conjecture 
should not stand in the way of this hard mathematics as it seemed to 
in the way of the original theoretically infeasible IOH.
The two concrete lower bounds of GCT that we discussed before 
illustrate that this exchange works in nontrivial instances.


As for as proving OH is concerned, there is nothing that we can
say at this point since it depends on the explicit forms of the polytopes 
in PH1/PH4. PH4 is a stronger form of PH1.
So the critical question here is how to prove PH1 and why  should 
hold. This will be discussed in Section~\ref{showph}. 


\ignore{
GCT6,7,and 8 suggest  an approach for this  via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
 lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for implementation of the
flip, i.e., for explicit construction of obstructions, based on
Theorem~\ref{tgct6}
seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to need   more. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.
}


==> GCT6_3.tex <==
\section{C: Formalization of  the complexity barrier in  characteristic zero}
\label{sgct6}
We now proceed to describe the main result of GCT for the general
permanent vs. determinant problem in characteristic zero in the context
of  Goal~\ref{gobs}--this result  yields formalization of the
complexity barrier for this problem.



Towards that end, we  define some
representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of copies of 
the Weyl module $V_{k\lambda}(G)$ that live on $X_{\#P}(n,m)$. 
Here $k \lambda$ denotes the partition obtained by multiplying each 
number in the integral sequence (partition) $\lambda$ by $k$.
Let $G_{\lambda,m}(k)$ denote the  dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$. Here
by an invariant we mean a fix point of $G_{\det}$. i.e., a point that
does not move under its action.

Given a polytope $Q$, we let $f_Q(k)$ denote the number of 
integer points in the dilated polytope $k Q$. 
More generally, given a parametrized  polytope $P(k)$
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
P(k): \qquad A x \le k b + c,
\end{equation}
where $A$ is an $s \times t$ matrix, $x$ a variable $t$-vector, and 
$b$ and $c$ some constant $s$-vectors, let 
$f_P(k)$ denote the number of integer points in $P(k)$. 



\begin{hypo} {\bf (PH1) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   an explicit  parametrized  polytope $P(k)=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is.
By explicit we mean 
it is given by 
a separation oracle \cite{lovasz} that, given any point $x$,
decides if $x \in P(k)$ and gives a separating hyperplane if it does not
in $\poly(n,\bitlength{m},\bitlength{x},\bitlength{k})$
time, where $\langle \ \rangle$ denotes the bitlength of
description.

\noindent (b) For every $m$, there exist an  explicit 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
If such a polytope exists it is guaranteed by a general result in GCT6 
that its dimension is $\poly(n)$ regardless of what $m$ is as long as
the length of $\lambda$ is $\poly(n)$ (as it will be in our applications).
Explicitness is defined similarly.
\end{hypo} 

Why PH1 should hold will be discussed in
Section~\ref{showph} below.
PH1, in particular, implies that $F_{\lambda,n,m}(k)$ and
$G_{\lambda,m}(k)$ have $\#P$ formulae. Positivity refers to the positive 
form of a $\#P$-formula, i.e., the absence of any negative sign
as in the usual formula for the permanent. 


\begin{theorem} (GCT6) \label{tgct6}
There exists an explicit family $\{O_n\}$ of  obstructions 
for the permanent vs. determinant problem 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH1, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

In particular, this says that the complexity barrier for verification for the 
$\#P$ vs. $NC$ (i.e. permanent vs. determinant) 
problem in characteristic zero is crossed 
assuming  PH1. Or in other words, the complexity barrier for verification
is formalized with PH1 being the mathematical hypothesis 
involved in this formalization (cf. Section~\ref{sflip}).

The complexity barrier for discovery is also crossed assuming a
stronger positivity hypothesis PH4 that we do not specify here \footnote{The
hypothesis is called PH4 instead of PH2 because PH2 and PH3 are some other
positivity hypotheses related to PH1 that we do not discuss here}.
Or in other words, the complexity barrier for discovery and hence
the whole complexity barrier is also formalized, with PH1 and PH4 being
the mathematical hypotheses involved in this formalization. 


Analogous results holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

For mathematical evidence and justification for why OH should hold
see [GCT2,6,7,8]. This result provides a formalization of the
complexity barrier in characteristic zero.
We  discuss its  reasonableness in
Section~\ref{showph} below. This addresses criterion C. 

The proof of Theorem~\ref{tgct6}, or rather the various results 
needed to justify its statement, is based on
the classical work of Hilbert in invariant theory \cite{mumford},
the fundamental work in algebraic geometry 
on the resolutions of singularities in characteristic zero
\cite{hironaka} and the 
cohomological works \cite{boutot,flenner} 
based on this resolution; cf. \cite{GCTriemann} and GCT6 for other references.

Here OH is a {\em complexity theoretic} hypothesis in the sense
that $m$ has to be small in comparison with $n$ for it to hold,
as in the original IOH for this problem (which is similar to the
IOH for  $P$ vs. $NP$ problem that we discussed before). 
In contrast, PH1 is a {\em mathematical} hypothesis in the sense
that there is no such restriction, and though there is a complexity 
theoretic component to it, it is not expected to be ``hard'' like the original 
$P \not = NP$ conjecture, because the dimensions of the various polytopes 
are already guaranteed to be $\poly(n)$, regardless of what $m$ is,
if they exist, and the complexity theoretic component is  basically 
linear programming on these small dimensional polytopes, which is 
generally regarded as  theoretically ``easy''.

Once  PH1 and PH4 are proved, the complexity
barrier is crossed and OH  becomes theoretically
feasible. Though, as we have already pointed out, actually proving OH
can be a mathematical challenge. 
Thus, in effect, this theorem has exchanged hard 
complexity theory (IOH) with hard mathematics (PH1+PH4+OH). What is
gained in this exchange is that the $P\not = NP$ conjecture 
should not stand in the way of this hard mathematics as it seemed to 
in the way of the original theoretically infeasible IOH.
The two concrete lower bounds of GCT that we discussed before 
illustrate that this exchange works in nontrivial instances.


As for as proving OH is concerned, there is nothing that we can
say at this point since it depends on the explicit forms of the polytopes 
in PH1/PH4. So we turn to PH1/4 next.


\section{Why should the positivity hypotheses 
hold and how to prove them?} \label{showph}
Reasonability of the formalization of the complexity barrier
in characteristic zero in Theorem~\ref{tgct6}
critically  hinges on  PH1 and PH4.
To show reasonability,
we have to  justify why these positivity hypotheses  should hold and 
why the $P\not = NP$ conjecture should not stand in the way of their proofs.
Let us just consider  PH1 (b), which is a basic prototype 
of the  general PH1 and PH4; for a discussion of the general PH1 and PH4,
see {GCT6,7,8].
So we have to now justify why PH1 (b)  should hold,  why the $P\not = NP$ 
conjecture should not stand in the way of its proof, and also briefly 
indicate GCT's plan for proving it.



The coefficients $G_{\lambda,m}(k)$ that occur in PH1 (b) 
are known as Kroncker coefficients in representation theory and hence we shall
refer to PH1 (b) as Kroncker PH1. It is a complexity 
theoretic version of the fundamental Kronecker problem in representation
theory that   has been intensively studied in the last century and 
is known to be formidable. And now 
it lies at the heart of this approach towards $P$ vs. $NP$. 

A special case of  Kronecker PH1 has been solved in representation theory.
for a very special class of Kronecker coefficients 
called Littlewood-Richardson (LR) coefficients. These 
are basically the multiplicities in the 
analogous  PH1 (b) that occurs in the proof of the
mathematical form of the $\#P\not = NC$ conjecture (Theorem~\ref{tmathform})
(formally LR coefficient is  the multiplicity of a given Weyl module
in the tensor product of other two given Weyl modules, 
but let us worry about its formal definition  here). 
We shall refer to this special case of the Kronecker PH1 
that occurs in the proof of the mathematical form as LR PH1.




Figure~\ref{fig:lift} gives  a pictorial
depiction of the plan to prove Kronecker PH1  
suggested  in [GCT4,6,7,8].
It strives  to extend the  proof of LR PH1 based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig},
where a standard quantum group is  a mathematical object that plays
the same role in quantum mechanics that the classical group 
$G=GL_n(\C)$ plays in classical physics.  
There it comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that every representation of 
the standard quantum group
has a canonical basis \cite{kashiwara,lusztig} 
whose structural coefficients that determine the action of the generators 
of the standard quantum group 
on this basis are polynomials in $q$ whose coefficients are 
all nonnegative  \cite{lusztig} (here $q$ stands for quantization 
parameter in physics). 
The only known proof of this positivity 
result is  based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2}  and the related works \cite{beilinson}.
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH1 can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH1, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic  proof. 
But the plan to extend the
proof of LR PH1 to Kronecker PH1 and (its other needed generalizations)
in GCT4,6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Kronecker PH1, more  precisely 
some  natural generalization of LR PH0 in this context which
we shall call Kronecker PH0.
Thus what is needed now 
is a systematic lifting  of the bottom row in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 


Initial  steps in this direction have been taken in GCT4,7,8. 
First, GCT4 and 7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
and plays the
same role in the context of Kronecker PH1
(and the   more general Plethysm PH1 which lies at the heart of 
the general PH1)
that the standard quantum group plays
in the context of  LR PH1. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Kronecker PH0,
which is some natural generalization of LR PH0, and is 
supported by experimental numerical evidence generated with the help
of a computer.


This numerical evidence is the main evidence for Kronecker PH0
and hence Kronecker  PH1 (i.e. PH1 (b)). 
It is reasonable because positivity (Kronecker PH0) is an extremely rigid 
property. Specifically, the structure coefficients involved in Kronecker 
PH0 are extremely complex mathematical quantities whose computation 
involves summing exponentially many terms of alternating signs.
If there were no reason for them to have any specific sign, 
they would be positive or negative with roughly the same probability,
naively speaking, and the probability that several hundred of these
mathematical quantities (which were computed) 
would all turn out to be of the same sign would be  absurdly  small 
(something like $2^{-500}$, again  naively speaking). 
Hence, this seems to be  a reasonble evidence  that PH1 (b)  should hold. 


This numerical evidence for positivity (PH0) is in the spirit 
of the existing numerical evidence for  the Riemann Hypothesis,
to which PH0 is
intimately related as shown in Figure~\ref{fig:lift}. Existing 
numerical evidence for the  Riemann Hypothesis has been   obtained 
by  computing the first few zeros of the Riemann zeta function 
and then checking  if they really lie on the critical line. 
If they do (as they do so far) that gives
us a reasonable assurance  that the Riemann Hypothesis is true.
Especially so because the Riemann Hypothesis 
is an extremely rigid mathematical statement. By extremely rigid, we mean
if it were false we expect it to collapse completely and the zeros 
to get scattered  all over. Similarly PH0 is also expected to be 
an extremely rigid property since
it is intimately related to the Riemann Hypothesis. If were wrong, we again
expect it to collapse completely and the signs of the structural
coefficients  to be $+$ or $-$ with roughly equal probability.
That PH0 holds in the substantial numerical evidence obtained so far
gives us reasonable assuarance that it should hold just 
like the Riemann Hypothesis.




We also have to justify why the $P \not = NP$ conjecture should not
stand in the way of proving Kronecker PH0. 
This is because it is a natural mathematical  generalization of LR PH0, and
we know now that the $P\not = NP$ conjecture did not stand in the way of the
proof of LR PH0 in \cite{lusztig} and also in the way of the
proof of  the Riemanna Hypothesis over finite fields in \cite{weil2} 
on which the proof in \cite{lusztig} depends. The main point 
here is that however hard the Riemann Hypothesis and the related positivity
hypotheses in mathematics  may be, they are  not
not complexity theoretic hypotheses. That is, hard complexity theoretic 
statements have not been encoded in their statements. 
Of course, we cannnot guarantee that the $P\not = NP$ conjecture 
would not stand in the way of the proof of the usual Riemann Hypothesis.
But the fact that it did not stand in the way of the proof of 
its analogue over finite fields in \cite{weil2} gives us a reasonable 
assurance that it should not stand in the way of the proof of the usual
Riemann Hypothesis either. And similarly,  also in the 
the way of the proofs of the related positivity 
hypotheses in mathematics,  however hard they may be to prove.



Finally,  let us briefly discuss the plan for proving Kronecker PH0 proposed 
in [GCt7,8,11].
The plan is besically  to complete the 
commutative diagram in Figure~\ref{fig:lift}. What is needed 
for this completion  is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Kronecker PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 
All the numerical evidence for the positivity suggests that 
what is needed in the top-right corner--some nonstandard extension
of the Riemann Hypothesis over finite fields--exists, but at present
we have no idea what it is. 
Whatever it is, the proof of PH0 promises to be a formidable affair.

To summarize, the discussion above suggests that there is now a good reason
to believe why the positivity hypotheses should hold, and why 
the $P\not = NP$ conjecture should not stand in the way of their
proofs--that is, why the formalization of the complexity barrier in
characteristic zero (Theorem~\ref{tgct6}) should be reasonable, and 
why this approach should thus penetrate the formidable circle around the
$P\not = NP$ conjecture in characteristic zero. But there is no reason
to believe that we are anywhere close to the proofs of these positivity
hypotheses. In fact, there is every reason to believe that we may be
very, very far away.






\ignore{
Thus the ultimate goal of GCT would be  to deduce the ultimate 
negative hypothesis of mathematics, $P \not = NP$ conjecture (in characteristic
 zero), 
from the ultimate positive hypotheses--namely, as yet unknown,
nonstandard Riemann
hypotheses (over finite fields); cf. Figure~\ref{fig:finalgoal}.
The reader may have noticed something striking here. Namely,
to prove the $P \not = NP$ conjecture in characteristic zero what is
needed is not nonstandard extension of the work surrounding the
Riemann hypothesis in characteristic zero (that is the standard 
Riemann hypothesis) but rather the one over finite fields. 
This flip from characteristic zero to finite fields happens in 
the theory of quantum groups for some profound reasons \cite{lusztig} that 
we shall not go into here. Similarly, the opposite flip is also plausible: 
namely, for proving the analogue of PH1 in positive characteristic
[GCT11]  nonstandard extension of the work surrounding  the usual Riemann 
hypothesis over $\Z$, or rather its generalizations that occur in
arithmetic algebraic geometry and the theory of automorphic forms
may be needed. 

Thus  this plan for implementing  the flip seems  to be a massive affair.







\begin{figure} 
\begin{center}
\psfragscanon
\epsfig{file=finalgoal.eps, scale=.6}
\end{center}
      \caption{The ultimate goal of GCT}
      \label{fig:finalgoal}
\end{figure}

}



\ignore{ GCT6,4,7,and 8 suggest  an approach for this  via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group,
and  which are supported by considerable computer generated numerical
evidence that constitutes  the main experimental evidence  for PH1.
The only known proofs of these positivity results in the theory
of the standard quantum group  are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme [GCT6,4,7,8] for implementation of the
flip  based on Theorem~\ref{tgct6}
seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem in
mathematics.
%which encompasses several areas of mathematics, such as algebraic geometry,
%representation theory, quantum groups and so forth.
This mathematical story is far beyond the scope of this article;
cf. the mathematical overview \cite{GCTriemann} and 
[GCT4,6,7,8] for more on this.}



\ignore{
This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexity theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to need   more. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.
}



==> complexity1.tex <==
\section{Complexity barrier} \label{scomplexity}
Before we turn to the complexity barrier, let us see why 
the  earlier known barriers towards the $P$ vs. $NP$ problem 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
and algebraic-degree [GCTlocal] barriers cannot be expected to 
capture the root difficulty of the $P$ vs. $NP$ problem. 

Let us begin with the algebraic degree barrier in [GCTlocal].
It basically says that the low degree techniques of the kind used in that
paper  would not help in the
fundamental separation problems. All these techniques are in one way or
the other related to the fundamental Bezout's theorem in algebraic geometry
and the notion of a degree of a polynomial
(we also include the low degree techniques used in other areas of 
complexity theory in this category). Though this is a nontrivial area of
mathematics, it is still very small compared to the whole of mathematics.
Hence, we can say that this  barrier is {\em local} 
in the sense that it applies to a very 
restricted class of techniques in mathematics. Furthermore, we can say 
that this barrier is primarily {\em mathematical} in the sense that low degree 
is a purely a mathematical notion, there is no complexity theory in it,
and though it  is very useful in complexity theory, this barrier is really a 
statement about the restricted nature  and weakness of these mathematical 
techniques rather than about the complexity theoretic difficulty 
of  the $P$ vs. $NP$ problem.
In a similar way, we may say that the relativization and natural proof 
barriers are also local and mathematical.  Mathematical  because the natural 
proof barrier is generally regarded as applying to proof techniques that 
work for most functions and most is a mathematical notion, 
so also the notion of relativization.

Unfortunately after  GCT1 and 2, wherein these local mathematical
barriers were bypassed (cf. Section~\ref{smathform}),  
it became clear that  the root 
difficulty of the $P$ vs. $NP$ problem still remained after bypassing
them  and the  main battle 
on the $P$ vs. $NP$ problem  really begins only after bypassing them.

In retrospect, this should not be surprising. 
We cannot expect local mathematical 
barriers to capture the root difficulty of the $P$ vs. $NP$ problem,
because this problem is a {\em universal complexity-theoretic} 
statement about all of mathematics.
Namely, if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal complexity theoretic 
nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal} and {\em complexity theoretic},
where by a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
A local barrier only  rules out a 
restricted  area of mathematics. 
Regardless of how many restricted   areas of mathematics we rule 
out in this way, that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do
given that the $P$ vs. $NP$ problem is a statement about all of mathematics. 
At some point we have to turn our attention from what is not to be done
to  what is to be done
and identify the root universal and complexity theoretic 
difficulty of this problem; i.e., 
a universal complexity theoretic barrier.

The complexity  barrier seems to be this universal complexity theoretic 
barrier.
Due its universality, it seems quite formidable, as expected.
To describe it,   let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any proof strategy for  the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question}[The folklore question of complexity theory]
\label{qfeasible} 
Why should the
proof strategy  be  even  {\em theoretically  feasible}, i.e., 
lead to a proof even theoretically? 
In other words, in what sense is it fundamentally 
different from the  trivial, infeasible strategy  above
and not just a restatement of the original problem? 

In general, what is a {\em theoretically feasible proof strategy} for the 
$P$ vs. $NP$ problem? 
Does such a strategy even exist?
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem stated above.
These local  barriers   roughly say that the proof techniques akin to
the ones used for proving three types of lower bounds, 
namely the classical hierachy theorems, lower bounds for 
constant depth circuits \cite{sipser} and the $P\not = NC$ result 
without bit operations [GCTlocal], would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
along with its variants and properties, 
rendering them theoretically infeasible, so to say.
Admittedly,  since these local barriers apply to 
proof techniques that constitute  only    very specific 
subareas of mathematics, 
we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions, why can it not
keep on  happening ad infinitum? 
This does not seem inconceivable 
since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the fundamental folklore question
that has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining:
why should a given proof technique 
be even {\em theoretically feasible}  as per some 
reasonable notion of theoretical feasibility. 


By the {\em  complexity barrier} we mean the task of answering this
Question~\ref{qfeasible} {\em formally}. The key phrase here is formally.
Because Question~\ref{qfeasible} itself is an informal folklore question
with no theorem or precise mathematics behind it. To answer it formally
means:

\begin{enumerate} 
\item Fix a proof strategy and  formalize the question by defining 
formally {\em theoretically feasibility} 
of the given  proof strategy,
justify why this  is a reasonable formalization, and then
\item Answer the formalized question, i.e., prove that
the proof strategy under consideration is theoretically feasible
as per this formal definition.
\end{enumerate} 
In other words,
formalization of the question  is itself a part of the challenge, a part 
of the root difficulty.

This is not a new phenomenon.
Indeed, many fundamental questions in science are informal folklore 
questions and a part or sometimes the whole of the
challenge lies in just formalizing them.
For example:

\begin{question}[The folklore question of computability theory] 
\label{qcomputable}
What is computable (decidable)? 
\end{question} 

This is informal. 
But the main challenge in computability theory as we know now--we shall
call this the {\em computability barrier}--was to  
formalize this question by giving a precise mathematical meaning to
the phrase {\em computable} (Church-Turing Hypothesis \cite{church,turing})
and then justify 
that  it is a reasonable formalization. 
Of course, formalization
of the phrase computable 
that we have today is  one reasonable  formalization. We will say that 
the present computability theory  is 
one way of crossing the computability barrier.
We cannot say that it is the only one. There may be other ways of 
reasonably formalizing this question. Every such way will correspond to
a different computability theory.
But if there are other reasonable computability theories,  
we do not know them today.


The crossing of this computability barrier is the key ingradient 
in proving  G\"odel's Incompleteness Theorem--namely, that 
the language of true statements in number theory is undecidable.
Actually, the Incompleteness Theorem
predated computability theory and 
was originally  stated in terms of definability rather than computability.
But let us ignore the history and imagine asking
(as was essentially done by Hilbert), if  number theory is 
decidable, without a formal definition of  decidable.
Then the fundamental difficulty in answering this question is 
just formalizing the informal Question~\ref{qcomputable}.
That is, crossing of the computability barrier above. Once this is done 
and  the phrase 
computable or decidable is given a formal meaning, proving Incompleteness 
Theorem is essentially routine--it only needs   encoding of computations.
The Incompleteness Theorem 
is also a universal statement about mathematics like the $P$ vs. $NP$ problem.
Hence, it is especially relavant to study 
the  nature of the fundamental conceptual difficulty in its proof. 
As we see in retrospect,  this was basically 
formalizing the  fundamental  folklore Question~\ref{qcomputable}.
If so, it should not be surprising if at least a part of the 
fundamental conceptual difficulty in  the proof of the other 
universal statement about mathematics--the $P$ vs. $NP$ problem--should 
also be just formalizing some other  fundamental folklore  question.


Question~\ref{qfeasible} seems to be that  question.
As per the folklore, it 
is supposed to be the  root 
difficulty of the $P$ vs. $NP$ problem, and a part of this
difficulty is just formally stating what the question is saying, i.e,
formalizing this question by giving a precise 
mathematical meaning to  {\em theoretically feasibility} of the given 
proof strategy. 
If by complexity theory (of lower bounds) we mean a theory for approaching
the $P$ vs. $NP$ and related  problems, then there are as many complexity 
theories as there are ways of formalizing this question reasonably, because
each such formalization  chalks out a way of crossing the
complexity barrier. GCT is one such way.
But there is one fundamental difference between computability theory
and complexity theory. We do not really expect many computability 
theories--i.e. ways of crossing the computability barrier--whereas we do expect
many complexity theories--i.e.  ways of crossing the complexity barrier. 


Now we have to explain what we mean 
by a reasonable  formalization of  Question~\ref{qfeasible}. We mean that 
it should be in the spirit of the reasonable formalization of 
Question~\ref{qcomputable} in \cite{church,turing}. Thus it should be 
absolutely precise and formal as in these articles, and the interpretation
of the phrase {\em theoretically feasible} should  be 
reasonable like the interpretation of the phrase {\em computable}
as in these articles. Specifically, we mean:

\begin{enumerate} 
\item[I] Give a mathematically precise formulation of  an  Obstruction
Hypothesis (OH) that is meant to be an alternative to IOH.
Here it must be proved unconditionally that OH implies  IOH.
Furthermore, this obstruction hypothesis should be of the form: 
\[({\bf OH}): \quad  \forall n \forall  m=\poly(n): s(n,m),\] 
where $s(n,m)$ is some formal mathematical statement. 
The statement $s(n,m)$ is supposed to  say that when $m=\poly(n)$ there 
exists  some cause of hardness (which we shall call an obstruction) 
because of which IOH holds. We put no restriction on the nature 
of this cuase. The cause could be existence of some
mathematical object in the spirit of a trivial obstruction, in which
case this object can be called an obstruction--an alternative to a
trivial obstruction.
But this is not necessary. The cause could be just some 
mathematical condition.
As long as it can be completely formalized in the form of a precise 
mathematical statement $s(m,n)$ and OH implies IOH unconditionally,
we do not care. We call OH a
{\em complexity theoretic hypothesis} because it is necessary that
$m$ be small in comparison to $n$ for it to hold.


\item[II] 
State precise formal {\em mathematical hypotheses} 
$MH1, MH2, \cdots, MH_r$, $r \ge 1$, and 
give a  mathematically  precise  formal  and reasonable definition of the
phrase {\em theoretical feasibility} (of OH)
such that if $MH_1,\cdots,MH_r$ hold then OH becomes theoretically 
feasible as per this definition.
Here theoretical feasibility of OH 
is supposed to mean that once $MH_1,\ldots,MH_r$
are proved  the $P\not = NP$ 
conjecture is not expected to stand in the way of proving OH thereafter.
Each mathematical hypothesis should be of the form 
\[ {\bf (MH_i):}  \forall n \forall m t_i(m,n), \] 
for some formal mathematical statements $t_i(m,n)$.
We are calling it mathematical because this is supposed to hold for
all $n$ and $m$, not just when $m=\poly(n)$ or small as in the
case of the complexity theoretic IOH or OH. 
In other words,  smallness  of $m$ with respect to  $n$, the 
complexity theoretic crux of the lower bound  problem under consideration, 
is supposed to be absent  in the mathematical hypotheses.

\item [III]
(a)  Give reasonable justification for  why OH should hold assuming IOH
(which we take on faith as true) or some reasonable stronger forms of IOH.
This is certainly a circular 
argument. Its only function here is to give us reasonable confidence
that  OH is actually true, i.e., there is no loss of truth in going 
from IOH to OH.

(b)  Give reasonable justification for why $MH_1,\ldots,MH_r$ should 
hold.

(c)  Give reasonable justification for why 
the $P \not = NP$ conjecture or some equally hard or harder 
complexity theoretic hypotheses  should
not stand in the way of proving $MH_1,\ldots, MH_r$ and
in the way of proving  OH once $MH_1,\ldots, MH_k$ are proved.
In other words, all these hypotheses should only involve ``easy'' 
complexity theoretic hypotheses, where by ``easy'' we mean the $P\not = NP$ 
conjecture or its equivalent or harder variants 
are not expected to stand in the way of their proofs.

At least one intuitve 
reason for why the $P\not = NP$ conjecture should not
stand in the way of proving the  mathematical hypotheses is already there:
namely, smallness of $m$ with respect $n$, the complexity theoretic crux of 
this  conjecture, is absent in these hypotheses. But just this is not enough. 
It is also necessary to give additional justifications as to why some
hard complexity theoretic hypotheses are not hidden or encoded within these 
mathematical hypotheses or  OH in some hard to recognize forms. 

\end{enumerate} 

\noindent {\em Remark:} In steps I,II, and III above 
we can substitute the usual uniform version of the $P\not = NP$ 
conjecture in place of IOH. That is, we do not really require here that 
the approach has  try to prove the stronger 
nonuniform version of the $P\not = NP$ conjecture. The usual uniform
version will do.


Once steps I to III are carried out  the 
``hard'' (i.e. theoretically infeasible) complexity
theoretic hypothesis IOH is transformed into an 
``easy'' (i.e. theoretically feasible) complexity theoretic hypothesis OH
with the help of a set of mathematical hypotheses $MH_1,\ldots,MH_k$
which too involve only ``easy'' complexity theoretic hypotheses, such
that the $P \not = NP$ conjecture is not expected to stand in the way of
the proofs of any of these ``easy'' complexity theoretic hypotheses.
Thus once Question~\ref{qfeasible} is fully formalized in this fashion,  hard 
complexity theory (IOH) is exchanged with hard mathematics 
($MH_1,\ldots,MH_r$ + OH). What is gained in this exchange is that 
the $P \not = NP$ conjecture is not expected to stand in the way 
doing this hard mathematics, and thus a fully formalized  mathematical 
program towards proving this  conjecture is chalked out.

We  say that {\em the feasibility barrier is crossed} (in this approach)
and that OH is {\em theoretically feasible} once $MH_1,\ldots,MH_r$
are proved--we also say that the proof strategy (approach) becomes 
theoretically feasible. Theoretical feasibility of the proof strategy 
does not automatically guarantee 
{\em practical feasibility}  of proving OH. That is, even after OH has
been proved to be theoretically feasible actually proving it may be
a mathematical challenge, though if it is a formally ``easy'' complexity
theoretic hypothesis then.
This is why we regarded  OH  as hard mathematics above.


Now arises the  next  question: 
what is meant by reasonable justifications in III? 
Certainly we cannot expect a proof technique to formally 
prove that the $P \not = NP$ 
conjecture or its harder variants 
would not stand in the way of proving $MH_1,\ldots,MH_r$ and
$OH$, because the only way to prove this formally is to actually prove them 
unconditionally thereby proving the $P \not = NP$ conjecture itself.
But this is a serious issue because regardless of how reasonable 
the justifications of a proof technique may look at the surface, 
what is the guarantee that 
the $P\not = NP$ conjecture or some 
equivalent  or harder complexity theoretic assumptions, such as 
existence of one way functions, pseudorandom generators etc. as per
the hardness vs. randomness principle \cite{nisan}, are not 
lying hidden within $MH_1,\ldots,MH_r$ and OH 
in some hard to recognize forms?  That is, what is the 
guarantee   that
the proof technique is not simply restating 
the problem in an equivalent terms  with  an ingenious encoding
and thus going   in circles, or worse,  making it harder
and thus going backwards, thereby simply evading 
Question~\ref{qfeasible} despite all this formalization?
Again we cannot ask for a complete guarantee, because that only comes
after proving $P \not = NP$. But we need some reasonable guarantee.


Towards that end,  we  stipulate 
that using  weaker forms of the proof technique it should be 
possible to prove 
unconditional lower bounds in restricted settings 
that meet   hard enough criteria of nontriviality.
Accordingly, we will say  that a proof strategy  is a {\em formal
approach towards the $P$ vs. $NP$ problem} if it meets the
following criteria: 



\begin{enumerate} 
\item[A]  Some weaker form of the  proof strategy yields 
a concrete unconditional superpolynomial 
lower bound that  is a 
restricted form and a formal implication 
of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] Some weaker form of the proof strategy 
yields a concrete    lower bound that is a restricted  form  of
of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} whose 
proof  demonstrates that the 
proof strategy  bypasses the earlier known  local barriers mentioned before.
Here, in view of the fundamental nature of these barriers and given
that they were proposed and accepted in the field as metabarriers,
we agree to take them in the meta sense--i.e., in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any proof strategy. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}
(this makes sense over the boolean field as well as over $\Q$ as long as
we take bitlengths of rational numbers into account in a natural way).
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.


\item[C] It provides a reasonable formalization of Question~\ref{qfeasible}
by carrying out steps I,II and III above.
\end{enumerate}

We shall refer to these as the criteria A,B, and C to determine if
a proof strategy is a formal approach. What is meant by  weaker forms
of the approach in A and B cannot be formalized. This should be clear 
by examining the proofs of the lower bounds in A and B.




All approaches can agree on A and B given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
implication of any of the fundamental separation 
problems in  Figure~\ref{fig:complexityclasses} 
and of crossing the earlier local barriers simultaneously has been
well recognized by now. An approach which is just restating the $P$ 
vs. $NP$ problem by hiding this conjecture or its equivalent or harder 
forms in any of its hypotheses will not be able to prove lower bounds 
that meet criteria A and B.
Hence if an approach can meet the criteria
A and B, this provides a 
reasonable guarantee  that it is not restating the original problem  and 
going in circles, which is  what crossing the complexity  barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem. Similarly, all approaches can agree on C given
that it has been accepted in the folklore that Question~\ref{qfeasible}
is the root difficulty of the $P$ vs. $NP$ problem and that any 
approach would have to finally answer it in one way or the other. 
But if a proof technique  cannot  even formally 
state the question that it is trying to answer how can we call it an approach? 

Once A, B, and C are met, the proof technique 
has chalked  out a complete mathematical program C towards the $P$ vs. $NP$
problem in the form of the hypotheses $MH_1,\ldots,MH_r$ and $OH$, provided 
reasonable justification  that the $P\not = NP$ conjecture should not 
stand in the way of proving $MH_1,\ldots,MH_r$ and hence $OH$,  and 
has provided  a reasonable guaratee  in the form of the landmarks
A and  B  that this path is actually going
forwards, and not in circles, or even worse, backwards. Hence it is then
reasonable to call it  a formal approach.



By a {\em complexity theory of the $P$ vs. $NP$ problem} we mean 
a mathematical theory of any formal approach towards this problem. 
Just as we have as many computability theories as there 
are formal approaches 
to cross the computability barrier, there are as many complexity 
theories of the $P$ vs. $NP$ problem as there are formal approaches to
cross the complexity barrier.
But unlike in the case of the computability theory, we expect
many complexity theories. 

The complexity barier can also be defined for other problems related 
to the $P$ vs. $NP$ problem, such as the $P$ vs. $NC$ or $\#P$ vs. $NC$ 
problems. Formal approaches and complexity theories associated with
these problems are defined similarly.

It may be noticed that the meaning of the phrase barrier in
complexity barrier is different from its meaning in the local barriers
such as the algebraic degree barrier. The algebraic degree barrier has a 
a precise and formal mathematical  definition, cf. Chapter 7 in GCTlocal.
In contrast, formalizing the complexity barrier is in fact 
a part  of that  barrier.
The complexity barrier is a 
barrier in the same sense that the computability barrier is a barrier.
There is no computability theory until the computability barrier is
formalized. Similarly, if we accept that Question~\ref{qfeasible} is the 
root difficulty of the $P$ vs. $NP$ problem, then there is no 
complexity theory of the $P$ vs. $NP$ problem in a formal sense 
until the complexity barrier is formalized.
In that sense we may say that the complexity barrier is the main
barrier of complexity theory. Whereas the algebraic degree barrier 
is more like a guiding post.
As long as we keep in  mind that  universal and 
local barriers are of a different kind, there should be no confusion.







==> complexity2.tex <==
\section{Complexity barrier} \label{scomplexity}
In this section we describe the complexity barrier.

Towards that end,    let us 
fix an  $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$, say SAT. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialobs}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.

\begin{figure} 
\begin{center}
\epsfig{file=trivialobs.eps, scale=.5}
\end{center}
      \caption{Trivial obstruction}
      \label{fig:trivialobs}
\end{figure} 



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so is the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any proof strategy for  the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} {\bf [The folklore version of the fundamental 
question of complexity theory]}
\label{qfeasible} 
Why should the
proof strategy  be  even  {\em theoretically  feasible}, i.e., 
lead to a proof even theoretically? 
In other words, in what sense is it fundamentally 
different from the  trivial, infeasible strategy  above
and not just a restatement of the original problem? 

In general, what is a {\em theoretically feasible proof strategy} for the 
$P$ vs. $NP$ problem? 
Does such a strategy even exist?
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the beginning  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem stated above.
These local  barriers   roughly say that the proof techniques akin to
the ones used for proving three types of lower bounds, 
namely the classical hierarchy theorems, lower bounds for 
constant depth circuits \cite{sipser} and the $P\not = NC$ result 
without bit operations [GCTlocal], would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
along with its variants and properties, 
rendering them theoretically infeasible, so to say.
Admittedly,  since these local barriers apply to 
proof techniques that constitute  only    very specific 
subareas of mathematics, 
we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions, why can it not
keep on  happening ad infinitum? 
This does not seem inconceivable 
since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the fundamental folklore question
that has been lurking in the background of the $P$ vs.
$NP$ problem right from the beginning:
why should a given proof technique 
be even {\em theoretically feasible}  as per some 
reasonable notion of theoretical feasibility. 


By the {\em  complexity barrier} we mean the task of answering this
Question~\ref{qfeasible} {\em formally}. The key phrase here is formally.
Because Question~\ref{qfeasible} itself is an informal folklore question
with no theorem or precise mathematics behind it. To answer it formally
means:

\begin{enumerate} 
\item[1] {\bf Formalize the question:} 
Fix a proof strategy and  formalize the question first by defining 
formally {\em theoretically feasibility} 
of this  proof strategy,
justify why this  is a reasonable formalization, and then
\item[2] {\bf Answer it:}
Answer the formalized question, i.e., prove that
the proof strategy under consideration is theoretically feasible
as per this formal definition.
\end{enumerate} 
Here step 1  may be possible 
for only  exceptional proof strategies. That is, the $P$ vs. $NP$ problem
seems so severe that it may not even allow most proof 
strategies to define formally their own theoretical feasibility, let alone
prove themselves to be theoretically feasible and come near the problem.
Thus formalization of the folklore question  as in step  1
is itself a part of the challenge, a part of the root difficulty in 
approaching the $P$ vs. $NP$ problem. 


This is not a new phenomenon.
Indeed, many fundamental questions in science are informal folklore 
questions and a part or sometimes the whole of the
challenge lies in just formalizing them.
For example:


\begin{question}{\bf [The folklore version of the fundamental 
question of computability theory] }

\label{qcomputable}
What is computable (decidable)? 
\end{question} 

This is informal. 
But the main challenge in computability theory as we know now--we shall
call this the {\em computability barrier}--was to  
formalize this question by giving a precise mathematical meaning to
the phrase {\em computable} (Computability Hypothesis proposed by Church and
Turing in  \cite{church,turing})
and then justify 
that  it is a reasonable formalization. 
Of course, formalization
of the phrase computable 
that we have today is  one reasonable  formalization--we shall also call it
a {\em formalization of the computability barrier} in the form of
a computability theory. Or, we will say that 
the present computability theory  is 
one way of formalizing  the computability barrier or one formal approach
to cross the computability barrier.
We cannot say that it is the only one. There may be other ways of 
reasonably formalizing  Question~\ref{qcomputable}.
Every such way will correspond to
a different computability theory.
But  there is just one computability theory today that has been universally 
accepted as reasonable. 



The formalization of this computability barrier is the key ingradient 
in proving  the fundamental Incompleteness Theorem of logic  proved by 
G\"odel  \cite{godel}--namely, that 
the language of true statements in number theory is undecidable.
Actually, the Incompleteness Theorem
predated computability theory and 
was originally  stated in terms of definability rather than computability.
But let us imagine asking
if  number theory is 
decidable, without even having a formal definition of  decidable.
(In fact, this is essentially  what happenned  in Entscheidungsproblem
posed by Hilbert \cite{hilbert} which
asked  if number theory  is decidable mechanically--and this
was just taken as a folklore notion.)
Then the fundamental difficulty in answering this question is 
just formalizing the informal Question~\ref{qcomputable}.
That is, formalization of the computability barrier above. Once this is done 
and  the phrase 
computable or decidable is given a formal meaning, it becomes possible to
prove the Incompleteness Theorem by encoding computations.
The Incompleteness Theorem 
is also a universal statement about mathematics like the $P$ vs. $NP$ problem.
Hence, it is especially relevant to study 
the  nature of the fundamental conceptual difficulty in its proof. 
As we see in retrospect,  this was basically 
formalizing the  fundamental  folklore Question~\ref{qcomputable}.
If so, it should not be surprising if at least a part of the 
fundamental conceptual difficulty in  the proof of the other 
universal statement about mathematics--the $P$ vs. $NP$ problem--should 
also be just formalizing some other  fundamental folklore  question.


Question~\ref{qfeasible} seems to be that  question.
As per the folklore, it 
is supposed to be the  root 
difficulty of the $P$ vs. $NP$ problem, and a part of this
difficulty is just formally stating what the question is saying, i.e,
formalizing this question by giving a precise 
mathematical meaning to  {\em theoretically feasibility} of a judiciously 
chosen proof strategy. 
If by complexity theory (of lower bounds) we mean a theory for approaching
the $P$ vs. $NP$ and related  problems, then there are as many complexity 
theories as there are ways of formalizing this question reasonably, because
each such formalization  chalks out a way of crossing the
complexity barrier. GCT is one such way.
But there is one fundamental difference between computability theory
and complexity theory. We do not really expect many computability 
theories--i.e. ways of crossing the computability barrier--whereas we do expect
many complexity theories--i.e.  ways of crossing the complexity barrier. 


Now we have to explain what we mean 
by a reasonable  formalization of  Question~\ref{qfeasible}. We mean that 
it should be in the spirit of the reasonable formalization of 
Question~\ref{qcomputable} in \cite{church,turing}. Thus it should be 
absolutely precise and formal as in these articles, and the interpretation
of the phrase {\em theoretically feasible} should  be 
reasonable like the interpretation of the phrase {\em computable}
as in these articles. Specifically, we mean:

\begin{enumerate} 
\item[I] Give a mathematically precise formulation of  an  Obstruction
Hypothesis (OH) that is meant to be an alternative to IOH.
Here it must be proved unconditionally that OH implies  IOH.
Furthermore, this obstruction hypothesis should be of the form: 
\[({\bf OH}): \quad  \forall n \forall  m=\poly(n): s(n,m),\] 
where $s(n,m)$ is some formal mathematical statement. 
The statement $s(n,m)$ is supposed to  say that when $m=\poly(n)$ there 
exists  some cause of hardness (which we shall call an obstruction) 
because of which IOH holds. We put no restriction on the nature 
of this cause. The cause could be existence of some
mathematical object in the spirit of a trivial obstruction, in which
case this object can be called an obstruction--an alternative to a
trivial obstruction.
But this is not necessary. The cause could be just some 
mathematical condition.
As long as it can be completely formalized in the form of a precise 
mathematical statement $s(m,n)$ and OH implies IOH unconditionally,
we do not care. We call OH a
{\em complexity theoretic hypothesis} because it is necessary that
$m$ be small in comparison to $n$ for it to hold.


\item[II] 
State precise formal {\em mathematical hypotheses} 
MH1, MH2, ... , MHr, $r \ge 1$, and 
give a  mathematically  precise  formal  and reasonable definition of the
phrase {\em theoretical feasibility} (of OH)
such that if MH1,...,MHr hold then OH becomes theoretically 
feasible as per this definition.
Here theoretical feasibility of OH 
is supposed to mean that once MH1, ..., MHr
are proved  the $P\not = NP$ 
conjecture is not expected to stand in the way of proving OH thereafter.
Each mathematical hypothesis should be of the form 
\[ {\bf (MHi):}  \forall n \forall m t_i(m,n), \] 
for some formal mathematical statements $t_i(m,n)$.
We are calling it mathematical because this is supposed to hold for
all $n$ and $m$, not just when $m=\poly(n)$ or small as in the
case of the complexity theoretic IOH or OH. 
In other words,  smallness  of $m$ with respect to  $n$, the 
complexity theoretic crux of the lower bound  problem under consideration, 
is supposed to be absent  in the mathematical hypotheses.

\item [III]
(a)  Give reasonable justification for  why OH should hold assuming IOH
(which we take on faith as true) or some reasonable stronger forms of IOH.
This is certainly a circular 
argument. Its only function here is to give us reasonable confidence
that  OH is actually true, i.e., there is no loss of truth in going 
from IOH to OH.

(b)  Give reasonable justification for why MH1,...,MHr should 
hold.

(c)  Give reasonable justification for why 
the $P \not = NP$ conjecture or some equally hard or harder 
complexity theoretic hypotheses  should
not stand in the way of proving MH1,..., MHr and
in the way of proving  OH once MH1,..., MHk are proved.
In other words, all these hypotheses should only involve ``easy'' 
complexity theoretic hypotheses, where by ``easy'' we mean the $P\not = NP$ 
conjecture or its equivalent or harder variants 
are not expected to stand in the way of their proofs.

At least one intuitive 
reason for why the $P\not = NP$ conjecture should not
stand in the way of proving the  mathematical hypotheses is already there:
namely, smallness of $m$ with respect $n$, the complexity theoretic crux of 
this  conjecture, is absent in these hypotheses. But just this is not enough. 
It is also necessary to give additional justifications as to why some
hard complexity theoretic hypotheses are not hidden or encoded within these 
mathematical hypotheses or  OH in some hard to recognize forms. 

\end{enumerate} 

\noindent {\em Remark:} In steps I,II, and III above 
we can substitute the usual uniform version of the $P\not = NP$ 
conjecture in place of IOH. That is, we do not really require here that 
the approach has  try to prove the stronger 
nonuniform version of the $P\not = NP$ conjecture. The usual uniform
version will do.


Once steps I to III are carried out  the 
``hard'' (i.e. theoretically infeasible) complexity
theoretic hypothesis IOH is transformed into 
complexity theoretic hypothesis OH which becomes 
``easy'' (i.e. theoretically feasible)  once 
the mathematical hypotheses MH1,...,MHk are proved, and these 
mathematical hypotheses too involve only ``easy'' complexity 
theoretic hypotheses, such
that the $P \not = NP$ conjecture is not expected to stand in the way of
the proofs of any of these ``easy'' complexity theoretic hypotheses.
Thus once Question~\ref{qfeasible} is fully formalized in this fashion,  hard 
complexity theory (IOH) is exchanged with hard mathematics 
(MH1,...,MHr + OH). What is gained in this exchange is that 
the $P \not = NP$ conjecture is not expected to stand in the way 
doing this hard mathematics, and thus a fully formalized  mathematical 
program towards proving this  conjecture is chalked out.
We say that the {\em complexity barrier is formalized} (in this approach)
once steps I to III are carried out and thus the folklore
Question~\ref{qfeasible} is formalized.


We  say that {\em the complexity barrier is crossed} (in this approach)
and that OH is {\em theoretically feasible} once MH1,...,MHr
are proved--we also say that the proof strategy (approach) becomes 
theoretically feasible. Theoretical feasibility of the proof strategy 
does not automatically guarantee 
{\em practical feasibility}  of proving OH. That is, even after OH has
been proved to be theoretically feasible actually proving it may be
a mathematical challenge, though  it is a formally ``easy'' complexity
theoretic hypothesis then.
This is why we regarded  OH  as hard mathematics above.


Now arises the  next  question: 
what is meant by reasonable justifications in III? 
Certainly we cannot expect a proof technique to formally 
prove that the $P \not = NP$ 
conjecture or its harder variants 
would not stand in the way of proving MH1,...,MHr and
$OH$, because the only way to prove this formally is to actually prove them 
unconditionally thereby proving the $P \not = NP$ conjecture itself.
But this is a serious issue because regardless of how reasonable 
the justifications of a proof technique may look at the surface, 
what is the guarantee that 
the $P\not = NP$ conjecture or some 
equivalent  or harder complexity theoretic assumptions, such as 
existence of one way functions, pseudorandom generators etc. as per
the hardness vs. randomness principle \cite{nisan}, are not 
lying hidden within MH1,...,MHr and OH 
in some hard to recognize forms?  That is, what is the 
guarantee   that
the proof technique is not simply restating 
the problem in an equivalent terms  with  an ingenious encoding
and thus going   in circles, or worse,  making it harder
and thus going backwards, thereby simply evading 
Question~\ref{qfeasible} despite all this formalization?


To see the seriousness of this issue, let us imagine ourselves  in the 
early seventies, before the work on pseudo-random generators, derandomization,
one-way functions and so forth began, and imagine that  some proof technique 
came along claiming to be an approach to the $NEXP$ vs. $P/poly$ 
problem--which is far, far weaker than the $P$ vs. $NP$ problem,
but let us ignore that--by  reducing this problem to 
the problem of showing that polynomial 
identity testing belongs to $P$ and then claiming to be theoretically
feasible because the latter is an upper bound problem involving $P$ which
stands for theoretically feasible. At that time  this
may have seemed like a reasonable justification. After all, if a proof
technique has reduced a lower bound problem to an upper bound problem 
over $P$, then it seems like  progress, at least, at the surface. 
Coming to back to the present, we know now, thanks to all the work on
the hardness vs. randomness principle \cite{hastad2,nisan,russell}
that has happenned in the meanwhile,
that the proof technique was just going in circles. Because polynomial
identity testing belongs to $BPP$ and as per \cite{russell} derandomization
of polynomial identity testing essentially amounts to proving the
original lower bound problem or worse the  harder permanent vs. determinant
problem. In other words, the hardness vs. randomness principle tells us today
that all arguments which look like reductions to 
upper bound problems at the surface 
but involve pseudorandom generators, one way functions, derandomizations,
and so forth  are circular, 
something that we may not have seen so clearly in the seventies. 

Indeed, one significant
outcome of the works on $NP$-completeness \cite{cook,karp,levin},
plausible formal independence of the $P$ vs. $NP$ problem 
(surveyed in \cite{aaronsonformal}),  the  local
barriers \cite{solovay,rudich,GCTlocal,aaronson},
and the hardness vs. randomness principle 
\cite{hastad2,nisan,russell} in the last few decades 
was the discovery of the formidable  circle around the $P$ vs. $NP$ 
problem. That is, they together raised Question~\ref{qfeasible} and 
pointed  out the extreme difficulty of penetrating this circle.



Which is why, though we cannot ask 
for a complete guarantee that the $P\not = NP$ conjecture or its
variants would not stand in the way of proving MH1,...MHr, and OH,
because that only comes
after proving $P \not = NP$,  we need at least some reasonably {\em hard}
guarantee that the proof technique has indeed penetrated 
this  circle.


To see how to get such a hard guarantee, let us closely compare 
the circle around the $P$ vs. $NP$ problem with  the one around 
the Incompleteness Theorem and then try to
transfer what we already know about how the circle around the latter was 
penetrated to get an idea about how the proof technique 
that penetrates the circle around the former ought to be.
There is a circle around the Incompleteness Theorem 
because when it says there exist unprovable statements
in mathematics or that the truth in number theory is undecidable 
it {\em seems} as if it is also hinting that it may be
unprovable itself or that its truth may be undecidable. There is a circle 
around the $P$ vs. $NP$ problem, because when it says that 
discovery is hard it {\em seems} as if it is also hinting that the discovery
of its own proof may be hard. Any proof strategy for the Incompleteness
Theorem or the $P$ vs. $NP$ problem has to break this
self-referential paradox--the circle. The conceptual breakthrough in 
\cite{godel} was to break this circle for the Incompleteness 
Theorem and show that it is talking about the rest of mathematics not itself.
If we closely examine the proof strategy in \cite{godel}, we see that it
is {\em extremely rigid}.
By this we mean that we know just one way of penetrating this circle
today, and though there are many versions and proofs of the Incompleteness
theorem, all of them essentially use the same basic idea.
Similarly, the formalization
of the the computability barrier  in \cite{church,turing}--the key 
ingradient in proving the Incompleteness Theorem--is also 
{\em extremely rigid}.
By this, we mean
we know just one reasonable formalization of the computability barrier today.
So far, we do not know any other formalization 
that is ``more or less reasonable'', ``close to reasonable'' or 
``almost reasonable''. 
In short, it is a $0$-$1$ game: it either works completely or fails completely.
We expect this $0$-$1$ game to continue 
in the $P$ vs. $NP$ problem as well.


This $0$-$1$ game cannot be  formalized.
But we can  state a certain   Rigidity Hypothesis formally which 
intuitively suggests this $0$-$1$ game for the complexity barrier as well.
Towards that end, let us assume that the proof technique has 
provided  as in the
the natural proof paper \cite{rudich} 
a formal statement 
of a Useful Property ($UP_n$), which lies at its heart, and assuming which 
it plans to prove $P \not = NP$. Formally, $UP_n$ is a subset of the set
of all $n$-ary boolean functions. Its definition is 
as in \cite{rudich} and we do not restate it here. 
Let $N=2^n$ be the truth table size of specifying any $n$-ary boolean 
function.


\begin{defn} \label{drigidcomplexity}
We say that a proof technique 
is 
\begin{enumerate} 
\item 
{\em Nonrigid} if  $|UP_n| \ge 2^N/N^c$, for some constant $c>0$,
\item {\em Mildly rigid} if $|UP_n| \le 2^N /N^c$ for every constant $c>0$,
as $n\rightarrow \infty$,  or
more strongly, $|UP_n| \le 2^N/2^{n^a}$, for some constant $a\ge 1$,
\item {\em Rigid} if  $ |UP_n| \le 2^{\epsilon N}$,
for some $0 \le \epsilon < 1$, 
\item {\em Strongly rigid} if 
$|UP_n| \le 2^{N^\epsilon}$, for some $0 \le \epsilon < 1$,  and 
\item {\em Extremely rigid} if 
$|UP_n| \le 2^{\poly(n)}$, i.e., $\le 2^{n^a}$ for some constant $a>0$.
\end{enumerate}
\end{defn} 

Thus probabilistic proof techniques to which the natural proof
barrier \cite{rudich} applies are nonrigid, and 
if a proof technique is mildly rigid it bypasses this
barrier, since it violates the largeness criterion in \cite{rudich}. 

\begin{hypo}[Rigidity Hypothesis (RH)] 
Any eventual proof (technique) that shows $P\not = NP$ is 
extremely rigid.
\end{hypo} 

The natural proof paper says that any eventual proof of the $P\not = NP$ 
conjecture is mildly rigid (assuming 
some hardness assumptions and an additional constructivity criterion). 
The Rigidity Hypothesis says  that the reality is extremely 
severe compared to this. Its detailed discussion with motivations etc.
will appear in GCTflip.

Computability Hypothesis \cite{church,turing} says that 
there is essentially just one reasonable way to formalize the computability 
barrier and that way--i.e., the specific notion of computability that 
we have today--is extremely rigid as explained above. 
In the case of the complexity barrier there need not be just one 
way to formalize it. The Rigidity Hypothesis suggests that that 
each way may be  extremely rigid again--i.e., the notion 
``a theoretically feasible proof technique''
may  also be an extremely rigid notion like ``computable''.
Unfortunately, we cannot formally define extreme rigidity of a notion. 
The Rigidity Hypothesis is the best that we can do formally. 
It is talking about extreme rigidity of a proof, but that may be taken
as suggesting extreme rigidity of the notion of 
``a theoretically feasible proof technique'', i.e., extreme rigidity of 
formalizing  the complexity barrier 
as in the case of the computability barrier.
Intuitively, this suggests that 
a formalization of the complexity barrier may be  either 
completely right or completely wrong like in the case of the computability
barrier. 
Which is why if a formalization  is reasonable  and
extremely rigid, then intuitively we 
expect only  two possibilities: either 
it is really an approach to the $P$ vs. $NP$ problem or just 
a circular  restatement, and we have to distinguish between the two. 
For this, all we have to do is to insist that some restricted form 
of the proof strategy  also 
yield an  unconditional  lower bound that is nontrivial  enough so that if
the proof strategy    were circular it will simply not be able to 
provide such a lower bound.  Furthermore, we also insist that 
the proof strategy  should  provide evidence that 
it  bypasses the earlier known local barriers.
If it does, then assuming that it is a  $0$-$1$ 
game, there is a reasonable assurance that 
the  formalization is indeed an approach to the $P$ vs. $NP$ problem.





With this  in mind, 
we will say  that a proof strategy  is a {\em formal
approach towards the $P$ vs. $NP$ problem} if it meets the
following criteria: 

\begin{enumerate} 
\item[A]  Some weaker form of the  proof strategy yields 
a concrete unconditional superpolynomial 
lower bound that  is a 
restricted form and a formal implication 
of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.

\item[B] The proof strategy bypasses the earlier known  
local barriers mentioned before simultaneously.
Here, in view of the fundamental nature of these barriers and given
that they were proposed and accepted in the field as metabarriers,
we agree to take them in the meta sense--i.e., in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any proof strategy. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}
(this makes sense over the boolean field as well as over $\Q$ as long as
we take bitlengths of rational numbers into account in a natural way, and 
if a restricted model is natural enough--which we require--it 
should come with  a natural meaning for most).
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.


\item[C] It provides a reasonable formalization of Question~\ref{qfeasible}
by carrying out steps I,II and III above.

We also require that the  OH in the proof of the lower bound in B be 
a natural restricted form of the OH in this formalization.

\item[D] (Extreme Rigidity): It formally states 
the UP for the $P$ vs. $NP$ problem. It should be clear that this UP 
lies at the heart of  the approach. 
We also require that the UP in the proof of the lower bound in B be a natural
restricted form of this UP. 
\end{enumerate}

We shall refer to these as the criteria A,B, C, and D to determine if
a proof strategy is a formal approach. 




All approaches can agree on A and B given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
implication of any of the fundamental separation 
problems in  Figure~\ref{fig:complexityclasses} 
and of crossing the earlier local barriers simultaneously has been
well recognized by now. An approach which is just restating the $P$ 
vs. $NP$  or related problem, such as the hypothetical proof strategy 
in the seventies above, by hiding the original lower bound problem
or its equivalent or harder 
forms in any of its hypotheses will not be able to prove lower bounds 
that meet criteria A and B.
Hence if an approach can meet the criteria
A and B, this provides a 
reasonable hard guarantee  that it is not restating the original problem  and 
going in circles, which is  what crossing the complexity  barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem. 
Similarly, all approaches can agree on C given
that it has been accepted in the folklore that Question~\ref{qfeasible}
is the root difficulty of the $P$ vs. $NP$ problem and that any 
approach would have to finally answer it in one way or the other. 
But if a proof technique  cannot  even formally 
state the question that it is trying to answer how can we call it an approach? 
Motivation behind D is the Rigidity Hypothesis stated above.

Once A, B, C, D are met, the proof technique 
has chalked  out a complete 
mathematical program C towards the $P$ vs. $NP$
problem in the form of the hypotheses MH1,...,MHr and OH, provided 
reasonable  justification  that the $P\not = NP$ conjecture should not 
stand in the way of proving MH1,...,MHr and hence OH,  and 
has provided  a reasonable hard guarantee  in the form of the landmarks
A and  B  that this path is actually going
forwards,  not in circles, or even worse, backwards, and has shown
that the program is extremely rigid. It is then
reasonable to call it  a formal approach to the $P$ vs. $NP$ problem
in view of the Rigidity Hypothesis and the  remarks  before and
after that hypothesis above. 



By a {\em complexity theory of the $P$ vs. $NP$ problem} we mean 
a mathematical theory of any formal approach towards this problem. 
Just as we have as many computability theories as there 
are formal approaches 
to cross the computability barrier, there are as many complexity 
theories of the $P$ vs. $NP$ problem as there are formal approaches to
cross the complexity barrier.
But unlike in the case of the computability theory, we expect
many complexity theories--though as we have already said, 
the $P\not = NP$ conjecture seems  so severe that each such complexity
theory may have to be exceptional (like the present computability theory) 
because otherwise formalization of the complexity barrier may simply be
impossible (as in the case of the computability barrier).



The complexity barrier can also be defined for other problems related 
to the $P$ vs. $NP$ problem, such as the $P$ vs. $NC$ or $\#P$ vs. $NC$ 
problems. Formal approaches and complexity theories associated with
these problems are defined similarly.

It may be noticed that the meaning of the phrase barrier in
complexity barrier is different from its meaning in the local barriers
such as the algebraic degree barrier. The algebraic degree barrier has a 
a precise and formal mathematical  definition, cf. Chapter 7 in GCTlocal.
In contrast, formalizing the complexity barrier is in fact 
a part  of that  barrier.
The complexity barrier is a 
barrier in the same sense that the computability barrier is a barrier.
There is no computability theory until the computability barrier is
formalized. Similarly, if we accept that Question~\ref{qfeasible} is the 
root difficulty of the $P$ vs. $NP$ problem, then there is no 
complexity theory of the $P$ vs. $NP$ problem in a formal sense 
until the complexity barrier is formalized.
In that sense we may say that the complexity barrier is the main
barrier of complexity theory. Whereas the algebraic degree barrier 
is more like a guiding post.
As long as we keep in  mind that  universal and 
local barriers are of a different kind, there should be no confusion.







==> explicitconj1.tex <==
\section{C: On crossing  the feasibility barrier  over finite fields} 
\label{sexpli}
Before we turn to that question, 
in this section we briefly discuss  the conjectural scheme 
for crossing the feasibility barrier via the flip for the
usual $\#P$ vs. $NC$ and $P$ vs. $NP$ problems defined over finite
fields (e.g. boolean). 

This is based on the following.



\begin{conj}[Explicit proof conjecture] (GCT6) (Characteristic zero)
\label{cexpproof0} 
The geometric obstructions for the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems 
in characteristic zero  defined in GCT1,2, and which 
were  discussed in Section~\ref{sgeomobs}, are extremely explicit. 
This means they are short, easy to verify, discover
and decode
(cf. Definitions~\ref{defnobstexplicit},\ref{defnobsstrongexp},\ref{ddecodeQ}).
Furthemore, short geometric obstructions
exist in the problems under consideration. Hence, extremely explicit  
proofs based on these geometric obstructions exist.
\end{conj}

(This is a strengthened from of PHflip in the earlier version of GCT6.)


\begin{conj} [Explicit proof conjecture] (GCT6) (Positive characteristic)
\label{cexpproofpos}
Similarly the analogous 
geometric obstructions for the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems 
in characteristic zero as defined in GCT6 over $\bar F_p$, the algebraic 
closure of the finite field $F_p$, $p$ a larg enough prime of $\poly(n)$,
are extremely explicit. Furthemore, such short geometric obstructions exist.
Hence, extremely explicit proofs bases on these geometric obstructions 
exist.
\end{conj}

\begin{theorem}[GCT6] \label{texpproof}
An extremely explicit proof  for the $\#P$ vs. $NC$ or $P$ vs. $NP$ 
conjecture over $\bar F_p$ as in Conjecture~\ref{cexpproofpos} implies 
an extremely explicit proof for these problems over $F_p$, and 
also over the boolean field, i.e., for the usual forms of the nonunifrom 
$\#P$ vs $NC$ and $P$ vs. $NP$ conjectures.
\end{theorem}

This suggests the following strategy for proving the $\#P \not = NC$ 
and $P \not = NP$ conjectures:

\begin{enumerate} 
\item[I] Find  extremely explicit proofs  for the 
$\#P$ vs. $NC$ and $P$ vs. $NP$ problems
in  characteristic zero as in Conjecture~\ref{cexpproof0}.

\item[II] Lift them  to get  extremely explicit proofs for these problem over
$\bar F_p$, for a suitable $p$ as in Conjecture~\ref{cexpproofpos}.

\item[III] By Theorem~\ref{texpproof} this implies extremely explicit proofs
over $F_p$ and the boolean field, the usual case.
\end{enumerate} 



Theoorem~\ref{texpproof}  reduces 
the search  for extremely explicit proofs over the  boolean field
(the usual case) to  the search for 
extremely explicit proofs over $\bar F_p$, for a large enough $p$.
The advantage of this reduction is that
the methods of algebraic geometry become applicable
over  algebraically closed fields. But algebraic geometry
in positive characteristic is harder than algebraic geometry in 
characteristic zero. This is why the goal is 
to get   an extremely explicit 
proof in characteristic zero  first (step I) and then lift it to 
algebraically closed fields of positive characteristic (step II). 
This {\em lift} 
promises to be a formidable mathematical challenge. A detailed
discussion of the problems  that need to be addressed in this lift
and additional relevant problems over finite fields will appear in GCT11.
Just as an example,
one of the crucial results that is used in the proof of Theorem~\ref{tgct6},
or rather a result needed to justify PH1 therein, is the 
resolution of singularities in characteristic zero \cite{hironaka}. Lifting
this resolution  to positive 
characteristic is one of the outstanding problems 
in algebraic geometry.  But the $P \not = NP$ conjecture is not expected 
to stand in the way of this lift, since the difficulty here is  
mathematical, not complexity theoretic. Similarly, 
if Conjecture~\ref{} can be proved, the 
$P \not = NP$ conjecture is not expected to stand in the way of
lifting its  proof (as in step II) to that of
Conjecture~\re{}.
Furthermore, the $P \not = NP$ conjecture is also not expected to stand in
the way of the decoding algorithm either, as we already discussed in
Section~\ref{sflip}.
Hence,  one may say that this approach should be  theoretically
feasible once  its  theoretical feasibility 
is established in characteristic zero, i.e., once the feasibility barrier is 
crossed in characteristic zero.  By Theorem~\ref{tgct6}, this means 
once PH1/PH4 is proved. 


\section{Why should PH1 hold and how to prove it?} \label{showph}
Thus  theoretical feasibility of this approach hinges on  PH1 and PH4.
Let us just consider here PH1 (b), which is a basic propertype 
for general PH1 and PH4. 

The coefficients $G_{\lambda,m}(k)$ that occur in PH1 (b) 
are known as Kroncker coefficients in representation theory and hence we shall
refer to PH1 (b) as Kroncker PH1. It is a complexity 
theoretic version of the fundamental Kronecker problem in representation
theory that   has been intensively studied in the last century and 
is known to be formidable. And now 
it lies at the heart of this approach towards $P$ vs. $NP$. 

A special case of  Kronecker PH1 has been solved in representation theory.
for a very special class of Kronecker coefficients 
called Littlewood-Richardson (LR) coefficients. These 
are basically the multiplicities in the 
analogous  PH1 that occurs in the proof of the
mathematical form of the $\#P\not = NC$ conjecture (Theorem~\ref{}).
We shall refer to this special case of the Kronecker PH1 
that occurs in the proof of the mathematical form as LR PH1.



A basic plan to prove Kronecker PH1 (and its 
generalization in representation theory called Plethysm PH1) that 
lies at the heart of PH1 (a)  is given in [GCT4,6,7,8].
See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH1 based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that the tensor 
product of two   Weyl modules of $SL_n(\C)$
has a canonical basis \cite{kashiwara,lusztig} 
whose structural parameters that determine the action of the
generators of $SL_n(\C)$ on this basis are all nonnegative  \cite{lusztig}
The only known proofs of this positivity 
result are based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2}  and the related works \cite{beilinson}, and
the simpler one goes via the theory of standard quantum group \cite{drinfeld}.
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Kronecker PH and its generalizations 
in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Kronecker PH. This is precisely 
is a generalization of LR PH0 called Kronecker PH0.
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 


Initial  steps in this direction have been taken in GCT4,7,8. 
First, GCT4 and 7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
and plays the
same role in the Kornecker (and plethysm)
setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
supported by experimental numerical evidence generated with the help
of a computer.


This numerical evidence is the main evidence for Plethysm PH0
and hence Plethysm PH1 and its generalization PH1. 
It is reasonable because positivity (Plethysm PH0) is an extremely rigid 
property. Specifically, the structure coefficients involved in Plethysm
PH0 are extremely complex mathematical quantities whose computation 
involves summing exponentially many terms of alternating signs.
If there were no reason for them to have any specific sign, 
they would be positive or negative with roughly the same probability,
naively speaking, and the probability that several hundred of these
mathematical quantities (which were computed) 
would all turn out to be of the same sign would be  absurdly  small. 
Hence, this seems to be  a reasonble evidence  that PH1 should hold. 
But the question is how to prove it? 





For that we have to complete the 
commutative diagram in Figure~\ref{fig:lift}. What is needed 
for this completion  is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 


Thus the ultimate goal of GCT would be  to deduce the ultimate 
negative hypothesis of mathematics, $P \not = NP$ conjecture (in characteristic
 zero), 
from the ultimate positive hypotheses--namely, as yet unknown,
nonstandard Riemann
hypotheses (over finite fields); cf. Figure~\ref{fig:finalgoal}.
The reader may have noticed something striking here. Namely,
to prove the $P \not = NP$ conjecture in characteristic zero what is
needed is not nonstandard extension of the work surrounding the
Riemann hypothesis in characteristic zero (that is the standard 
Riemann hypothesis) but rather the one over finite fields. 
This flip from characteristic zero to finite fields happens in 
the theory of quantum groups for some profound reasons \cite{lusztig} that 
we shall not go into here. Similarly, the opposite flip is also plausible: 
namely, for proving the analogue of PH1 in positive characteristic
[GCT11]  nonstandard extension of the work surrounding  the usual Riemann 
hypothesis over $\Z$, or rather its generalizations that occur in
arithmetic algebraic geometry and the theory of automorphic forms
may be needed. 

Thus  this plan for implementing  the flip seems  to be a massive affair.







\begin{figure} 
\begin{center}
\psfragscanon
\epsfig{file=finalgoal.eps, scale=.6}
\end{center}
      \caption{The ultimate goal of GCT}
      \label{fig:finalgoal}
\end{figure}

\section{Is  all this necessary?} 
That leads to the final inevitable question: is all this 
really necessary? There are two questions here.
First, is positivity in abstract GCT necessary? 
And second, is abstract GCT, i.e., geometric flip based on 
extremely rigid explicit constructions, necessary? 


Let us deal with the first question first. Here the 
existing mathematical evidence and arguments [GCTflip] 
suggest that any abstract GCT approach
to cross the feasibility  barrier would have to say  
something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly};
a detailed story and a precise meaning of the key 
phrase {\em implicit} will appear in the revised version of GCTflip.
Thus,   positivity (Plethysm PH and PH0)  seems to lie at the heart 
of abstract  GCT, and if we wish to follow this approach then 
we have to be willing face profound positivity questions in mathematics.





That then leads to the second question. In this context,
we have already remarked that there is no reason to believe that
abstract GCT is the only appraoch towards $P$ vs. $NP$, and that
there ought to be  nonconstructive approaches as well, perhaps several.
But these unnatural approaches may turn out to be even
harder than the natural approach. A concrete evidence towards this 
is provided in Figure~\ref{fig:summary}, which 
summarizes the discussion in this article.
Here it can be seen that as the lower bounds start moving towards the 
$P$ vs. $MP$ problem their existing
proof techniques  become more and more geometric,
explicit, and rigid for some inexplicable reasons that we do not
understand. 

Another evidence in this direction is provided by the fundamental work on 
explicit construction of Ramanujan graphs \cite{sarnak}, which was
in fact a starting motivation for  GCT.  At present, this is the  only 
known way of showing existence of  Ramanujan graphs,
and it needs explicit construction
that  is extremely rigid in the sense that it proves Ramanujan property for 
only extremely special graphs. 
As per the natural proof barrier, 
Ramanujan graphs seem to be the only expander graphs  that are 
useful in the context of  lower bounds. Because most graphs are expanders
and hence in the terminology of \cite{rudich}  expansion is not
a useful property in this context, whereas 
though most graphs are close to Ramanujan \cite{friedman}, they are not 
expected to be exactly Ramanujan. That is, the Ramanujan property 
gets out of the jaws of the natural proof barrier, though  just barely. 
The proof of correctness of explicit Ramnujan graphs in \cite{sarnak} 
also  needs the Riemann hypothesis over finite fields (for curves).
But explicit Ramnujan graphs   cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results may 
need  much  more because the universal
feasibility barrier seems far more severe than
the local natural proof barrier that the Ramanujan graphs clear.
Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for extremely rigid explicit constructions in GCT, 
that is only to be expected.

Also, the feasibility barrier is universal. So if profound 
positivity properties are needed to cross it in  one approach
then  it is plausible that they may 
be neeeded in one way or the other to cross it via  any other approach
because that is what universal is supposed to mean.

All this  suggests that in the context of the $P$ vs. $NP$ problem
there may be after all something special about  geometry, extremely rigid
explicit constructions, positivity, and the Riemann hypothesis,
and unless and until we have a concrete 
alternative approach that meets the criteria A, B and C, it may make sense
to just stick to the obvious and the natural, i.e.,  GCT.

But paradoxically the obvious and the natural
has turned out to be such a massive affair that
it is fair to say that what has been done in GCT so far is only 
the easy initial part--easy in comparison to what remains to be done--and the 
hard part (positivity)  is yet to begin. And the hard part seems so 
hard that without an extensive collaboration between complexity theory
and mathematics further progress on this approach seems unlikely. It
is our hope that this small initial step towards the $P$ vs. $NP$  problem
will lead to such extensive collaboration between the two fields.




\begin{figure} 
\begin{center} 
\epsfig{file=summary.eps, scale=.9}
\end{center}
      \caption{Circuits lower bounds vs. their proof techniques}
      \label{fig:summary}
\end{figure} 












==> feasibility.tex <==
\section{Complexity barrier}
Before we turn to the complexity barrier, let us see why 
the  earlier known barriers towards the $P$ vs. $NP$ problem 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
and algebraic-degree [GCTlocal] barriers do not seem to  capture the root 
difficulty of the $P$ vs. $NP$ problem. 

To be specific, let us consider the algebraic degree barrier in [GCTlocal].
It basically says that low degree techniques of the kind used in that 
paper  would not help in the
fundamental separation problems. All these techniques are in one way or
the other related to the fundamental Bezout's theorem in algebraic geometry
(we also include the low degree techniques used in the proof of the IP=PSPACE
and PCP results in this category). Though this is a nontrivial area of
mathematics, it is still very small compared to the whole of mathematics.
Hence, we can say that this  barrier is {\em local} 
in the sense that it applies to a very 
restricted class of techniques in mathematics. Furthermore, we can say 
that this barrier is primarily {\em mathematical} in the sense that low degree 
is really a purely a mathematical notion, there is no complexity theory in it,
and though it  is very useful in complexity theory, this barrier is really a 
statement about the restricted nature  of these mathematical 
techniques rather than about the complexity theoretic difficulty 
of  the $P$ vs. $NP$ problem.
In a similar way, we can say that the relativization and natural proof 
barriers are also local and mathematical. The latter because the natural 
proof barrier is generally regarded as applying to proof techniques that 
work for most functions, and most is a mathematical notion, 
so also the notion of relativization.

Unfortunately after  GCT1 and 2, wherein these local mathematical
barriers were bypassed in a sense explained in Section~\ref{},  
it became clear that  the root 
difficulty of the $P$ vs. $NP$ problem still remains after bypassing
them  and the  main battle 
on the $P$ vs. $NP$ problem  really begins only after bypassing them.

In retrospect, this should not be surprising. 
We cannot expect local mathematical 
barriers to capture the root difficulty of the $P$ vs. $NP$ problem,
because this problem is a {\em universal complexity} 
statement about all of mathematics.
Namely, if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal complexity theoretic 
nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal} and {\em complexity theoretic},
where by a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
A local barrier only  rules out a 
restricted  area of mathematics. 
Regardless of how many restricted   areas of mathematics we rule 
out in this way, that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do
given that the $P$ vs. $NP$ problem is a statement about all of mathematics. 
At some point we have to turn our attention from what is not to be done
to  what is to be done
and identify the root universal and complexity theoretic 
difficulty of this problem; i.e., 
a universal complexity theoretic barrier.

The complexity  barrier seems to be this universal complexity theoretic 
barrier.
Due its universality, it seems quite formidable, as expected.
To describe it,   let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any proof strategy for  the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} 
Why should the proof strategy  be  even  {\em theoretically  feasible}, i.e., 
lead to a proof even theoretically? 
In other words, in what sense is it fundamentally 
different from the  trivial, infeasible strategy  above
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem stated above.
These local  barriers   roughly say that the proof techniques akin to
the ones used for proving three types of lower bounds, 
namely the classical hierachy theorems, lower bounds for 
constant depth circuits \cite{sipser} and the $P\not = NC$ result 
without bit operations, would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
along with its variants and properties, 
rendering them theoretically infeasible, so to say.
Admittedly,  since these local barriers apply to 
proof techniques that constitute  only    very specific 
subareas of mathematics, 
we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions, why can it not
keep  happening ad infinitum? 
This does not seem inconceivable 
since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the fundamental folklore question
that has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining:
why should a given proof technique 
be even {\em theoretically feasible}  as per some 
reasonable notion of theoretical feasibility. 


By the {\em  complexity barrier} we mean the task of answering 
Question~\ref{qfeasible} {\em formally}. The key phrase here is formally.
Because Question~\ref{qfeasible} itself is an informal folklore question
with no theorem or precise mathematics behind it. To answer it formally:
\begin{enumerate} 
\item The proof technique  has to first formalize the question by giving 
precise mathematical meaning to the phrase {\em theoretically feasible proof 
strategy},
justify why this  is a reasonable formalization, and then
\item Answer the formalized question, i.e., prove that
the proof strategy under consideration is theoretically feasible
as per this formal definition of theoretical feasibility. 
\end{enumerate} 
In other words,
formalization of the question  is itself a part of the challenge, a part 
of the root difficulty.

This is not a new phenomenon either. 
Indeed, many fundamental questions in science are informal folklore 
questions and a part or sometimes the whole of the
challenge lies in just formalizing them.
For example, one well known folklore question of computer science is: 
what is computable (decidable)? This is informal. 
But the main challenge in computability theory as we know now 
\cite{church,turing}--we shall
call this the {\em computability barrier}--was to  
formalize this question by giving a precise mathematical meaning to
the phrase {\em computable} and then justify 
that  it is a reasonable formalization. 
Of course, formalization
of the phrase computable 
that we have today is  one reasonable  formalization. We will say that 
the present computability theory  is 
one way of crossing the computability barrier.
We cannot say that it is the only one. There may be other ways of 
reasonably formalizing this question. Every such way will correspond to
a different computability theory.
But if there are other reasonable computability theories,  
we do not know them today.


The crossing of the computability barrier is the key ingradient 
in proving the Incompleteness Theorem of logic \cite{}--namely, that 
the language of true statements in number theory is undecidable.
Actually, the Incompleteness Theorem
predated theory of computability and 
was originally  stated in terms of definability rather than computability.
But let us ignore the history and imagine asking, 
as was essentially done in \cite{hilbert}, if  number theory is 
decidable, without actually knowing what decidable really means. 
Then the fundamental difficulty in answering this question is 
just formalizing the informal question--what is decidable (computable)? 
That is, crossing of the computability barrier above. Once this is done 
and  the phrase 
computable or decidable is given a formal meaning, proving Incompleteness 
Theorem is essentially routine--it only needs   encoding of computations.
The Incompleteness Theorem 
is also a universal statement about mathematics.
Indeed, this is essentially the
only universal statement about mathematics that we know today other than
the $P$ vs. $NP$ problem. Hence, it is especially relavant to study 
the  nature of the fundamental conceptual difficulty in its proof. 
As we see in retrospect,  this was basically 
formalizing a fundamental  informal question--what is computable?. If so, 
it should not be surprising if at least a part of the 
fundamental conceptual difficulty in  the proof of the other 
universal statement about mathematics--the $P$ vs. $NP$ problem--should 
also be just formalizing some other  fundamental informal question.




Question~\ref{qfeasible} seems to be that  other fundamental informal
question. As per the folklore, it 
is supposed to be the  root 
difficulty of the $P$ vs. $NP$ problem, and a part of this
difficulty is just formally stating what the question is saying, i.e,
formalizing this question by giving a precise 
mathematical meaning to the phrase {\em theoretically feasible 
proof strategy}. 
If by complexity theory (of lower bounds) we mean a theory for approaching
the $P$ vs. $NP$ and related  problems, then there are as many complexity 
theories as there are ways of formalizing this question reasonably. 


By a reasonable  formalization of  Question~\ref{qfeasible}
we mean:
\begin{enumerate} 
\item[I] Give a mathematically precise formulation of  an  Obstruction
Hypothesis (OH) that is meant to be an alternative to IOH.
Here it must be proved unconditionally that OH implies  IOH.
Furthermore, this obstruction hypothesis should be of the form: 
\[({\bf OH}): \quad  \forall n \forall  m=\poly(n): s(n,m),\] 
where $s(n,m)$ is some formal mathematical statement. 
The statement $s(n,m)$ is supposed to  say that when $m=\poly(n)$ there 
exists  some cause of hardness (which we shall call an obstruction) 
because of which IOH holds. We put no restriction on the nature 
of this cuase. The cause could be existence of some
mathematical object in the spirit of a trivial obstruction, in which
case this object can be called an obstruction--an alternative to a
trivial obstruction.
But this is not necessary. The cause could be just some 
mathematical condition.
As long as it can be completely formalized in the form of a precise 
mathematical statement $s(m,n)$ and OH implies IOH unconditionally,
we do not care. We call OH a
{\em complexity theoretic hypothesis} because it is necessary that
$m$ be small in comparison to $n$ for it to hold.


\item[II] 
State precise formal {\em mathematical hypotheses} 
$MH1, MH2, \cdots, MH_r$, $r \ge 1$, and 
give a  mathematically  precise  formal  definition of the
phrase {\em theoretical feasibility} (of OH)
such that if $MH_1,\cdots,MH_r$ hold then OH becomes theoretically 
feasible as per this definition.
Here theoretical feasibility of OH 
is supposed to mean that once $MH_1,\ldots,MH_r$
are proved  the $P\not = NP$ 
conjecture is not expected to stand in the way of proving OH thereafter.
Each mathematical hypothesis should be of the form 
\[ {\bf ($MH_i$):}  \forall n \forall m t_i(m,n), \] 
for some formal mathematical statements $t_i(m,n)$.
We are calling it mathematical because this is supposed to hold for
all $n$ and $m$, not just when $m=\poly(n)$ or small as in the
case of the complexity theoretic IOH or OH. 
In other words,  smallness  of $m$ with respect to  $n$, the 
complexity theoretic crux of the lower bound  problem under consideration, 
is supposed to be absent  in the mathematical hypotheses.

\item [III]
Give reasonable justification for  why OH should hold assuming IOH
(which we take on faith as true) or some reasonable stronger forms of IOH.
This is certainly a circular 
argument. Its only function here is to give us reasonable confidence
that  OH is actually true, i.e., there is no loss of truth in going 
from IOH to OH.

Give reasonable justification for why the $P \not = NP$ conjecture should
not stand in the way of proving $MH_1,\ldots, MH_r$ and
in the way of proving  OH once $MH_1,\ldots, MH_k$ are proved.
At least one intuitve 
reason for why the $P\not = NP$ conjecture should not
stand in the way of proving the  mathematical hypotheses is already there:
namely, smallness of $m$ with respect $n$, the complexity theoretic crux of 
this  conjecture, is absent in these hypotheses. But just this is not enough. 
It is also necessary to give additional justifications as to why some
hard complexity theoretic hypotheses are not lying hidden within these 
mathematical hypotheses. 
\end{enumerate} 
Once steps I to III are carried out  the 
``hard'' (i.e. theoretically infeasible) complexity
theoretic hypothesis IOH is transformed into an 
``easy'' (i.e. theoretically feasible) complexity theoretic hypothesis OH
with the help of a set of mathematical hypotheses $MH_1,\ldots,MH_k$.



We  say that {\em the feasibility barrier is crossed} (in this approach)
and that OH is {\em theoretically feasible} once $MH_1,\ldots,MH_r$
are proved. We also say that the proof strategy (approach) becomes 
theoretically feasible. Theoretical feasibility of the proof strategy 
does not automatically guarantee 
{\em practical feasibility}  of proving OH. That is, even after OH has
been proved to be theoretically feasible actually proving it may be
a mathematical challenge, even if it is formally ``easy'' then.
Thus once Question~\ref{qfeasible} is fully formalized in this fashion,  hard 
complexity theory (IOH) is exchanged with hard mathematics 
($MH_1,\ldots,MH_r$ + OH). What is gained in this exchange is that 
the $P \not = NP$ conjecture is not expected to stand in the way 
doing this hard mathematics, and thus a fully formalized  mathematical 
program towards proving this  conjecture is chalked out.

Now arises the  next  question: 
what is meant by reasonable justifications in I, II, III? 
Certainly we cannot expect a proof technique to formally 
prove that the $P \not = NP$ 
conjecture would not stand in the way of proving $MH_1,\ldots,MH_r$ and
$OH$, because the only way to prove this formally is to actually prove them 
unconditionally thereby proving the $P \not = NP$ conjecture itself.
But this is a serious issue because regardless of how reasonable 
the justifications of a proof technique may look at the surface, 
what is the guarantee that 
the $P\not = NP$ conjecture or some 
equivalent  or harder complexity theoretic assumptions, such as 
existence of one way functions, pseudorandom generators etc. as per
the hardness vs. randomness principle \cite{}, are not 
lying hidden within $MH_1,\ldots,MH_r$ and OH 
in some hard to recognize forms?  That is, what is the 
guarantee   that
the proof technique is not simply restating 
the problem in an ingenious way 
and going   in circles, or worse,  making it harder
and going backwards, thereby simply evading 
Question~\ref{qfeasible} despite all this formalization?
Again we cannot ask for a complete guarantee, because that only comes
after proving $P \not = NP$. But we need some reasonable guarantee.


Towards that end,  we  stipulate 
that using  weaker forms of the proof technique it should be 
possible to prove 
unconditional lower bounds in restricted settings 
that meet   hard enough criteria of nontriviality.
Accordingly, we will say  that a proof strategy  is a {\em concrete 
approach towards the $P$ vs. $NP$ problem} if it meets the
following criteria: 



\begin{enumerate} 
\item[A]  Some weaker form of the  proof strategy yields 
a concrete unconditional superpolynomial 
lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] Some weaker form of the proof strategy 
yields a concrete    lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
proof strategy  bypasses the earlier known  local barriers mentioned before.
Here, in view of the fundamental nature of these barriers and given
that they were proposed and accepted in the field as metabarriers,
we agree to take them in the meta sense--i.e., in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any proof strategy. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}
(this makes sense over the boolean field as well as over $\Q$ as long as
we take bitlengths of rational numbers into account in a natural way).
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.


\item[C] The proof strategy has completely formalized  Question~\ref{qfeasible}
by carrying out steps I,II and III above.
\end{enumerate}

We shall refer to these as the criteria A,B, and C to determine if
a proof strategy is a concrete approach.


All approaches can agree on A and B given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, this provides a 
reasonable guarantee  that it is not restating the original problem or 
going in circles, which is  what crossing the complexity  barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem. Similarly, all approaches can agree on C given
that it has been accepted in the folklore that Question~\ref{qfeasible}
is the root difficulty of the $P$ vs. $NP$ problem and that any 
approach would have to finally answer it in one way or the other. 
But if a proof technique  cannot  even formally 
state the question that it is trying to answer how can we call it an approach? 









The  feasiblity   barrier seems to be    the root cause 
of  the  difficulties in the $P$ vs. $NP$ and related problems, and 
not surprisingly,  turns out to be extremely formidable. Indeed, 
all the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. Hence it is elaborated 
here so that the need for  the nonelementary techniques 
that enter into GCT to tackle this barrier becomes clear at a high level.


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present concrete
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the feasibility barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present we are not aware of  any other superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier. Furthermore, 
being purely algebraic and degree independent, it 
is fundamentally different from the known proofs to which
the relativization \cite{solovay}, and 
algebraic degree [GCTlocal] barriers apply, and hence, 
it bypasses these barriers too in this sense.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit}  basically says that 
any low degree or degree based proof technique, such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. As far as we can see, the  recent 
algebrization barrier \cite{aaronson} also says   something similar.
Hence it is not treated  separately in this article.

Though the proof of the mathematical form above thus bypasses the earlier 
known barriers, that is unfortunately not enough.
Because in a sense the main battle 
on the $P$ vs. $NP$ problem seems to begin only after bypassing these
earlier barriers. 
In retrospect, this should not be surprising. To see why, let us observe that
these earlier barriers are 
{\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
But  the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal}. By a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.

The  feasibility barrier seems to be  this universal barrier.
It is  simply the task of answering the following question: 

\begin{question} {(bf Feasibiilty barrier)}
Why should a given proof technique be even theoretically feasible, i.e., 
lead to a proof even theoretically?
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers mentioned above. Indeed all these local barriers 
roughly say that the proof techniques akin to
the ones used for proving lower bounds for classical hierarchy theorems,
constant depth circuits \cite{sipser}, $P\not = NC$ result without bit
operations  would not work for the $P$ vs. $NP$ problem
in a sense because the problem  
itself  stands in their way, along with its variants and related  properties,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   very specific 
subareas of mathematics, which is why these  barriers can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions to the proof 
techniques for the lower bounds associated with these barriers, 
why could it not keep on happening again and again?
This does not seem inconceivable since the problem itself says that the 
discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It seems  universal in the sense that Question~\ref{qfeasible}
seems to be the root difficulty of  proving the $P\not = NP$ 
conjecture, and 
every approach may ultimately have to face it in one way or the other.


There is though a fundamental difference between this barrier
and the earlier local barriers. The latter are mathematical barriers 
based on precise mathematical statements. Whereas the feasibility barrier
is based on only  a vague philosophical   question with 
no theorem or precise mathematics behind it. 
Unfortunately, the precisely stated  mathematical local 
barriers do not seem to  capture the root difficulty of the
the $P$ vs. $NP$ problem. Because each local barrier only rules out a 
small area of mathematics. For example, the algebraic degree barrier 
in [GCTlocal] rules out low degree techniques in mathematics.
Though this is a substantial subarea of mathematics, it is still very 
small compared to the whole of mathematics. 
Regardless of how many restricted   areas of mathematics we knock 
out on the basis of such local barriers that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do,
given that the $P$ vs. $NP$ problem is a statement about all of mathematics.
Indeed this is precisely 
what happened after the work on GCT1 and 2 was finished.
It was realized then that though the earlier local barriers were bypassed 
similtaneously therein, the root difficulty of the $P$ vs. $NP$ problem
was yet not addressed.
And Question~\ref{} seems to be that root difficulty.


Fortunately, though this question cannot be formalized,
the most obvious approach to answer it (the flip) can be. 
That is, GCT gives a precise 
mathematical definition of theoretical feasibility, 
justifies why it is a reasonable notion, and 
then formulates precise mathematical hypotheses such that once 
these are proved the approach  is  theoretical feasible
and Question~\ref{} is answered, i.e.,
the feasibility barrier is crossed in this formal mathematical sense.
Specifically, the main result of GCT [GCT6,7,8,11]
says that this barrier can be crossed subject to some mathematical positivity 
hypotheses called PH1 and PH4, whose high level description is
given here (cf. Section~\ref{swithoutbit}), and which turn out 
to be intimately  related to the Riemann Hypothesis over finite fields 
\cite{} and related positivity questions in the theory of 
of quantum groups.  The articles GCT6,7,8,11 also propose a plan for proving
these positivity hypotheses and provide concrete mathematical evidence
and justifications for why they should hold. 
Implementation of this plan seems to be a highly nontrivial 
affair,  and it is fair 
to say that what has been done in GCT so far is only the easy part of this
implementation and the hard part (positivity) is yet to begin.  
Rather the main result of GCT at present  lays out
a precisely formulated mathematical program to cross the feasibilty barrier
based on the most obvious flip strategy
with concrete lower bounds and results in its justification.
And  though there is no theorem or precise mathematics behind Question~\ref{}, 
there is a theorem (Theorem~\ref{}) and precise mathematics in 
the form of PH1 and PH4 behind this particular way of answering it.
The mathematical story surrounding positivity hypotheses (PH1/4) is far 
beyond the scope of this article. 
The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures where this story is discussed and PH1 and 
PH4 are laid out with full mathematical details.


It must be stressed here that there may be other nonobvious ways of
crossing the feasibility barrier, perhaps several. But at present 
we do not have any other program for  answering Question~\ref{} 
which can thus be chalked out and
formalized in precise mathematical terms. 
In fact, this formal chalking out of the program, i.e.
precise formalization  of all mathematical
hypotheses to answer Question~\ref{}, with concrete lower bounds and results
in their justification which meet certain criteria A, B, C stated in 
Section~\ref{}, is a critical part of   
what it means to cross the feasibility barrier. 
This can be done at present only the most obvious way.
Whether there are  similarly formalizable  nonobvious ways is open at present.





\ignore{
It 
is our hope that this small initial step towards the $P$ vs. $NP$ problem 
will bring  out  formidability of the feasibility barrier, its 
intimate relationship with deep posititivity issues in mathematics, and
perhaps  suggest what needs to be done in future for progress on these 
fundamental  issues in mathematics  and complexity theory.}



without getting into the philosophical 
issues concerning  the feasibility barrier. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such philosophical 
issues may wish to read that article first and come back to this
article later. The reader who would rather stick
to mathematics and not worry about philosophy may just  skip this 
article and proceed to \cite{}. But the reader who wishes to
know the root cause of all the 
difficulties and the need for  nonelementary 
techniques  at a philosophical level before getting into any mathematics 
may wish to read this article first. 
We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The feasibility barrier
is discussed in Section~\ref{sfeasibility}, the flip in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, 
the main result, a conjectural scheme 
for crossing the feasibility barrier via  flip, in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
feasibility barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is grateful to 
Josh Grochow,  Hari Narayanan, Partha Niyogi, and Janos Simon for discussions 
that were helpful in writing this article.




==> feasibility1.tex <==
\section{The  feasibility barrier} \label{sfeasibility} 
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quite formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it is difficult to 
formalize it fully.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible, i.e., lead to a proof
even theoretically? In other words, in what sense is it fundamentally 
different from the  trivial, infeasible approach above
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem 
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier   roughly says that the proof techniques akin to
the ones used for proving lower bounds for 
constant depth circuits \cite{sipser},
would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a  local
barrier (for the reasons explained in more detail in Sections~\ref{sflip}
and \ref{scharsym}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify the  meaning of answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggests such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,monotone,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
for every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{agarwal} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
decoding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or for that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results
\cite{sipser,monotone,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonuniform obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments like the ones  based on uniform 
objects such as  conjectural pseudo random generators 
which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there seems to be  a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  superpolynomial lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier known  local barriers mentioned before.
%relativization \cite{solovay}, natural-proof \cite{rudich}, and
%algebraic degree [GCTlocal] barriers simultaneously.
Here, in view of the fundamental nature of these barriers,
we agree to take them in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any approach. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}.
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.
\item[C] Concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.




==> feasibility2.tex <==
\section{The  feasibility barrier} \label{sfeasibility} 
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quite formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it is difficult to 
formalize it fully.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible, i.e., lead to a proof
even theoretically? In other words, in what sense is it fundamentally 
different from the  trivial, infeasible approach above
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem 
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier   roughly says that the proof techniques akin to
the ones used for proving lower bounds for 
constant depth circuits \cite{sipser},
would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a  local
barrier (for the reasons explained in more detail in Sections~\ref{sflip}
and \ref{scharsym}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify the  meaning of answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggests such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,monotone,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
for every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{agarwal} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
decoding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or for that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results
\cite{sipser,monotone,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonuniform obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments like the ones  based on uniform 
objects such as  conjectural pseudo random generators 
which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there seems to be  a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  superpolynomial lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier known  local barriers mentioned before.
%relativization \cite{solovay}, natural-proof \cite{rudich}, and
%algebraic degree [GCTlocal] barriers simultaneously.
Here, in view of the fundamental nature of these barriers,
we agree to take them in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any approach. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}.
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.
\item[C] Concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.




==> flip1.tex <==
\section{The flip: going for explicit construction} \label{sflip}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of a (nonuniform)
obstruction (cf. Definition~\ref{dobst})
that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}.
Formally:

\begin{defn} \label{defnobstexplicit}
We say that an obstruction family ${\cal O}$ (Definition~\ref{dobst}) 
is {\em explicit} if:
\begin{enumerate}
\item {\bf Shortness:}
For any $n$ and $m< 2^n$, if there exists  an 
obstruction in ${\cal O}_{n,m}$ 
to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction $O_{n,m}$ in ${\cal O}_{n,m}$, 
where by short we mean 
the bitlength $\bitlength{O_{n,m}}$ of its specification is
$\poly(n)$ (note the bound does not depend on $m$).
\item {\bf Easy-to-verify:} Given $n,m$ and a bit string $x$, whether 
it is the specification $[O_{n,m}]$ of an obstruction  
$O_{n,m} \in {\cal O}_{n,m}$ can be decided  in $\poly(n,\bitlength{x})$
time, where $\bitlength{x}$ denotes the bitlength of $x$.
\end{enumerate}
\end{defn} 

This means that the problem of verifying (recognizing)
an obstruction (or rather its specification) belongs to $P$, and hence,
is theoretically feasible (``easy''). Thus this notion 
of an obstruction is then fundamentally better than the theoretically
infeasible trivial obstruction as far as verification is concerned.





Now, to prove $P \not = NP$ it  suffices  to show that 
${\cal O}_{n,m}$ is nonempty if $m=\poly(n)$, $n \rightarrow \infty$.
In this step, the approach should also justify on the basis of
mathematical evidence why this should be
so assuming  $P \not = NP$ (nonuniform).
This circular reasoning at this stage is only meant to convince us 
before we  plunge ahead that such obstructions should exist, i.e., there 
is no loss of essential information,  
assuming $P \not = NP$, which we take on faith, and the goal
now is to prove the existence of these obstructions.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of 
the new  explicit 
obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
to verify if $f(X)=F_C(X)$, we have to evaluate 
$f_C(X)$,   cannot be  done   in polynomial time, i.e., in
$n^a$ time for some fixed $a>0$,  if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$) or alternatively,
if $m=n^b$ where $b$ is much larger than $a$. In other words,
even one row of a trivial obstruction cannot be evaluated in
$n^a$ time for any fixed $a$.
To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in $O(n^a)$ time for some fixed $a$, but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction using
the associated decoding procedure to get an exponential
size trivial obstruction. In fact, this seems impossible even 
if we were to allow ourselves $\poly(m)$ time, because verification of 
a trivial obstruction given in the form of an oracle (say) is a 
$\Pi_2$-problem which we do not expect to belong to $P$ if $P \not = NP$.
Thus it may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way. That is,
the computational complexity of the associated decoding algorithm 
(which we are only assuming is decidable) could be extremely high. 
And for that matter, we do not even need such a decoding algorithm 
as long as there is a guarantee that existence of an obstruction implies
existence of a trivial obstruction.
But if it is possible to get a trivial obstruction from a new obstruction
easily; i.e., if the asociated {\em decoding algorithm} works in polynomial
time, by  which we mean 
given specification of 
a new obstruction $O_{n,m}$ and a small $C$ of size $m$ it
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Note that if $O_{n,m}$ is short, i.e., $\bitlength{O_{n,m}}=\poly(n)$,
then this running time is $\poly(n,m)$.
Though we do not need the decoding algorithm to work in
polynomial time, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


It may be noticed that a final proof of the $P \not = NP$ conjecture 
is  an explicit obstruction for every $n$ and $m=\poly(n)$ 
as per Definition~\ref{defnobstexplicit} since it can be verified 
in $O(1)$ time. That is how it ought be since a final proof is 
the most explicit obstruction to the equality  of $NP$ with $P$ that one
can imagine. Similarly, an $O(1)$-size  program  for a one 
way function is an explicit obstruction for every $n$ and $m=\poly(n)$ 
after there is a final proof 
that it is indeed a one way function, i.e., when it is accompanied by
such a final proof  (without  it it is not even an 
obstruction, as already pointed out). 
But we are assuming here that the approach has not been
so lucky as to come with a final proof right in the first step. That is, 
the new obstruction in this first step is not a 
final proof or  accompanied by a final proof
but only a vehicle towards the final proof
as in the proofs of the earlier nonuniform lower bounds. 





\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing the specification of
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Formally, 

\begin{defn} \label{defnobsstrongexp}
We say that an explicit family of obstructions
(Definition~\ref{defnobstexplicit})
is {\em strongly explicit} if 
there is a discovery algorithm that given any $n$ and $m < 2^n$ 
decides in $\poly(n)$ time if ${\cal O}_{n,m}$ is nonempty
and, if so, produces in this much time specification $[O_{n,m}]$ of
an obstruction $O_{n,m} \in {\cal O}_{n,m}$.

We say that a strongly explicit family is {\em extremely explicit} 
if the obstructions are easy to decode; i.e., 
given the specifcation of a new obstruction $O_{n,m} \in {\cal O}_{n,m}$
and a small $C$ of size $m$ the associated decoding algorithm 
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$. 
\end{defn}

Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_{n,m} \in {\cal O}_{n,m}$. 

%We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs the specification of 
an obstruction $O_{n,m}$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
%If it is correct, we 
%call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

\begin{defn} \label{dexpproof}
We  call a proof of the $P\not = NP$ conjecture an {\em explicit proof}
based on the given notion of obstructions if 
it is based on the flip and carries out the step I, a {\em strongly explicit
proof} if it carries out both steps I and II, and an 
{\em extremely explicit proof} if
in addition, the obstructions are easy to decode.
\end{defn}

Explicit and strongly explicit proofs 
that go for proof-certificates that are easy to verify and discover make sense
in  a large class of problems in mathematics, 
not  just in complexity theory as here. See \cite{GCTflip} for a 
detailed discussion of explicit proofs in mathematics (they were
referred to as $P$-verifiable and $P$-constructible proofs in the earlier 
version of GCTflip). 
We shall not worry about this wider issue  here.

We  say that OH becomes {\em theoretically feasible}
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then become theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH, and 
however hard the task of proving OH may be mathematically,
the $P\not = NP$ conjecture  can be expected not to stand in the way
of its proof.
Hence, the name of this strategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both the barriers are 
crossed. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach   basically
means that the $P\not = NP$ conjecture should 
no longer stand in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{pi3}{{\small $\Pi_3$}}
\psfrag{pi2}{{\small $\Pi_2$}}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{{\small $T$}}
\psfrag{inpi3}{{\small $DP(IOH) \in \Pi_3$}}
\psfrag{inNP}{{\small $DP(OH) \in NP$}}
\psfrag{inP}{{\small $DP(OH) \in P$}}
\epsfig{file=IOHcomplexityintro.eps, scale=.8}
\end{center}
      \caption{The flip and the polynomial time hierarchy}
      \label{fig:IOHcomplexityintro}
\end{sidewaysfigure}



Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{eqiohp}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_3$. We refer to this as the decision
problem associated with IOH and denote it by $DP(IOH)$.
When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
Let $DP(OH)$ be  the decision problem 
associated with OH, by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ and $m$ specified in unary. 
It belongs  to $NP$
after execution of the step I and to $P$ after the step II.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that  $DP(IOH) \in \Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH logically (both becoming tautologies),
and yet the decision problem for the 
new OH for general $m$ 
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH is also a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, such reduction
of a universal statement in $\Pi_3$ to another in $NP$ and then
to $P$ may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{fig:IOHcomplexityintro},
it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.





For mathematical problems which are not universal, theoretical feasibility
can be meaningless. For example, consider 
a trivial  assertion $\forall A, B: A + B = B + A$ where $A$ and $B$ 
are $n\times n$ matrices.
The problem of brute force verification of this assertion 
belongs to $\Pi_1$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality and because 
those alternating quantifiers are intimately related to the 
the alternating quantifiers used to define the conjecturally 
noncollapsible  polynomial time hierarchy.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 


The  flip can also be formulated
in the theory of pseudorandom generators. For that we  fix 
an explicit $NP$-computable pseudorandom generator 
$g$ that conjecturally fools 
small  circuits (assuming which  $P \not = NP$). We  then express 
this property as an IOH for $g$ and associate a decision problem with it.
But it will be seen that this decision problem lies even higher in
the complexity hierarachy than the IOH for the $P$ vs. $NP$ problem; 
specifically it lies  in $\Pi_3^{BPP}$. Hence
the corresponding flip, which begins at this IOH  and runs towards FOH for $g$ 
through the complexity hierarchy, is harder.
In other words,  this says  that the theory
of pseudorandom generation (derandomization)
is in general  harder than the theory of lower bounds, and hence,
hardness should be proved first  and then transformed into
pseudorandom generation  as per the hardness vs. randomness 
principle \cite{nisan}. This is why we focus on lower bounds in GCT at present.





The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
\ignore{It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.}
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. The same  for a local strongly explicit obstruction.
In this sense, the global flip is stronger than the local flip.
The global   flip also implies   the local  flip if there is a polynomial 
time decoding algorithm, since then 
from a  global  obstruction one can get 
a local  strongly  explicit  obstruction easily. 
The $P\not = NP$ conjecture is not expected to 
stand in the way of this decoding since it simply amounts to spelling out 
what the approach has been doing implicitly anyway.
Hence intuitively the global (strong) flip subsumes the local (strong) flip.
A local strong flip is used in the proof of the $P\not = NC$ result 
without bit operations described below (Section~\ref{swithoutbit}).
But it does not seem 
effective for the harder separation problems in view of the algebraic 
degree barrier discussed below (Section~\ref{swithoutbit}).
%We do not understand why. 







The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.



So far we have been assumming that the underlying field of 
computation is the boolean field. But the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems can also be defined over an arbitrary ring or
field, and we are  specifically  interested in 
the rings and fields of characteristic zero such as $Z$, $\Q$ and $\C$. 
Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
By the nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
we mean  the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
But we shall not worry about it here because all the basic ideas of GCT
are  illustrated in the $\#P$ vs. $NC$ problem in characteristic zero.
We  focuss  on characteristic zero  in this article  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

The flip can also be defined for the $P$ vs. $NP$ and $\#P$ vs. $NC$ 
problems over fields of characteristic zero such as $Q$ or $\C$ and for
algebraically closed fields of positive characteristic such as $\bar F_p$, 
the algebraic closure of the finite field $F_p$, $p$ prime.
All  definitions in the flip 
can be lifted to this setting in the obvious way. We  only give
one critical definition as an illustration:

\begin{defn} \label{ddecodeQ}
Assume that the underlying 
field is $Q$. In this case we say that an
obstruction family is {\em easy to decode} 
if there is a decoding algorithm which given the specification of 
an obstruction $O=O_{n,m}$ and a small circuit $C$ over $\Q$ of size $m$ 
(i.e. whose whole description is of bitlength $m$)
produces in $\poly(n,m, \bitlength{O})$ time a counter example (local
obstruction) $X$ for 
$C$ whose description has  $\poly(n,\bitlength{O})$ bitlength, 
independent of $m$ as long as it is $\le n^{\log n}$ (say). If 
$\bitlength{O}$ is $\poly(n)$ the bitlength of $X$ is then $\poly(n)$
independent of $m$. In other words, smallness
of  obstructions independent of $m$ is to be preserved
in the process of decoding.

Definition over $\bar F_p$ is analogous.
\end{defn} 



The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts are fine and also inevitable as long as 
the spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip also has the following disturbing   feature.
Namely,  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, as per the flip,  modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same.
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.

After all the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Theorem~\ref{tmathform}) has a nonconstructive   proof
which applies to only very specific  functions (generalized permanents) 
and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in this   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative.
After all, as pointed out in Section~\ref{sfeasibility}, 
any approach to the $P$ vs. $NP$ problem has 
to meet at least the criteria A, B, and C stated there.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{swithoutbit}) addresses (A).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{smathform})   addresses (B).
The main result [GCT6,7,8,11] of GCT  (cf. Sections~\ref{sgct6} and 
\ref{sexpli})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero;
[GCT6,11] does  the same for   any
field including the finite field (the usual case). This
addresses (C). 


But, at present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction.


We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.


==> flip2.tex <==
\section{The flip: going for explicit construction} \label{sflip}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point of view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short of polynomial-size and easy to verify in polynomial-time, 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of a (nonuniform)
obstruction (cf. Definition~\ref{dobst})
that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}.
Formally:

\begin{defn} \label{defnobstexplicit}
We say that an obstruction family ${\cal O}$ (Definition~\ref{dobst}) 
is {\em explicit} if:
\begin{enumerate}
\item {\bf Shortness:}
For any $n$ and $m< 2^n$, if there exists  an 
obstruction in ${\cal O}_{n,m}$ 
to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction $O_{n,m}$ in ${\cal O}_{n,m}$, 
where by short we mean 
the bitlength $\bitlength{O_{n,m}}$ of its specification is
$\poly(n)$ (note the bound does not depend on $m$).
\item {\bf Easy-to-verify:} Given $n$ in unary, $m$ in binary 
and a bit string $x$, whether 
it is the specification $[O_{n,m}]$ of an obstruction  
$O_{n,m} \in {\cal O}_{n,m}$ can be decided  in $\poly(n,\bitlength{x})$
time, where $\bitlength{x}$ denotes the bitlength of $x$
(note the bound again does not depend on $m$).
\end{enumerate}
\end{defn} 

This means that the problem of verifying (recognizing)
an obstruction (or rather its specification) belongs to $P$, and hence,
is theoretically feasible (``easy''). Thus this notion 
of an obstruction is then fundamentally better than the theoretically
infeasible trivial obstruction as far as verification is concerned.





Now, to prove $P \not = NP$ it  suffices  to show that 
${\cal O}_{n,m}$ is nonempty if $m=\poly(n)$, $n \rightarrow \infty$.
In this step, the approach should also justify on the basis of
mathematical evidence why this should be
so assuming  $P \not = NP$ (nonuniform).
This circular reasoning at this stage is only meant to convince us 
before we  plunge ahead that such obstructions should exist, i.e., there 
is no loss of essential information,  
assuming $P \not = NP$, which we take on faith, and the goal
now is to prove the existence of these obstructions.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of 
the new  explicit 
obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
to verify if $f(X)=f_C(X)$, we have to evaluate 
$f_C(X)$,   cannot be  done   in polynomial time, i.e., in
$n^a$ time for some fixed $a>0$,  if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$) or alternatively,
if $m=n^b$ where $b$ is much larger than $a$. In other words,
if $a$ is fixed and we want to evaluate circuits of polynomial size
of nonfixed degree we are in trouble and 
even one row of a trivial obstruction cannot be evaluated in
$n^a$ time for any fixed $a$
To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in $O(n^a)$ time for some fixed $a$, but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction using
the associated decoding procedure to get an exponential
size trivial obstruction. In fact, this seems impossible even 
if we were to allow ourselves $\poly(m)$ time, because verification of 
a trivial obstruction given in the form of an oracle--let us call it
$O$--is a 
$\Pi_2^O$-problem, which we do not expect to belong to $P$ if $P \not = NP$.
Thus it may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way. That is,
the computational complexity of the associated decoding algorithm 
(which we are only assuming is decidable) could be extremely high. 
And for that matter, we do not even need such a decoding algorithm 
as long as there is a guarantee that existence of an obstruction implies
existence of a trivial obstruction.
But if it is possible to get a trivial obstruction from a new obstruction
easily; i.e., if the asociated {\em decoding algorithm} works in polynomial
time, by  which we mean 
given specification of 
a new obstruction $O_{n,m}$ and a small $C$ of size $m$ it
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counterexample $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Note that if $O_{n,m}$ is short, i.e., $\bitlength{O_{n,m}}=\poly(n)$,
then this running time is $\poly(n,m)$.
Though we do not need the decoding algorithm to work in
polynomial time, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


It may be noticed that a final proof of the $P \not = NP$ conjecture 
is  an explicit obstruction for every $n$ and $m=\poly(n)$ 
as per Definition~\ref{defnobstexplicit} since it can be verified 
in $O(1)$ time. That is how it ought to be since a final proof is 
the most explicit obstruction to the equality  of $NP$ with $P$ that one
can imagine. Similarly, an $O(1)$-size  program  for a one 
way function is an explicit obstruction for every $n$ and $m=\poly(n)$ 
after there is a final proof 
that it is indeed a one way function, i.e., when it is accompanied by
such a final proof  (without  it it is not even an 
obstruction, as already pointed out). 
But we are assuming here that the approach has not been
so lucky as to come with a final proof right in the first step. That is, 
the new obstruction in this first step is not a 
final proof or  accompanied by a final proof
but only a vehicle towards the final proof
as in the proofs of the earlier nonuniform lower bounds. 





\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing the specification of
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Formally, 

\begin{defn} \label{defnobsstrongexp}
We say that an explicit family of obstructions
(Definition~\ref{defnobstexplicit})
is {\em strongly explicit} if 
there is a discovery algorithm that given any $n$ and $m < 2^n$ 
decides in $\poly(n)$ time if ${\cal O}_{n,m}$ is nonempty
and, if so, produces in this much time specification $[O_{n,m}]$ of
an obstruction $O_{n,m} \in {\cal O}_{n,m}$.

We say that a strongly explicit family is {\em extremely explicit} 
if the obstructions are easy to decode; i.e., 
given the specification of a new obstruction $O_{n,m} \in {\cal O}_{n,m}$
and a small $C$ of size $m$ the associated decoding algorithm 
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counterexample $X$ for 
$C$. 
\end{defn}

Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_{n,m} \in {\cal O}_{n,m}$. 

%We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs the specification of 
an obstruction $O_{n,m}$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
%If it is correct, we 
%call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

\begin{defn} \label{dexpproof}
We  call a proof of the $P\not = NP$ conjecture an {\em explicit proof}
based on the given notion of obstructions if 
it is based on the flip and carries out  step I, a {\em strongly explicit
proof} if it carries out both steps I and II, and an 
{\em extremely explicit proof} if
in addition, the obstructions are easy to decode.
\end{defn}

Explicit and strongly explicit proofs 
that go for proof-certificates that are easy to verify and discover make sense
in  a large class of problems in mathematics, 
not  just in complexity theory as here. See [GCTflip] for a 
detailed discussion of explicit proofs in mathematics (they were
referred to as $P$-verifiable and $P$-constructible proofs in the earlier 
version of GCTflip). 
We shall not worry about this wider issue  here.

We  say that OH becomes {\em theoretically feasible}
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then become theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH, and 
however hard the task of proving OH may be mathematically,
the $P\not = NP$ conjecture  can be expected not to stand in the way
of its proof.
Hence, the name of this strategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both steps I and II are 
caried out. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach   basically
means that the $P\not = NP$ conjecture should 
no longer stand in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there seems to be   a serious problem.



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{pi3}{{\small $\Pi_3$}}
\psfrag{pi2}{{\small $\Pi_2$}}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{{\small $T$}}
\psfrag{inpi3}{{\small $DP(IOH) \in \Pi_3$}}
\psfrag{inNP}{{\small $DP(OH) \in NP$}}
\psfrag{inP}{{\small $DP(OH) \in P$}}
\epsfig{file=IOHcomplexityintro.eps, scale=.8}
\end{center}
      \caption{The flip and the polynomial time hierarchy}
      \label{fig:IOHcomplexityintro}
\end{sidewaysfigure}



Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $f(X) \not = f_C(X)$
belongs to $P^{NP}$.
Since there are two alternating layers of quantifiers in (\ref{eqiohp}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_2^{NP} \subseteq \Pi_3$.
We refer to this as the decision
problem associated with IOH and denote it by $DP(IOH)$.
When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
Let $DP(OH)$ be  the decision problem 
associated with OH, by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ in unary and $m$  in binary. 
It belongs  to $NP$
after execution of the step I and to $P$ after the step II.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that  $DP(IOH) \in \Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH logically (both becoming tautologies),
and yet the decision problem for the 
new OH for general $m$ 
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH is also a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, such reduction
of a universal statement in $\Pi_3$ to another in $NP$ and then
to $P$ may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{fig:IOHcomplexityintro},
it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.





For mathematical problems which are not universal, theoretical feasibility
can be meaningless. For example, consider 
a trivial  assertion $\forall A, B: A + B = B + A$ where $A$ and $B$ 
are $n\times n$ matrices.
The problem of brute force verification of this assertion 
belongs to $\Pi_1$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality and because 
those alternating quantifiers are intimately related to the 
the alternating quantifiers used to define the conjecturally 
noncollapsing  polynomial-time hierarchy.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 



It may be noticed  that  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, on any approach based on  the flip, 
modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same. 
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.
But in view of the universality of the feasibility barrier, it is 
plausible that this is a universal phenomenon. That is, the same thing
may well happen on any approach towards the $P$ vs. $NP$ problem. 

The  flip can also be formulated
in the theory of pseudorandom generators. For that we  fix 
an explicit $NP$-computable pseudorandom generator 
$g$ that conjecturally fools 
small  circuits (assuming which  $P \not = NP$). We  then express 
this property as an IOH for $g$ and associate a decision problem with it.
But it will be seen that this decision problem lies even higher in
the complexity hierarachy than the IOH for the $P$ vs. $NP$ problem; 
specifically it lies  in $\Pi_3^{BPP}$. Hence
the corresponding flip, which begins at this IOH  and runs towards FOH for $g$ 
through the complexity hierarchy, is harder.
In other words,  this says  that the theory
of pseudorandom generation (derandomization)
is in general  harder than the theory of lower bounds, and hence,
hardness should be proved first  and then transformed into
pseudorandom generation  as per the hardness vs. randomness 
principle \cite{nisan}. This is why we focus on lower bounds in GCT at present.





The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean 
a table specifying a counterexample $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
\ignore{It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counterexample $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.}
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. The same  for a local strongly explicit obstruction.
In this sense, the global flip is stronger than the local flip.
The global   flip also implies   the local  flip if there is a polynomial 
time decoding algorithm, since then 
from a  global  obstruction one can get 
a local  strongly  explicit  obstruction easily. 
The $P\not = NP$ conjecture is not expected to 
stand in the way of this decoding since it simply amounts to spelling out 
what the approach has been doing implicitly anyway.
Hence intuitively the global (strong) flip subsumes the local (strong) flip.
A local strong flip is used in the proof of the $P\not = NC$ result 
without bit operations described below (Section~\ref{swithoutbit}).
But it does not seem 
effective for the harder separation problems in view of the algebraic 
degree barrier discussed there.








The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.



So far we have been assumming that the underlying field of 
computation is the boolean field. But the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems can also be defined over an arbitrary ring or
field, and we are  specifically  interested in 
the rings and fields of characteristic zero such as $Z$, $\Q$ and $\C$. 
Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
By the nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
we mean  the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
But we shall not worry about it here because all the basic ideas of GCT
are  illustrated in the $\#P$ vs. $NC$ problem in characteristic zero.
In this article we  mostly focuss  on characteristic zero     because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. But since the actual $P$ vs. $NP$ problem
is over a finite field (boolean), the flip over a finite field 
is briefly discussed in Section~\ref{sexpli}, with a  detailed discussion 
of the problems that arise in this context  postponed to   GCT11. 

The flip can also be defined for the $P$ vs. $NP$ and $\#P$ vs. $NC$ 
problems over fields of characteristic zero such as $Q$ or $\C$ and for
algebraically closed fields of positive characteristic such as $\bar F_p$, 
the algebraic closure of the finite field $F_p$, $p$ prime.
All  definitions in the flip 
can be lifted to this setting in the obvious way. We  only give
one critical definition as an illustration:

\begin{defn} \label{ddecodeQ}
Assume that the underlying 
field is $Q$. In this case we say that an
obstruction family is {\em easy to decode} 
if there is a decoding algorithm which given the specification of 
an obstruction $O=O_{n,m}$ and a small circuit $C$ over $\Q$ of size $m$ 
(i.e. whose whole description is of bitlength $m$)
produces in $\poly(n,m, \bitlength{O})$ time a counterexample (local
obstruction) $X$ for 
$C$ whose description has  $\poly(n,\bitlength{O})$ bitlength, 
independent of $m$ as long as it is $\le n^{\log n}$ (say). If 
$\bitlength{O}$ is $\poly(n)$ the bitlength of $X$ is then $\poly(n)$
independent of $m$. In other words, smallness
of  obstructions independent of $m$ is to be preserved
in the process of decoding.

Definition over $\bar F_p$ is analogous.
\end{defn} 



The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts are fine and also inevitable as long as 
the spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip is only the most obvious and natural way to cross
the feasibility barrier. 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
will not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques for the reasons 
explained in Section~\ref{scharsym}. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Theorem~\ref{tmathform}) has a nonconstructive   proof
which applies to only very specific  functions (generalized permanents) 
and which 
bypasses  the natural-proof, relativization, and 
algebraic-degree (algebrization) 
barriers simultaneously  in this   setting. 
This gives  concrete evidence that
explicit constructions are  not needed to bypass these local barriers, that
they may be bypassed by nonconstructive proof techniques as well, and that 
there is no reason why the universal feasibility barrier too could not be
crossed by such nonconstructive techniques.



But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may  be  even harder than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof, and in fact
a bit harder.
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative at present.
After all, as pointed out in Section~\ref{sfeasibility}, 
any approach to the $P$ vs. $NP$ problem has 
to meet at least the criteria A, B, and C stated there.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{swithoutbit}) addresses criterion A.
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{smathform})   addresses criterion B.
The main result [GCT6,7,8,11] of GCT  (cf. Sections~\ref{sgct6} and 
\ref{sexpli})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero and also 
over the finite field (the usual case). This
addresses criterion C. 


But, at present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction.


We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.


==> intro1.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ and related problems
\cite{cook,karp,levin,valiant}
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
The main barrier 
towards these problems seems to be  the {\em   feasibility
barrier} described  here.
In essence, it  just asks as per the folklore why the
$P$ vs. $NP$ problem  should not preclude its own proof.
The most obvious and natural strategy to cross this barrier,
called the {\em flip} [GCT6,GCTflip], 
is suggested by the problem itself. It is to 
go for its  {\em explicit proof}. By this we
mean a proof that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify}
in $\poly(n)$ time. In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a conjectural scheme [GCT6,7,8,11] 
for constructing such explicit proofs for the lower bound problems 
under consideration.
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6].
This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 



The  feasiblity   barrier seems to be    the root cause 
of  the  difficulties in the $P$ vs. $NP$ and related problems, and 
not surprisingly,  turns out to be extremely formidable. Indeed, 
all the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. Hence it is elaborated 
here so that the need for  the nonelementary techniques 
that enter into GCT to tackle this barrier becomes clear at a high level.


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present concrete
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the feasibility barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present we do not know any other superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier. Furthermore, 
being purely algebraic and degree independent, it 
is fundamentally different from the known proofs to which
the relativization \cite{solovay} , 
algebraic degree [GCTlocal] and barriers apply, and hence, 
it bypasses these barriers too in this sense.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit}  basically says that 
any low degree or degree based proof technique, such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. As far as we can see, the  recent 
algebrization barrier \cite{aaronson} also says  something similar.
Hence it is not treated  separately in this article.

Though the proof of the mathematical form above thus bypasses the earlier 
known barriers, that is unfortunately not enough, and in retrospect, not
surprising. Because in a sense the main battle 
on the $P$ vs. $NP$ problem seems to begin only after bypassing these
earlier barriers. This battle is basically the task of
crossing the feasibility barrier. The main result of GCT [GCT6,7,8,11]
says that this barrier can be crossed subject to some mathematical positivity 
hypotheses called PH1 and PH4, whose high level description is
given here (cf. Section~\ref{swithoutbit}), and which turn out 
to be intimately  related to the Riemann Hypothesis over finite fields 
\cite{} and related positivity questions in the theory of 
of quantum groups.  The articles GCT6,7,8,11 also propose a plan for proving
these positivity hypotheses. 
Implementation of this plan seems to be a highly nontrivial 
affair far beyond our  expertize, and it is fair 
to say that what has been done in GCT so far is only the easy part
and the hard part (positivity) is yet to begin.  It 
is our hope that this small initial step towards the $P$ vs. $NP$ problem 
will bring  out  formidability of the feasibility barrier, its 
intimate relationship with deep posititivity issues in mathematics, and
perhaps  suggest what needs to be done in future for progress on these 
fundamental  issues in mathematics  and complexity theory.


The mathematical story surrounding positivity is
beyond the scope of this article. 
The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures where this story is discussed
without getting into the philosophical
issues concerning  barriers. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such issues may wish to read that article first. On the 
other hand, the reader who wishes to know the root cause of all the 
difficulties and the need for  nonelementary 
techniques  before getting into any mathematics 
may wish to read this article first. We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The feasibility barrier
is discussed in Section~\ref{sfeasibility}, the flip in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, 
the main result, a conjectural scheme 
for crossing the feasibility barrier via  flip, in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
feasibility barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is grateful to 
Josh Grochow,  Hari Narayanan, Partha Niyogi, and Janos Simon for discussions 
that were helpful in writing this article.




==> intro2.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ 
\cite{cook,karp,levin}, permanent vs. 
determinant \cite{valiant} and related problems
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
The main barrier 
towards these problems seems to be  the {\em   complexity
barrier} described  here.
In essence, it  just asks as per the folklore why the
$P$ vs. $NP$ problem  should not preclude its own proof.
The most obvious and natural strategy to cross this barrier,
called the {\em flip} [GCT6,GCTflip], 
is suggested by the problem itself. It is to 
go for its  {\em explicit proof}. By this we
mean a proof that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify}
in $\poly(n)$ time. In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a conjectural scheme [GCT6,7,8,11] 
for constructing such explicit proofs for the lower bound problems 
under consideration.
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6].
This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 



The  feasibility   barrier seems to be    the root cause 
of  the  difficulties in the $P$ vs. $NP$ and related problems, and 
not surprisingly,  turns out to be extremely formidable. Indeed, 
all the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. Hence it is elaborated 
here so that the need for  the nonelementary techniques 
that enter into GCT to tackle this barrier becomes clear at a high level.


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present concrete
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the feasibility barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present we are not aware of  any other superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier. Furthermore, 
being purely algebraic and degree independent, it 
is fundamentally different from the known proofs to which
the relativization \cite{solovay}, and 
algebraic degree [GCTlocal] barriers apply, and hence, 
it bypasses these barriers too in this sense.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit}  basically says that 
any low degree or degree based proof technique, such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. As far as we can see, the  recent 
algebrization barrier \cite{aaronson} also says   something similar.
Hence it is not treated  separately in this article.

Though the proof of the mathematical form above thus bypasses the earlier 
known barriers, that is unfortunately not enough.
Because in a sense the main battle 
on the $P$ vs. $NP$ problem seems to begin only after bypassing these
earlier barriers. 
In retrospect, this should not be surprising. To see why, let us observe that
these earlier barriers are 
{\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
But  the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal}. By a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.

The  feasibility barrier seems to be  this universal barrier.
It is  simply the task of answering the following question: 

\begin{question} {(bf Feasibiilty barrier)}
Why should a given proof technique be even theoretically feasible, i.e., 
lead to a proof even theoretically?
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers mentioned above. Indeed all these local barriers 
roughly say that the proof techniques akin to
the ones used for proving lower bounds for classical hierarchy theorems,
constant depth circuits \cite{sipser}, $P\not = NC$ result without bit
operations  would not work for the $P$ vs. $NP$ problem
in a sense because the problem  
itself  stands in their way, along with its variants and related  properties,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   very specific 
subareas of mathematics, which is why these  barriers can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions to the proof 
techniques for the lower bounds associated with these barriers, 
why could it not keep on happening again and again?
This does not seem inconceivable since the problem itself says that the 
discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It seems  universal in the sense that Question~\ref{qfeasible}
seems to be the root difficulty of  proving the $P\not = NP$ 
conjecture, and 
every approach may ultimately have to face it in one way or the other.


There is though a fundamental difference between this barrier
and the earlier local barriers. The latter are mathematical barriers 
based on precise mathematical statements. Whereas the feasibility barrier
is based on only  a vague philosophical   question with 
no theorem or precise mathematics behind it. 
Unfortunately, the precisely stated  mathematical local 
barriers do not seem to  capture the root difficulty of the
the $P$ vs. $NP$ problem. Because each local barrier only rules out a 
small area of mathematics. For example, the algebraic degree barrier 
in [GCTlocal] rules out low degree techniques in mathematics.
Though this is a substantial subarea of mathematics, it is still very 
small compared to the whole of mathematics. 
Regardless of how many restricted   areas of mathematics we knock 
out on the basis of such local barriers that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do,
given that the $P$ vs. $NP$ problem is a statement about all of mathematics.
Indeed this is precisely 
what happened after the work on GCT1 and 2 was finished.
It was realized then that though the earlier local barriers were bypassed 
similtaneously therein, the root difficulty of the $P$ vs. $NP$ problem
was yet not addressed.
And Question~\ref{} seems to be that root difficulty.


Fortunately, though this question cannot be formalized,
the most obvious approach to answer it (the flip) can be. 
That is, GCT gives a precise 
mathematical definition of theoretical feasibility, 
justifies why it is a reasonable notion, and 
then formulates precise mathematical hypotheses such that once 
these are proved the approach  is  theoretical feasible
and Question~\ref{} is answered, i.e.,
the feasibility barrier is crossed in this formal mathematical sense.
Specifically, the main result of GCT [GCT6,7,8,11]
says that this barrier can be crossed subject to some mathematical positivity 
hypotheses called PH1 and PH4, whose high level description is
given here (cf. Section~\ref{swithoutbit}), and which turn out 
to be intimately  related to the Riemann Hypothesis over finite fields 
\cite{} and related positivity questions in the theory of 
of quantum groups.  The articles GCT6,7,8,11 also propose a plan for proving
these positivity hypotheses and provide concrete mathematical evidence
and justifications for why they should hold. 
Implementation of this plan seems to be a highly nontrivial 
affair,  and it is fair 
to say that what has been done in GCT so far is only the easy part of this
implementation and the hard part (positivity) is yet to begin.  
Rather the main result of GCT at present  lays out
a precisely formulated mathematical program to cross the feasibilty barrier
based on the most obvious flip strategy
with concrete lower bounds and results in its justification.
And  though there is no theorem or precise mathematics behind Question~\ref{}, 
there is a theorem (Theorem~\ref{}) and precise mathematics in 
the form of PH1 and PH4 behind this particular way of answering it.
The mathematical story surrounding positivity hypotheses (PH1/4) is far 
beyond the scope of this article. 
The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures where this story is discussed and PH1 and 
PH4 are laid out with full mathematical details.


It must be stressed here that there may be other nonobvious ways of
crossing the feasibility barrier, perhaps several. But at present 
we do not have any other program for  answering Question~\ref{} 
which can thus be chalked out and
formalized in precise mathematical terms. 
In fact, this formal chalking out of the program, i.e.
precise formalization  of all mathematical
hypotheses to answer Question~\ref{}, with concrete lower bounds and results
in their justification which meet certain criteria A, B, C stated in 
Section~\ref{}, is a critical part of   
what it means to cross the feasibility barrier. 
This can be done at present only the most obvious way.
Whether there are  similarly formalizable  nonobvious ways is open at present.





\ignore{
It 
is our hope that this small initial step towards the $P$ vs. $NP$ problem 
will bring  out  formidability of the feasibility barrier, its 
intimate relationship with deep posititivity issues in mathematics, and
perhaps  suggest what needs to be done in future for progress on these 
fundamental  issues in mathematics  and complexity theory.}



without getting into the philosophical 
issues concerning  the feasibility barrier. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such philosophical 
issues may wish to read that article first and come back to this
article later. The reader who would rather stick
to mathematics and not worry about philosophy may just  skip this 
article and proceed to \cite{}. But the reader who wishes to
know the root cause of all the 
difficulties and the need for  nonelementary 
techniques  at a philosophical level before getting into any mathematics 
may wish to read this article first. 
We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The feasibility barrier
is discussed in Section~\ref{sfeasibility}, the flip in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, 
the main result, a conjectural scheme 
for crossing the feasibility barrier via  flip, in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
feasibility barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is grateful to 
Josh Grochow,  Hari Narayanan, Partha Niyogi, and Janos Simon for discussions 
that were helpful in writing this article.




==> intro3.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ 
\cite{cook,karp,levin}, permanent vs. 
determinant \cite{valiant} and related problems
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
The main barrier 
towards these problems seems to be  the {\em   feasibility
barrier} described  here.
In essence, it amounts to {\em formally} answering 
the the folklore question: why the
$P$ vs. $NP$ problem  should not preclude its own proof.
The most obvious and natural strategy to cross this barrier,
called the {\em flip} [GCT6,GCTflip], 
is suggested by the problem itself. It is to 
go for its  {\em explicit proof}. By this we
mean a proof that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify}
in $\poly(n)$ time. In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a conjectural scheme [GCT6,7,8,11] 
for constructing such explicit proofs for the lower bound problems 
under consideration.
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6].
This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


\subsection{Feasibility barrier}
Before we turn to the feasibility barrier, let us observe that 
the  earlier known barriers towards the $P$ vs. $NP$ problem 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
and algebraic-degree [GCTlocal] barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as they were in GCT1 and 2
as explained below. (The recent algebrization barrier \cite{aaronson}
seems similar to the algebraic degree barrier in [GCTlocal] 
as explained in Section~\ref{} and hence
is not discussed separately here.) 
Unfortunately, after the work on GCT1 and 2 
was completed, it became clear that  the root 
difficulty of the $P$ vs. $NP$ problem still remains after bypassing
these  local barriers and in a sense the  main battle 
on the $P$ vs. $NP$ problem  begins only after bypassing them.

In retrospect, this should not be surprising. 
We cannot expect local 
barriers to capture the root difficulty of the $P$ vs. $NP$ problem,
because this problem is a {\em universal} statement about all of mathematics.
Namely, if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal}. By a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
A local barrier only  rules out a 
small area of mathematics. For example, the algebraic degree barrier 
in [GCTlocal] rules out low degree techniques in mathematics.
Though this is a substantial subarea of mathematics, it is still 
small compared to the whole of mathematics. 
Regardless of how many restricted   areas of mathematics we knock 
out on the basis of such local barriers, that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do,
given that the $P$ vs. $NP$ problem is a statement about all of mathematics. 
At some point we have to turn our attention to what is to be done
and identify the root universal difficulty of this problem; i.e., 
a universal barrier.

The feasibility barrier seems to be this universal barrier.
Due its universality, it seems quite formidable, as expected.
To describe it,   let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any proof strategy for  the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} 
Why should the proof strategy  be   {\em theoretically  feasible}, i.e., 
lead to a proof even theoretically? 
In other words, in what sense is it fundamentally 
different from the  trivial, infeasible strategy  above
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem stated above.
These local  barriers   roughly say that the proof techniques akin to
the ones used for proving the classical hierachy theorems, lower bounds for 
constant depth circuits \cite{sipser}, and the $P\not = NC$ result 
without bit operatations would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
along with its variants and properties, 
rendering them theoretically infeasible, so to say.
Admittedly, and as already observed,
such proof techniques constitute  only   a very specific 
subarea of mathematics, which is why we are calling these  barriers 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the fundamental question
that has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 


By the {\em  feasibility barrier} we mean the task of answering 
Question~\ref{qfeasible} {\em formally}. The key phrase here is formally.
Because Question~\ref{qfeasible} itself is an informal folklore question
with no theorem or precise mathematics behind it. To answer it formally,
the proof technique  has to first formalize the question, justify why
it is a reasonable formalization,
and then answer the formalized question. In other words,
formalization of the question  is itself a part of the challenge, a part 
of the difficulty.
Indeed, many fundamental questions in science are informal folklore 
questions and the challenge lies in formalizing them.
For example, one well known folklore question of computer science is: 
what is computable? This is informal. 
But the main challenge in computability theory, as we know now, 
was to  formalize this question by giving a precise mathematical meaning to
the phrase {\em computable} and then justify 
why it is a reasonable formalization. Of course, the formalization
of the phrase computable 
that we have today is  one plausible formalization.
We cannot say that it is the only one. But it seems to be  reasonable,
and if there are other reasonable formalizations we do not know them
today.

Similarly Question~\ref{qfeasible} is another folklore 
question of computer science which seems to capture the root 
difficulty of the $P$ vs. $NP$ problem and a part of the 
difficulty is just formalizing this question.

By formalization of  Question~\ref{qfeasible}, we mean:
\begin{enumerate} 
\item[I] Give a mathematically precise formulation of  an  Obstruction
Hypothesis (OH) that is meant to be an alternative to IOH.
Here it must be proved unconditionally that OH implies  IOH.
Furthermore, this obstruction hypothesis should be of the form: 
\[({\bf OH}): \quad  \forall n \forall  m=\poly(n): s(n,m),\] 
where $s(n,m)$ is some formal mathematical statement. 
The statement $s(n,m)$ is supposed to  say that when $m=\poly(n)$ there 
exists  some cause of hardness (which we shall call obstruction) 
because of which IOH holds. We put no restriction on the nature 
of this cuase. The cause could be existence of some
mathematical object in the spirit of the trivial obstruction. In this
case this object can be called an obstruction--an alternative to the
trivial obstruction.
But this is not necessary. The cause could be just some mathematical condition.
As long as it can be completely formalized in the form of a precise 
mathematical statement $s(m,n)$, we do not care. We call OH a
{\em complexity theoretic hypothesis} because it is necessary that
$m$ be small in comparison to $n$ for it to hold.

\item[II] 
State precisely formal {\em mathematical hypotheses} 
$MH1, MH2, \cdots, MH_r$, $r \ge 1$, and 
give a mathematically  precise and formal  definition of the
phrase {\em theoretical feasibility of OH} 
such that if $MH_1,\cdots,MH_r$ hold then OH becomes theoretically 
feasible as per this definition.
Here theoretical feasibility of OH 
is supposed to mean that once $MH_1,\ldots,MH_r$
are proved  the $P\not = NP$ 
conjecture is not expected to stand in the way of proving OH thereafter.
Each mathematical hypothesis should be of the form 
\[ {\bf (MH_i):}  \forall n \forall m t_i(m,n), \] 
for some formal mathematical statements $t_i(m,n)$.
We are calling it mathematical because this is supposed to hold for
all $n$ and $m$, not just when $m=\poly(n)$ or small as in the
case of the complexity theoretic IOH or OH. 

\item [III]
Give reasonable justification for why the $P \not = NP$ conjecture should
not stand in the way of proving $MH_1,\ldots, MH_r$ and
in the way of proving  OH once $MH_1,\ldots, MH_k$ are proved.
\end{enumerate} 

We will say that {\em the feasibility barrier is crossed} and
that OH is {\em theoretically feasible} once $MH_1,\ldots,MH_r$
are proved.
Theoretical feasibility of OH does not automatically guarantee 
{\em practical feasibility}  of proving it. That is, even after OH has
been proved to be theoretically feasible actually proving it may be
a mathematical challenge. 
Thus once Question~\ref{qfeasible} is fully formalized in this fashion  hard 
complexity theory (IOH) is exchanged with hard mathematics 
($MH_1,\ldots,MH_r$). What is gained in this exchange is that 
the $P \not = NP$ conjecture is not expected to stand in the way 
doing this hard mathematics. In this way a fully formalized  mathematical 
program towards  the $P \not = NP$ conjecture is thus laid out.

The next  question: what is meant by reasonable justifications in III? 
Certainly we cannot expect a proof technique to prove that the $P \not = NP$ 
conjecture would not stand in the way of proving $MH_1,\ldots,MH_r$ and
$OH$, because the only way to prove this is to actually prove them 
unconditionally thereby proving the $P \not = NP$ conjecture itself.
But this is a serious issue because regardless of how reasonable 
the justifications of a proof technique may look at the surface 
what guarantee is there that the $P\not = NP$ conjecture or some 
equivalent  or harder complexity theoretic assumptions such as 
existence of one way functions or  pseudo random generators (cf. 
hardness vs. randomness principle \cite{})
are  not lying hidden within $MH_1,\ldots,MH_r$ and OH 
in some hard to recognize forms?  That is, what is the guarantee that
the proof technique is not simply restating 
the problem, or worse,  making it harder, thereby simply evading 
Question~\ref{qfeasible}. 

The only way to provide a reasonable guarantee towards this seems to be
by proving  some unconditional lower bounds  that meet some  hard enough
criteria of nontriviality.
Accordingly, we will say that a proof technique is an {\em approach towards
the $P$ vs. $NP$ problem} if 
it meets the following criteria: 


\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  superpolynomial lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier known  local barriers mentioned before.
%relativization \cite{solovay}, natural-proof \cite{rudich}, and
%algebraic degree [GCTlocal] barriers simultaneously.
Here, in view of the fundamental nature of these barriers,
we agree to take them in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any approach. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}.
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.
\item[C] Concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.



The  feasiblity   barrier seems to be    the root cause 
of  the  difficulties in the $P$ vs. $NP$ and related problems, and 
not surprisingly,  turns out to be extremely formidable. Indeed, 
all the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. Hence it is elaborated 
here so that the need for  the nonelementary techniques 
that enter into GCT to tackle this barrier becomes clear at a high level.


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present concrete
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the feasibility barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present we are not aware of  any other superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier. Furthermore, 
being purely algebraic and degree independent, it 
is fundamentally different from the known proofs to which
the relativization \cite{solovay}, and 
algebraic degree [GCTlocal] barriers apply, and hence, 
it bypasses these barriers too in this sense.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit}  basically says that 
any low degree or degree based proof technique, such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. As far as we can see, the  recent 
algebrization barrier \cite{aaronson} also says   something similar.
Hence it is not treated  separately in this article.

Though the proof of the mathematical form above thus bypasses the earlier 
known barriers, that is unfortunately not enough.
Because in a sense the main battle 
on the $P$ vs. $NP$ problem seems to begin only after bypassing these
earlier barriers. 
In retrospect, this should not be surprising. To see why, let us observe that
these earlier barriers are 
{\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
But  the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal}. By a universal barrier we
mean a barrier that every approach has to cross regardless of what 
areas of mathematics it goes through. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.

The  feasibility barrier seems to be  this universal barrier.
It is  simply the task of answering the following question: 

\begin{question} {(bf Feasibiilty barrier)}
Why should a given proof technique be even theoretically feasible, i.e., 
lead to a proof even theoretically?
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers mentioned above. Indeed all these local barriers 
roughly say that the proof techniques akin to
the ones used for proving lower bounds for classical hierarchy theorems,
constant depth circuits \cite{sipser}, $P\not = NC$ result without bit
operations  would not work for the $P$ vs. $NP$ problem
in a sense because the problem  
itself  stands in their way, along with its variants and related  properties,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   very specific 
subareas of mathematics, which is why these  barriers can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such   local
barriers.
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. 
That is, what happened on the earlier three occasions to the proof 
techniques for the lower bounds associated with these barriers, 
why could it not keep on happening again and again?
This does not seem inconceivable since the problem itself says that the 
discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It seems  universal in the sense that Question~\ref{qfeasible}
seems to be the root difficulty of  proving the $P\not = NP$ 
conjecture, and 
every approach may ultimately have to face it in one way or the other.


There is though a fundamental difference between this barrier
and the earlier local barriers. The latter are mathematical barriers 
based on precise mathematical statements. Whereas the feasibility barrier
is based on only  a vague philosophical   question with 
no theorem or precise mathematics behind it. 
Unfortunately, the precisely stated  mathematical local 
barriers do not seem to  capture the root difficulty of the
the $P$ vs. $NP$ problem. Because each local barrier only rules out a 
small area of mathematics. For example, the algebraic degree barrier 
in [GCTlocal] rules out low degree techniques in mathematics.
Though this is a substantial subarea of mathematics, it is still very 
small compared to the whole of mathematics. 
Regardless of how many restricted   areas of mathematics we knock 
out on the basis of such local barriers that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do,
given that the $P$ vs. $NP$ problem is a statement about all of mathematics.
Indeed this is precisely 
what happened after the work on GCT1 and 2 was finished.
It was realized then that though the earlier local barriers were bypassed 
similtaneously therein, the root difficulty of the $P$ vs. $NP$ problem
was yet not addressed.
And Question~\ref{} seems to be that root difficulty.


Fortunately, though this question cannot be formalized,
the most obvious approach to answer it (the flip) can be. 
That is, GCT gives a precise 
mathematical definition of theoretical feasibility, 
justifies why it is a reasonable notion, and 
then formulates precise mathematical hypotheses such that once 
these are proved the approach  is  theoretical feasible
and Question~\ref{} is answered, i.e.,
the feasibility barrier is crossed in this formal mathematical sense.
Specifically, the main result of GCT [GCT6,7,8,11]
says that this barrier can be crossed subject to some mathematical positivity 
hypotheses called PH1 and PH4, whose high level description is
given here (cf. Section~\ref{swithoutbit}), and which turn out 
to be intimately  related to the Riemann Hypothesis over finite fields 
\cite{} and related positivity questions in the theory of 
of quantum groups.  The articles GCT6,7,8,11 also propose a plan for proving
these positivity hypotheses and provide concrete mathematical evidence
and justifications for why they should hold. 
Implementation of this plan seems to be a highly nontrivial 
affair,  and it is fair 
to say that what has been done in GCT so far is only the easy part of this
implementation and the hard part (positivity) is yet to begin.  
Rather the main result of GCT at present  lays out
a precisely formulated mathematical program to cross the feasibilty barrier
based on the most obvious flip strategy
with concrete lower bounds and results in its justification.
And  though there is no theorem or precise mathematics behind Question~\ref{}, 
there is a theorem (Theorem~\ref{}) and precise mathematics in 
the form of PH1 and PH4 behind this particular way of answering it.
The mathematical story surrounding positivity hypotheses (PH1/4) is far 
beyond the scope of this article. 
The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures where this story is discussed and PH1 and 
PH4 are laid out with full mathematical details.


It must be stressed here that there may be other nonobvious ways of
crossing the feasibility barrier, perhaps several. But at present 
we do not have any other program for  answering Question~\ref{} 
which can thus be chalked out and
formalized in precise mathematical terms. 
In fact, this formal chalking out of the program, i.e.
precise formalization  of all mathematical
hypotheses to answer Question~\ref{}, with concrete lower bounds and results
in their justification which meet certain criteria A, B, C stated in 
Section~\ref{}, is a critical part of   
what it means to cross the feasibility barrier. 
This can be done at present only the most obvious way.
Whether there are  similarly formalizable  nonobvious ways is open at present.





\ignore{
It 
is our hope that this small initial step towards the $P$ vs. $NP$ problem 
will bring  out  formidability of the feasibility barrier, its 
intimate relationship with deep posititivity issues in mathematics, and
perhaps  suggest what needs to be done in future for progress on these 
fundamental  issues in mathematics  and complexity theory.}



without getting into the philosophical 
issues concerning  the feasibility barrier. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such philosophical 
issues may wish to read that article first and come back to this
article later. The reader who would rather stick
to mathematics and not worry about philosophy may just  skip this 
article and proceed to \cite{}. But the reader who wishes to
know the root cause of all the 
difficulties and the need for  nonelementary 
techniques  at a philosophical level before getting into any mathematics 
may wish to read this article first. 
We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The feasibility barrier
is discussed in Section~\ref{sfeasibility}, the flip in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, 
the main result, a conjectural scheme 
for crossing the feasibility barrier via  flip, in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
feasibility barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is grateful to 
Josh Grochow,  Hari Narayanan, Partha Niyogi, and Janos Simon for discussions 
that were helpful in writing this article.




==> intro4.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ 
\cite{cook,edmonds,karp,levin}, permanent vs. 
determinant \cite{valiant} and related problems
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
The main barrier 
towards these problems seems to be  the {\em   complexity
barrier} described  here.
In essence, it amounts to {\em formally} answering 
the folklore question: why should the
$P$ vs. $NP$ problem   not preclude its own proof by standing 
in the way of every approach, and hence, why should the given approach 
be feasible even theoretically? The key phrase here is formally. This means 
the approach has to first formalize the question by giving a precise 
mathematical meaning to the phrase theoretically feasible, 
and then prove that the approach under consideration is theoretically 
feasible as per this definition of theoretical feasibility.
In other words, formalization of the informal folklore question is itself
a nontrivial part of the fundamental conceptual difficulty (barrier) 
in approaching the $P$ vs. $NP$ and related problems. 
The most obvious and natural strategy to cross this barrier,
called the {\em flip} [GCT6,GCTflip], 
is suggested by the problem itself. It is to 
go for its  {\em explicit proof}. By this we
mean a proof that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify}
in $\poly(n)$ time; i.e., the problem of verification of the proof certificates
belongs to $P$ and hence is theoretically feasible.
In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a complete formalization of the above folklore
question and 
a conjectural scheme [GCT6,7,8,11] 
for constructing such explicit proofs for the lower bound problems 
under consideration.
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6].
This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 

\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 



The  complexity    barrier seems to be    the root cause 
of  the  difficulties in the $P$ vs. $NP$ and related problems, and 
not surprisingly,  turns out to be extremely formidable. Indeed, 
all the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. The main result of GCT [GCT6] 
gives a formal mathematical programme to cross this barrier
based on the flip strategy. 



Hence it is elaborated 
here so that the need for  the nonelementary techniques 
that enter into GCT to tackle this barrier becomes clear at a high level.


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present concrete
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the complexity barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present we are not aware of any other superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier as explained 
in  Sections~\ref{} and Section~\ref{}. Furthermore, 
it also bypasses the relativization \cite{solovay} 
and the algebraic degree [GCTlocal] barriers in the sense that 
it works over algebrized forms of computations, does not use 
any low degree technique and hence is fundamentally different 
from the proof techniques to which these barriers apply.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit} basically 
says that any low degree or degree based proof technique, 
such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. 
The  recent algebrization barrier \cite{aaronson} suggests   something similar.
Hence it is not treated  separately in this article.

Though the proof of the mathematical form above thus bypasses the earlier 
known barriers, that is unfortunately not enough, and in retrospect, not
surprising. Because in a sense the main battle 
on the $P$ vs. $NP$ problem seems to begin only after bypassing these
earlier barriers. This battle is basically the task of
crossing the complexity barrier. The main result of GCT [GCT6,7,8,11]
says that this barrier can be crossed subject to some mathematical positivity 
hypotheses called PH1 and PH4, whose high level description is
given here (cf. Section~\ref{swithoutbit}), and which turn out 
to be intimately  related to the Riemann Hypothesis over finite fields 
\cite{} and related positivity questions in the theory of 
of quantum groups.  The articles GCT6,7,8,11 also propose a plan for proving
these positivity hypotheses. 
Implementation of this plan seems to be a highly nontrivial 
affair far beyond our  expertize, and it is fair 
to say that what has been done in GCT so far is only the easy part
and the hard part (positivity) is yet to begin.  It 
is our hope that this small initial step towards the $P$ vs. $NP$ problem 
will bring  out  formidability of the complexity barrier, its 
intimate relationship with deep posititivity issues in mathematics, and
perhaps  suggest what needs to be done in future for progress on these 
fundamental  issues in mathematics  and complexity theory.


The mathematical story surrounding positivity is
beyond the scope of this article. 
The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures where this story is discussed
without getting into the philosophical
issues concerning  barriers. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such issues may wish to read that article first. On the 
other hand, the reader who wishes to know the root cause of all the 
difficulties and the need for  nonelementary 
techniques  before getting into any mathematics 
may wish to read this article first. We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The complexity barrier
is discussed in Section~\ref{scomplexity}, the flip in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, 
the main result, a conjectural scheme 
for crossing the complexity barrier via  flip, in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
complexity barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is deeply grateful to Scott Aaronson, 
Laci Babai, Josh Grochow, Russell Impagliazzo,
Hari Narayanan, Partha Niyogi, Sasha Razborov,  Janos Simon and 
Avi Wigderson for discussions 
that were helpful in writing this article.




==> intro5.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ 
\cite{cook,karp,levin}, permanent vs. 
determinant \cite{valiant} and related problems
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
There seems to be a fundamental root diffculty, 
which we call the {\em complexity
barrier}, that must be overcome by any proof technique that could settle 
these problems.  Not surprisingly this barrier turns out to be 
extremely formidable.
All the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. In fact, even formalization
of this barrier turns out to be quite nonelementary and cannot be done at 
present without algebraic geometry and representation theory.
The main result of GCT [GCT6] provides such a formalization and 
a mathematical programme for crossing the barrier, which has been 
partially implemented in  [GCT6,7,8,11]. But the full implementation of 
this programme seems to be quite a nonelementary affair. 
Hence this paper provides an informal  exposition of the 
complexity barrier to explain why it may  be the root difficulty 
of the $P$ vs. $NP$ problem and what makes it so formidable
so that the need for  the nonelementary techniques 
that enter into GCT to tackle this  barrier becomes clear at a high level.

But before we turn to this barrier, let us first see why the earlier 
known barriers such as the relativization \cite{solovay}, natural-proof
\cite{rudich}, algebraic degree [GCTlocal] and  algebrization \cite{aaronson}
barriers are not only not obstactles to the eventual proof but do not even 
capture the main source of difficulties that needs to be overcome by an 
eventual proof.
This became clear after these barriers were bypassed in the early papers of 
GCT [GCTlocal,GCT1,GCT2]. Let us now explain the concrete lower bounds 
of GCT whose proof techniques bypass these barriers and then 
explain why the root difficulty still remains after bypassing them.



towards these problems seems to be  the {\em   complexity
barrier} described  here. 
Crossing this barrier means   answering {\em formally}
the folklore question: why should the
$P$ vs. $NP$ problem   not preclude its own proof by standing 
in the way of any  approach, and hence, why should the given approach 
be feasible even theoretically? The key phrase here is answring formally. 
This  means:
(1) fix a proof strategy (approach) and
formalize the question by defining precisely and
formally what
theoretically feasibility of this fixed proof strategy
means, and (2) then answer the formalized question by proving that this
proof strategy is indeed theoretically feasible as per this definition.
In other words, formalization of the informal folklore question as in step (1)
is itself a  part of the challenge. If this is carried out, we say that 
the complexity barrier has been formalized in this approach. 
The most obvious and natural abstract strategy to cross this barrier,
called the {\em flip} [GCT6,GCTflip], 
is suggested by the problem itself. It is to 
go for its    {\em explicit proof}. By this we
mean a proof  that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify} 
in $\poly(n)$ time; i.e., the problem of verification 
of the proof certificates belongs to $P$ and hence is theoretically feasible.
In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Abstractly, GCT is any geometric 
approach to the $P$ vs. $NP$ and related problems based on the flip; i.e., 
construction of  explicit proofs.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a complete formalization [GCT6] of the 
complexity barrier (in a specific approach) and a
mathematical programme 
[GCT6,7,8,11] to  cross the formalized complexity  barrier via the flip
for the $P$ vs. $NP$ and related problems. 
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6].
This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 

\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present formal
GCT is one such approach. 
Though this   is the most obvious and natural 
way   to cross the complexity barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
All the mathematical results of GCT together suggest that the flip
should be feasible however counterintuitive it may seem,
and the main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 



The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal],
was proved using a weaker form of the flip 
much before it was formalized in [GCTflip,GCT6]. It says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present this may be the only superpolynomial lower bound 
that is a restricted form of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.

The second lower bound, a mathematical form of the $\#P\not = NC$ 
conjecture in characateristic zero [GCT1,2,6],  is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$. 
It is essentially a direct consequence of GCT1 and 2 in conjunction
with a fundamental result \cite{kempf} of geometric invariant theory that
was used there, though the lower bound was not mentioned there. It can
be found in \cite{GCTexplicit} and [GCT6] with an explicit proof that 
provides a concrete support for the explicit proof conjecture and 
the flip.
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTexplicit,GCT6} is not naturalizable
and hence bypasses the natural proof barrier as explained 
in  Sections~\ref{scharsym} and Section~\ref{smathform}. Furthermore, 
it also bypasses the relativization \cite{solovay} 
and the algebraic degree [GCTlocal] barriers in the sense that 
it works over algebrized forms of computations, does not use 
any low degree technique and hence is fundamentally different 
from the proof techniques to which these barriers apply.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers.

\noindent Remark: The algebraic degree barrier in GCTlocal explained
in Section~\ref{swithoutbit} basically 
says that any low degree or degree based proof technique, 
such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. 
As far as we can see, 
the  recent algebrization barrier \cite{aaronson} also 
suggests   something similar.
Hence it is not treated  separately in this article.

The complementry article \cite{GCTexplicit} gives a mathematical overview 
of GCT based on the IAS lectures 
without getting into the meta
issues concerning  barriers. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such issues may wish to read that article first. On the 
other hand, the reader who wishes to know the root difficulty of the $P$ 
vs. $NP$ and related problems and the need for  nonelementary 
techniques  before getting into any mathematics 
may wish to read this article first. We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The complexity barrier
is discussed in Section~\ref{scomplexity},  high level statement of 
the main result of GCT--a formalization of the 
complexity barrier--in Section~\ref{sGCT}.
Abstract  flip is described in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, elaboration of the 
main result  in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
complexity barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTexplicit}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is deeply grateful to Janos Simon.
This paper arose out of a series of discussions on GCT with 
Janos over the last two years.
The goal was to communicate to him the root difficulty that GCT is trying to 
overcome and its  basic plan for doing so. That root difficulty is the
complexity barrier described here. This paper  basically consists of
answers to his tough and insightful questions. 
The author is also grateful to  Scott Aaronson, 
Laci Babai, Josh Grochow, Russell Impagliazzo,
Hari Narayanan, Partha Niyogi, Sasha Razborov,
Avi Wigderson for helpful discussions.





==> intro6.tex <==
\section{Introduction} \label{sintro}
Geometric complexity
theory (GCT) is an approach to  the $P$ vs. $NP$ 
\cite{cook,karp,levin}, permanent vs. 
determinant \cite{valiant} and related problems
(Figure~\ref{fig:complexityclasses}) suggested 
in a series of  articles we call GCTlocal \cite{GCTlocal},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
There seems to be a fundamental root difficulty, 
which we call the {\em complexity
barrier}, that must be overcome by any proof technique that could settle 
these problems.  Not surprisingly this barrier turns out to be 
extremely formidable.
All the mathematical effort in   GCT in a sense 
goes towards crossing this barrier. In fact, even formalization
of this barrier turns out to be quite nonelementary and cannot be done at 
present without algebraic geometry and representation theory.
The main result of GCT [GCT6] provides such a formalization and 
a mathematical programme for crossing the barrier, which has been 
partially implemented in  [GCT6,7,8,11]--this turns 
out to be quite a nonelementary affair. 
This paper provides an informal  exposition of the 
complexity barrier to explain why it may  be the root difficulty 
of the $P$ vs. $NP$ problem and what makes it so formidable
so that the need for  these nonelementary techniques 
that enter into GCT to tackle this  barrier becomes clear at a high level.



\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


But before we turn to this barrier, let us first see why the earlier 
known barriers such as the relativization \cite{solovay}, natural-proof
\cite{rudich}, algebraic degree [GCTlocal] and  algebrization \cite{aaronson}
barriers do not really capture the 
main source of difficulties that needs to be overcome by an 
eventual proof.
This became clear after these barriers were bypassed in the early papers of 
GCT [GCTlocal,GCT1,GCT2]. Let us now explain the concrete lower bounds 
of GCT whose proof techniques bypass these barriers and then 
explain why the root difficulty still remained after bypassing them.

The first lower bound, the $P\not = NC$ result 
without bit operations [GCTlocal], 
is a special case of the $P\not = NC$ result.
It was proved using a weaker form of GCT's strategy  for crossing
the complexity barrier (discussed below) 
much before it was formalized in [GCTflip,GCT6]. 
The result  says that
the maxflow problem cannot be solved  in the PRAM model without bit operations
in polylogarithmic time using polynomially many processors.
At present this may be the only superpolynomial lower bound 
that is a special case of any of the fundamental separation problems in
Figure~\ref{fig:complexityclasses}
and  holds unconditionally in a natural and realistic 
model of computation that is  heavily used  in practice.
Furthermore, as explained in Section~\ref{swithoutbit}, 
its  proof technique is fundamentally different from 
the proof techniques to which the relativization 
and natural-proof barriers apply. 

But that is not enough. Because GCTlocal  pointed out 
a third barrier in complexity theory, which we shall call 
the {\em algebraic degree barrier}, but which was not called a barrier 
there for the reasons explained below. 
This basically says that any low degree or degree based proof technique, 
such as the one there,
which associates with a computation algebraic objects 
and then reasons solely on the basis of the degrees of those 
objects will not work for unrestricted 
fundamental separation problems. 
As far as we can see, 
the  recent algebrization barrier \cite{aaronson} also 
suggests   something similar \footnote{But on the basis of lower bounds 
which may not be as closely related with the fundamental separation
problems in Figure~\ref{fig:complexityclasses} as 
the $P\not = NC$ result without bit operations in GCTlocal.}.
Hence it is not treated  separately in this article.



GCTlocal also suggested 
an idea for crossing the algebraic degree barrier:
namely, associate with complexity 
classes algebraic varieties with group actions that capture the symmetries
of computation and then reason
on the basis of the deeper representation theoretic 
structure of these varieties rather than just their degrees.


This led to the investigation in GCT1 and 2, which suggested 
an approach to the fundamental lower bound problems via algebraic geometry
and representation theory. The results in GCT1 and 2 in conjunction
with a fundamental result in geometric invariant theory \cite{kempf} 
that was used there lead to the 
the second lower bound of GCT, which however was not stated there--it 
would appear in GCT6. We call it 
a mathematical form of the $\#P\not = NC$ 
conjecture in characteristic zero [GCT1,2,6]. It 
is a strengthened form of a
weaker implication of the permanent vs. determinant problem \cite{valiant}
over $\C$ or $\Q$.  
It says that no generalized permanent of $k$ $n\times n$ variable 
matrices $X_1,\ldots, X_k$ can be expressed as a polynomial in the traces 
of $\bar X_i^j$, $j \ge 0$, where $\bar X_i=B_i X_i C_i$ for 
any complex possibly singular 
$n\times n$ matrices $B_i$ and $C_i$. Here by a generalized
permanent we mean any polynomial with exactly the same symmetries as 
the permanent. 
A  {\em weak form} of this lower bound for $k=1$ and the usual permanent
was earlier  stated in
the IAS lectures in February 2009 \cite{IAS}.
The article \cite{boris} showed that
it is too weak by giving a direct elementary proof which    is 
naturalizable; i.e., which does not cross the natural proof barrier 
\cite{rudich}. The proof of the quadratic lower bound for the 
permanent \cite{ressayre} is also naturalizable. In contrast,
it may be   conjectured 
that  the  mathematical form of the 
$\#P \not = NC$ conjecture cannot be proved by any 
naturalizable proof technique.
Its   proof in \cite{GCTriemann,GCT6} is not naturalizable
and hence bypasses the natural proof barrier as explained 
in  Sections~\ref{scharsym} and Section~\ref{smathform}. Furthermore, 
it also bypasses the relativization \cite{solovay} 
and the algebraic degree [GCTlocal] barriers in the sense that 
it works over algebrized forms of computations, does not use 
any low degree technique and hence is fundamentally different 
from the proof techniques to which these barriers apply.
In contrast, it seems  \cite{aaronson} that the proof techniques
of the earlier known lower bounds in complexity theory
may not bypass all  these earlier well studied barriers simultaneously.


Unfortunately after  GCT1 and 2, wherein the earlier known 
barriers were thus bypassed,
it became clear that  the root 
difficulty of the $P$ vs. $NP$ problem still remained after bypassing
these barriers  and the  main battle 
on the $P$ vs. $NP$ problem  really begins only after bypassing them.

In retrospect, this should not be surprising. 
The relativization,  natural-proof,
and algebraic-degree  barriers cannot be  expected to 
capture the root difficulty of the $P$ vs. $NP$ problem. 

To see why, 
let us begin with the algebraic degree barrier in [GCTlocal].
It applies to the low degree techniques of the kind used in that
paper.  All these techniques are in one way or
the other related to the fundamental Bezout's theorem in algebraic geometry
and the notion of a degree of a polynomial
(we also include the low degree techniques used in other areas of 
complexity theory in this category). Though this is a nontrivial area of
mathematics, it is still very small compared to the whole of mathematics.
Hence, we can say that this  barrier is {\em local} 
in the sense that it applies to a very 
restricted class of techniques in mathematics. 
If a proof technique does not belong to this class, the barrier 
is simply bypassed, i.e., is not applicable. 
In this sense, it  is not really a barrier--if by a barrier
we mean a conceptual obstacle 
that any eventual proof of the $P\not = NP$ conjecture would need to 
overcome regardless of which areas of mathematics it goes through--but 
rather a trap  that a proof technique has to avoid.
This is why it  was not  called a barrier in GCTlocal.

We can also say 
that the algebraic degree  barrier is primarily {\em mathematical} 
in the sense that low degree 
is a purely a mathematical notion, there is no complexity theory in it,
and though it  is very useful in complexity theory, this barrier is really a 
statement about the restricted nature   of these mathematical 
techniques rather than about the complexity theoretic difficulty 
of  the $P$ vs. $NP$ problem. 


In a similar way, we may say that the relativization and natural proof 
barriers are also local and mathematical.  Mathematical  because the natural 
proof barrier is generally regarded as applying to proof techniques that 
work for most functions and most is a mathematical notion, 
so also the notion of relativization.


Now we can explain why  local mathematical 
barriers cannot be expected to
capture the root difficulty of the $P$ vs. $NP$ problem.
Because this problem is a {\em universal complexity-theoretic} 
statement about all of mathematics.
Namely, if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal complexity theoretic 
nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal} and {\em complexity theoretic},
where by a universal barrier we
mean a barrier that every approach has to cross regardless of which
areas of mathematics it goes through. 
In other words, a local barrier is like 
a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
A local barrier only  rules out a 
restricted  area of mathematics. 
Regardless of how many restricted   areas of mathematics we rule 
out in this way, that still rules  out only a 
small subarea of mathematics, tells us a few things that we should not do,
but gives us  essentially no idea about what to do
given that the $P$ vs. $NP$ problem is a statement about all of mathematics. 
At some point we have to turn our attention from what is not to be done
to  what is to be done
and identify the root universal and complexity theoretic 
difficulty of this problem; i.e., 
a universal complexity theoretic barrier.

The complexity  barrier described in this article 
seems to be this universal complexity theoretic barrier.
Crossing this barrier basically means   answering {\em formally}
the folklore question: why should the
$P$ vs. $NP$ problem   not preclude its own proof by standing 
in the way of any  approach, and hence, why should any given approach 
be feasible even theoretically? The key phrase here is answering formally. 
This  means:
(1) fix an appropriate  proof strategy (approach) and
formalize the question by defining precisely and
formally what
theoretically feasibility of this fixed proof strategy
means, and (2) then answer the formalized question by proving that this
proof strategy is indeed theoretically feasible as per this definition.
In other words, formalization of the informal folklore question as in step (1)
is itself a  part of the challenge. If this is carried out, we say that 
the complexity barrier has been formalized in this approach. 
The $P\not = NP$ conjecture seems so severe that for most proof strategies
it may not  even be possible to carry out step (1). That is, formal
definition theoretical feasibility may be possible 
for only some exceptional proof strategies. This is why just 
formalization of the complexity  barrier seems  to be such a challenge.


The most obvious and natural abstract strategy to cross the complexity 
barrier, called the {\em flip} [GCT6,GCTflip], 
is suggested by the $P$ vs. $NP$ problem itself. It is to 
go for its    {\em explicit proof}. By this we
mean a proof  that shows existence of  proof certificates
of hardness for an NP-complete function $f(X)=f(x_1,\ldots,x_n)$ 
that are {\em short} of $\poly(n)$ size and  {\em easy to verify} 
in $\poly(n)$ time; i.e., the problem of verification 
of the proof certificates belongs to $P$ and hence is theoretically feasible.
In other words, the flip seeks proof certificates 
for nonmembership of $f(X)$ in $P$ akin to those for its membership in $NP$.
Abstractly, GCT is any geometric 
approach to the $P$ vs. $NP$ and related problems based on the flip; i.e., 
on construction of  explicit proofs.
Such explicit 
proofs based on the specific 
proof certificates  defined in GCT1,2 and 6, called 
{\em geometric  obstructions}, 
exist as per the {\em explicit proof conjecture} [GCT6].
The main result of  GCT  is a complete formalization [GCT6] of the 
complexity barrier (in this specific approach) and a
mathematical programme 
[GCT6,7,8,11] to  cross the formalized complexity  barrier via the flip
for the $P$ vs. $NP$ and related problems. 
It is supported by 
two concrete lower bounds of GCT based on  the flip and its local form: namely,
{\em the  $P \not = NC$ result without bit operations} [GCTlocal] 
and {\em a mathematical  form of the $\#P\not = NC$ conjecture in 
characteristic zero} [GCT1,2,6] discussed above.

This article  gives a complexity theoretic 
overview  of GCT outlining these developments. 

This also allows us to  place  GCT in the landscape of all possible 
approaches to cross this main barrier in complexity theory.
For that, we define  GCT abstractly 
as any geometric approach based on the flip 
towards the $P$ vs. $NP$ and related 
problems, where geometric means based on
the  symmetries of a judiciously chosen $f(X)$. The present formal
GCT is one such approach. 
Though the flip   is the most obvious and natural 
way   to cross the complexity barrier, 
paradoxically it also  turns out to be  very counterintuitive and hard to
believe at the same time.
The formalization of the complexity barrier mentioned above 
basically provides a concrete mathematical program to implement the flip and 
says that the flip
should be feasible however counterintuitive it may seem.
The main goal of this article is to justify this from the complexity
theoretic perspective.
Two concrete lower bounds of GCT mentioned above play a crucial role in
this justification. 


The complementary article \cite{GCTriemann} gives a mathematical overview 
of GCT based on the IAS lectures 
without getting into the meta
issues concerning  barriers. The reader who wishes to 
get a concrete mathematical picture of the approach 
before worrying about such issues may wish to read that article first. On the 
other hand, the reader who wishes to know the root difficulty of the $P$ 
vs. $NP$ and related problems and the need for  nonelementary 
techniques  before getting into any mathematics 
may wish to read this article first. We leave the choice to the readers.
See also the recent article \cite{landsberg} for 
an external mathematical  review of GCT1 and 2.


The rest of this article is organized as follows. The complexity barrier
is discussed in Section~\ref{scomplexity},  high level statement of 
the main result of GCT--a formalization of the 
complexity barrier--in Section~\ref{sGCT}.
Abstract  flip is described in Section~\ref{sflip},
the first lower bound in Section~\ref{swithoutbit},
the meaning of the phrase geometric in Section~\ref{scharsym},
the second lower bound  in Section~\ref{smathform}, elaboration of the 
main result  in 
Sections~\ref{sgct6} and \ref{sexpli},  and finally the question--is the
complexity barrier really so formidable?--in Section~\ref{sformidable}. 
Sections~\ref{scharsym}-\ref{sexpli} constitute
an extended abstract of Chapter 1 in \cite{GCTriemann}.



\noindent {\em Remark:} 
Natural in GCT means explicit unlike in  \cite{rudich} where it means
probabilistic. The meaning should be clear from the context. 



\noindent {Acknowledgements:} The author is deeply grateful to Janos Simon
without whom this paper would not exist.
The paper grew out of a series of discussions on GCT with 
him over the last year.
The goal was to communicate to him the root difficulty that GCT is trying to 
overcome and its  basic plan for doing so. That root difficulty is the
complexity barrier described here. This paper  basically consists of
answers to his tough and insightful questions. 
The author is also grateful to  Scott Aaronson, 
Laci Babai, Josh Grochow, Russell Impagliazzo,
Hari Narayanan, Partha Niyogi, Sasha Razborov, and
Avi Wigderson for helpful discussions.





==> lecture1.tex <==
\section*{Introduction}

This article   gives a mathematical  overview of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.



We  focus here on only the nonuniform versions of the above problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$--what this means will be explained below.
The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 


The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTlocal. We shall refer
to it as the $P\not = NC$ result without bit operations.
It says that the max flow problem cannot be solved in the 
PRAM model without bit operations in $\polylog(N)$ time using 
$\poly(N)$ processors where $N$ is the bitlength of the input.
This  may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weaker (local)
form of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented %(cf. Figure~\ref{fig:matrices})
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
% quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we 
concentrate  on only the former problem,
since this illustrates all the basic ideas. 



The complementary article \cite{GCTexplicit} gives a complexity-theoretic
overview of GCT. It describes   the main complexity theoretic
barrier towards these problems 
called the {\em feasibility barrier} and the defining
strategy of GCT for crossing it called the {\em flip} [GCT6,GCTflip]: 
which is to go 
for {\em explicit proofs}. By an explicit proof 
we mean a proof that provides proof certificates of hardness  for the 
hard function under consideration that are short (of polynomial size) 
and easy to verify (in polynomial time). This barrier turns out to be
extremely formidable and is the root cause of all difficulties 
in these problems. Nonelementary techniques are brought into GCT precisely
to cross this barrier. It is not discussed in these lectures. 
The goal here is to describe the basic ideas of GCT at a concrete mathematical
level without getting into such meta issues. But the readers who wish
to know the need for the nonelementary techniques in GCT before getting
into any mathematics   may wish to read that
article before this one. On the other hand, the readers who would rather avoid 
meta issues before getting a concrete mathematical
picture  may wish to read this article first. We  leave the
 choice to the readers.

The original IAS lectures stated a lower bound called a 
{\em weak form  of the $\#P$ vs. $NC$
problem}. This is a special case of a far more general result of 
GCT, which may be considered its second unconditional lower bound result, and 
which we shall call {\em a mathematical form of the $\#P \not = NC$ 
conjecture}.  It is essentially a direct consequence of the general 
results in GCT1 and 2 in conjunction with a fundamental result \cite{kempf} 
of geometric invariant theory \cite{mumford} that was used there, though
the lower bound was not stated there. It would appear in revised GCT6
with an explicit proof which needs an additional result \cite{ariki} 
in representation theory.
The article \cite{boris} showed that the weak form  stated in the IAS 
lectures is  too weak because it has a direct elementary proof 
which is naturalizable, i.e., which  does not cross the natural proof barrier
\cite{rudich}. Hence in this article it has been replaced with the 
mathematical form of the $\#P\not = NC$ conjecture mentioned above; cf. 
Section~\ref{sweaklec1}. 
We cannot prove this  mathematical form by such elementary naturalizable 
proof techniques for the reasons given in Sections~\ref{sweaklec1} and 
\ref{sweak}. 





The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short mathematical 
overview of the basic plan of GCT,  
which is elaborated in the next two lectures. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality,
to the authors of \cite{boris} for pointing out weakness of the 
lower bound stated during the lectures, and to Shrawan Kumar for
bringing the reference \cite{ariki} to his attention and 
helpful discussions.




\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$,

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$  with obvious constraints 
on the product of the diagonal entries of $A$ and $B$ when they are diagonal.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property (P)
henceforth.


A basic idea [GCT1]  is to a get a handle on 
the permanent vs. determinant problem 
by exploiting exceptional nature of these polynomials--i.e.,
their characteristic properties (P) and  (D).
Representation theory and 
algebraic geometry enter inevitably into  the study of these properties,
because
to understand symmetries representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
To show how these characteristic properties can be exploited, 
we now state one application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below)--before
going any further.

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices $X_1,\ldots,X_k$  
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U_i$ and $V_i$, $i \le k$, 
\[ p(U_1 X_1 V_1,\ldots, U_k X_k V_k)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U_i X V_i)=\perm (X) \quad \forall i.\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U_i$ and $V_i$ above have to be permutation
or diagonal matrices (with obvious constraints on the product of their 
diagonal entries), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. 
At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
For general  $n$ and $k$, almost any polynomial 
in $\perm(X_i)$'s, $i \le k$, is  a generalized permanent, but 
there are many others besides these.
For general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


Now we have the following:

\begin{obs}[Implication of the nonuniform $\#P \not = NC$ conjecture]

Assuming the nonuniform $\#P \not = NC$ conjecture in characteristic zero,
no $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree can be expressed as an $NC$-computable polynomial function of the 
traces of  $\bar X_i^j$, $1 \le i \le k$, $j=\poly(n,k)$, where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{obs}
(Here $X_i^j$ are  clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this implication is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture (in characteristic 
zero),
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of  $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This, i.e., the 
general $\#P \not = NC$ conjecture in characteristic zero, 
cannot be proved unconditionally at present.
But the next case of this implication,  $n>1$ and $k$ arbitrary, can be:

\vfil \eject 
\begin{theorem}[GCT1,2,6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
$\bar X_i^j$, $1 \le i \le k$, $j \ge 0$,  where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{theorem}

When  $k=1$ and $p(X_1)$ is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces,
(though for trivial reasons
we can assume without loss of generality that 
the polynomial in the traces is computable in $2^{\poly(n,k,d)}$ time, 
where $d$ is  the degree of $p$). 
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a  polynomial  whose Galois group is not
solvable cannot be solved by any number of
radical operations, without any restriction on the number of such
operations (though again there is a trivial  upper bound on the number of
such operations needed if the polynomial is solvable by radicals). 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completeness property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the mathematical property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is complete in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
similar completeness,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such completeness
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show [GCT6] that most functions do not
have property (P) when $n>1$ and $k$ is arbitrary.
\ignore{It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultaneously.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.}



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{kempf,mumford} and
the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with the  nontrivial underlying difficulties in
the problem explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the   mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general (i.e. complexity theoretic) permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it, and furthermore the groups of
symmetries of the permanent and the determinant, which we shall
refer to as $G_{perm}$ and $G_{det}$,  are embedded in this group $G$
as its subgroups in some way. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length  at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k \le l$,
where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.

A strong obstruction $O_n$ is a Weyl module $V_\lambda(G)$ 
that occurs as a subrepresentation in $R_{\#P}(n,m)_d^*$ but 
does not contain a nonzero 
invariant (fix point) of the subgroup $G_{det} \subset G$ of the symmetries 
of the determinant.
It can be shown \cite{GCT2} that a strong obstruction
is an obstruction in the above sense.
\end{defn}

Here by  an invariant we mean a point in $V_{\lambda}(G)$ 
which is fixed (does not move) with respect to the action of the subgroup
$G_{det} \subset G$.

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This   follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of a (strong) 
obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}.
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists a (strong)  obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a 
family $\{O_n=V_\lambda(G)\}$ of (strong) obstructions, with a different $G$
than in the general complexity theoretic case.
Furthermore this family  is {\em strongly explicit} in the sense  that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\ignore{\noindent {\em Remark:}
There is also a second nonconstructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same phenomenon
in the general case in what follows.
}

\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation.
Let $G_{\lambda,m}(k)$ denote the multiplicity of the trivial one dimensional
representation (invariant) of $G_{det} \subset G$ in 
$V_{k\lambda}(G)$. In other words, $G_{\lambda,m}(k)$ is the dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$.
These are statistical functions
associated with the class variety $X_{\#P}(n,m)$ 
and the subgroup embedding  $G_{det} \hookrightarrow  G$.
In the first case,  the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ and in the second 
case the dimension of the subspace of invariants of the symmetries of the
determinant in $V_{k \lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$.  It is known to be  an asymptotic
 quasi-polynomial. We shall call it the asymptotic 
Ehrhart quasi-polynomial  of the parametrized polytope $P(k)$. 
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 
From the context it should be clear whether $P$ is a usual nonparametrized 
polytope or a parametrized polytope.









\begin{theorem} (GCT6) \label{tquasi}

\noindent (a) The  function $G_{\lambda,m}(k)$ is a quasi-polynomial.


\noindent (b) The function $F_{\lambda,n,m}(k)$ is 
an asymptotic quasi polynomial.

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 


The proof of Theorem~\ref{tquasi} is based on:
\begin{enumerate} 
\item The classical work of Hilbert in invariant theory, 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.

\noindent {\em Remark:} 
The original IAS lecture   stated a conditional form of (b),
which said that $F_{\lambda,n,m}(k)$ is a quasi-polynomial if the
singularities of the class variety $X_{\#P}(n,m)$ are rational and normal 
(in some algebro-geometric sense). 
Recently, Shrawan Kumar  \cite{shrawan}  has shown that 
the singularities of $X_{\#P}(n,m)$ are not normal if $m>n$. This means 
$F_{\lambda,n,m}(k)$ need not be  a quasi-polynomial and 
asymptotic quasi-polynomiality as in  (b) is all that we can expect.
This is fine 
as long as the singularities of $X_{\#P}(n,m)$ are not too bad 
in the sense described in Remark 3  after Hypothesis~\ref{hph1} below.

The following hypothesis 
says that $G_{\lambda,m}(k)$  can be realized as the Ehrhart quasi-polynomial
of a polytope, and 
$F_{\lambda,n,m}(k)$ 
can be realized as the asymptotic Ehrhart quasi-polynomial 
of a parametrized  polytope.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) For every $m$, there exists a (usual nonparametrized) 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
It is assumed here that there exists for $Q_{\lambda,m}$ a 
specification of the form (\ref{eqpara}) with $k=1$ and $c=0$  
where $A$ is independent of $\lambda$, and $b$ is 
is a  piecewise homogeneous linear function of $\lambda$.




Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 



If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in mathematics are quasi-polynomials 
or asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold 
because of the exceptional nature of the determinant and the permanent. 
For concrete  mathematical evidence and justification, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of (strong) obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous OH that arises in the context of the mathematical form
of the $\#P\not = NC$ conjecture can be  proven unconditionally.

We call  $\lambda$ a {\em polyhedral  obstruction}
(or rather, polyhedral  obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
a (strong)  obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point.
Henceforth, whenever we say obstruction, we actually mean polyhedral
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
parametrized polytope $P_{\lambda,n,m}=P_{\lambda,n,m}(k)$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
(nonparametrized) polytope $Q_{\lambda,m}$  satisfying   PH (b)
with the polynomial bounds that 
depend on $n$ and the bitlength of $\lambda$, but not on $m$.
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurrence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$), and the absence 
of $m$ in the polynomial bounds in (b), which means they again are 
$\poly(n)$ when  $\bitlength{\lambda}=\poly(n)$).
The reasons for this will be explained in Lecture 3 
(cf. remarks before Hypothesis~\ref{hph1tilde} and 
after Hypothesis~\ref{hph1restatement}). 



\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,m}(k)$ belong to the complexity class $\#P$. 

\noindent {\em Remark 3:} PH1 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$, i.e.,  the bitlength
of the deviation is polynomial.  As remarked after Theorem~\ref{tquasi},
this deviation would have been zero, i.e., $F_{\lambda,n,m}(k)$ would
have been a (strict) quasi-polynomial, if the singularities of the class
variety $X_{\#P}(n,m)$ were all normal and rational, which, as we know now,
is not the case \cite{shrawan}. So small deviation from quasi-polynomiality
implied by PH1 
basically means that the deviation from rationality and normality of
the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
This is the basic minimum that is required by PH1.


Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (polyhedral) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid polyhedral obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of polyhedral 
obstructions is equivalent to saying
that the problem of deciding existence of polyhedral obstructions
for given $n$ in unary and $m$ in binary 
belongs to $NP$--we shall refer to this decision problem as $DP(OH)$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. \cite{GCTexplicit} and GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geometry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant and $C$ ranges over 
circuits of size $m=\poly(n)$.
For given $X$ and $C$, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to  $P^{\#P}$.  Let $DP(IOH)$ denote the decision problem 
of deciding for given $n$ and $m$ (in unary) whether 
(\ref{eqioh}) holds with $C$ ranging over circuits of size $m$.
Since there are two alternating layers of quantifiers in (\ref{eqioh}), it
belongs to $\Pi_2^{\#P}$, which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence (\ref{eqioh})
is expected to  be verifiable for small  $m=\poly(n)$ 
in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi_2^{\#P}$}}
\psfrag{sigma1p}{$\Sigma_1^{\#P}$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$DP(OH) \in NP$}
\psfrag{inP}{$DP(POH) \in P$}
\psfrag{insigma2p}{$DP(IOH) \in \Pi_2^{\#P}$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  decision problem associated 
with the obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each small $C$
as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, $DP(OH)$, the decision 
problem  of deciding if a new polyhedral obstruction exists, belongs 
to $NP$ (in a stronger sense assuming that $n$ is given in unary but
$m$ is given in binary
instead of unary) as we have already observed. Thus, assuming PH1, we have 
transformed the original decision problem for trivial obstructions
$DP(IOH) \in \Pi_2^{\#P}$ to the  decision problem for the  new polyhedral 
obstructions $DP(OH) \in NP$,
in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new polyhedral obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
complexity of the decision problem associated with the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH$, whose associated decision problem  $DP(OH)$ belongs to $NP$,
can be transformed 
to POH (Positivity Obstruction Hypothesis),  whose associated
decision problem $DP(POH) \in P$; i.e.,  whether a new obstruction 
exists for given $n$ in unary and $m$ in binary 
can then be decided in polynomial time,
and if so, it can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified and constructed in
$O(1)$ time--i.e., the associated decision problem $DP(FOH)$ 
is $O(1)$-time solvable. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the decision problem associated with 
the  obstruction hypothesis until 
the obstruction hypothesis  is finally 
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{m}= \{ \lambda: Q_{\lambda,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

The following is a consequence of a fundamental result \cite{brion} in 
geometric invariant theory \cite{mumford}.
\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{m}$ are convex polytopes in $\C^k$.
\end{theorem} 


Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurences of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$, considered as a 
$G$-module by letting 
$G$ act on each factor of the tensor product independently. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
GCT does suggest  that proving OH/POH  should be feasible 
``in theory'', i.e., {\em theoretically feasible},  assuming PH1/4,
since then DP(OH)/DP(POH)  belong to NP/P and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be theoretically feasible. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 







\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explicit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility  barrier} \cite{GCTexplicit,GCTflip}
which is universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and  the natural way may well be 
among the most effective. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}


%\input{lecture1_maintext}


==> nonuniform1.tex <==
\section{The  feasibility barrier} \label{sfeasibility} 
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quite formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it is difficult to 
formalize it fully.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time of the obvious algorithm 
to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}--it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
say that  IOH  is {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible, i.e., lead to a proof
even theoretically? In other words, in what sense is it fundamentally 
different from the  trivial, infeasible approach above
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental local
barriers towards this problem 
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier   roughly says that the proof techniques akin to
the ones used for proving lower bounds for 
constant depth circuits \cite{sipser},
would not work for the $P$ vs. $NP$ problem
in a sense because the problem  itself  stands in their way,
rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only   a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a  local
barrier (for the reasons explained in more detail in Sections~\ref{sflip}
and \ref{scharsym}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify the  meaning of answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggests such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,monotone,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
for every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{agarwal} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
decoding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or for that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results
\cite{sipser,monotone,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonuniform obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments like the ones  based on uniform 
objects such as  conjectural pseudo random generators 
which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there seems to be  a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  superpolynomial lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier known  local barriers mentioned before.
%relativization \cite{solovay}, natural-proof \cite{rudich}, and
%algebraic degree [GCTlocal] barriers simultaneously.
Here, in view of the fundamental nature of these barriers,
we agree to take them in  spirit rather than letter. 
Because formally  the natural proof barrier \cite{rudich}  is
defined only for the unrestricted $P$ vs. $NP$ problem and
is crossed only after proving $P\not = NP$, which is of no help 
in evaluating any approach. Fortunately, this and other local barriers
make sense in spirit in  any reasonable restricted setting. 
Thus we will say that 
a proof technique bypasses the natural proof barrier \cite{rudich} 
if it does not
apply to most functions, with the meaning of most like in \cite{rudich}.
We will say that it bypasses the relativization barrier \cite{solovay} 
if it is algebraic, 
i.e., works on algebrized forms of computations  in the spirit 
of the $IP=PSPACE$ result.
We will say that it bypasses the algebraic degree barrier [GCTlocal] if it 
does not use low degree techniques.
\item[C] Concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.




==> nonuniform2.tex <==
\section{Abstract nonuniform approaches} \label{snonuniform} 
Let us get back to  the lower bound problem in the begining of 
Section~\ref{scomplexity}. The problem is to  show
nonexistence of small circuits  for computing $f(X)$ as there.
Now we formulate  an abstract  nonuniform approach to  cross the
complexity  barrier in the context of this problem. 


Intuitively, 
by  nonuniform we mean unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggests such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
By  a nonuniform approach to this problem, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,monotone,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
for every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{agarwal} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
decoding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or for that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the complexity barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results
\cite{sipser,monotone,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonuniform obstructions
which lie on the way from the trivial to the final obstruction.


To formalize Question~\ref{qfeasible}
a nonuniform approach has to carry out steps I,II and III in 
Section~\ref{scomplexity}. 


\noindent [I]:
 Come up with a new formal notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments like the ones  based on uniform 
objects such as  conjectural pseudo random generators 
which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
define formally  the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there seems to be  a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the complexity barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:







==> text.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
The main barrier 
towards these problems is   the {\em   feasibility
barrier} described here (Section~\ref{})   and  the basic strategy
of GCT for crossing this barrier is called the flip [GCT6,GCTflip].
The main result of  GCT [GCT6,7,8,GCT11] is conjectural scheme for
the implementation of the flip.
Its  final goal
is to prove the {\em explicit proof conjecture} (Section~\ref{}),
which says that
the $P\not = NP$ conjecture has an {\em extremely explicit proof}, by 
which we mean a proof  
that shows existence of  proof certificates
of hardness for the $NP$-complete function under consideration 
that are short (of polynomial size), easy to verify, discover and decode 
(in polynomial time); cf. Section~\ref{}.
This  is supported by 
two concrete lower bounds of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] (Section~\ref{})
and a mathematical  form of the $\#P\not = NC$ conjecture in characteristic
zero (Section~\ref{}).
This introduction gives a short overview  of GCT outlining these developments.


The original lectures did not describe the 
the  feasiblity   barrier  and the explicit proof conjecture.
But all the mathematical effort in   GCT as described in these lectures 
goes towards crossing this barrier and  producing such an explicit proof.
Hence, we describe  them   here so that the root cause of 
all difficulties encountered in GCT and the need for nonelementary techniques
to cross this formidable barrier
becomes clear  at a high level before we get into any mathematics. 


The original IAS lectures did not state the first lower bound and
only stated   a special case of the second 
lower bound called  the weak form of the $\#P$ vs.
$NC$ problem. The article \cite{boris} showed that this weak form 
is too weak; i.e., it can be proved    by an elementary  technique
that  cannot cross the natural-proof barrier \cite{rudich}.
We cannot prove the full mathematical form by such
techniques for the reasons given in Sections~\ref{}.
Its  proof here 
is based on the results of GCT1,2 and geometric invariant theory 
\cite{mumford}. It crosses the relativization \cite{solovay}, 
natural proof \cite{rudich}, 
algebraic degree \cite{GCTlocal}, and algebrization \cite{aaronson} 
barriers simultaneously  and is (strongly) explicit. 
These two lower bound results  provide a concrete support  for 
the GCT approach.









\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 




\section{The  feasibility barrier} \label{sfeasibility}
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggest such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,razborov,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
of every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $\C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
deconding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or far that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results 
\cite{sipser,razborov,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonunifrom obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments, like the ones  based on uniform 
objects which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier 
relativization \cite{solovay}, natural-(probabilistic)-proof {rudich}, 
algebraic degree [GCTlocal], and 
algebrization \cite{aaronson} barriers simultaneously.
Here, in view of the fundamental nature of these barriers, we agree to
take them in spirit rather than letter. Because, though these barriers 
are defined only for the unrestricted $P$ vs. $NP$ problem, they make 
sense in  any reasonable restricted setting. Thus we assume that
the relativization barrier   applies to any technique that views 
computation abstractly without algebrizing it, algebraic degree or
algebrization barrier to any low degree technique,
and the natural proof barrier to any technique that works 
for most functions with the meaning of most as in \cite{rudich}. 
\item[C] A concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.



\section{The flip: going for explicit construction}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of a (nonuniform)
obstruction (cf. Definition~\ref{dobst})
that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}.
Formally:

\begin{defn} \label{defnobstexplicit}
We say that an obstruction family ${\cal O}$ (Definition~\ref{dobst}) 
is {\em explicit} if:
\begin{enumerate}
\item {\bf Shortness:}
For any $n$ and $m< 2^n$, if there exists  an 
obstruction in ${\cal O}_{n,m}$ 
to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction $O_{n,m}$ in ${\cal O}_{n,m}$, 
where by short we mean 
the bitlength $\bitlength{O_{n,m}}$ of its specification is
$\poly(n)$ (note the bound does not depend on $m$).
\item {\bf Easy-to-verify:} Given $n,m$ and a bit string $x$, whether 
it is the specification $[O_{n,m}]$ of an obstruction  
$O_{n,m} \in {\cal O}_{n,m}$ can be decided  in $\poly(n,\bitlength{x})$
time, where $\bitlength{x}$ denotes the bitlength of $x$.
\end{enumerate}
\end{defn} 

This means that the problem of verifying (recognizing)
an obstruction (or rather its specification) belongs to $P$, and hence,
is theoretically feasible (``easy''). Thus this notion 
of an obstruction is then fundamentally better than the theoretically
infeasible trivial obstruction as far as verification is concerned.





Now, to prove $P \not = NP$ it  suffices  to show that 
${\cal O}_{n,m}$ is nonempty if $m=\poly(n)$, $n \rightarrow \infty$.
In this step, the approach should also justify on the basis of
mathematical evidence why this should be
so assuming  $P \not = NP$ (nonuniform).
This circular reasoning at this stage is only meant to convince us 
before we  plunge ahead that such obstructions should exist, i.e., there 
is no loss of essential information,  
assuming $P \not = NP$, which we take on faith, and the goal
now is to prove the existence of these obstructions.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of 
the new  explicit 
obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time, but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction using
the associated decoding procedure to get an exponential
size trivial obstruction.
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way. That is,
the computational complexity of the associated decoding algorithm 
(which we are only assuming is decidable) could be extremely high. 
And for that matter, we do not even need such a decoding algorithm 
as long as there is a guarantee that existence of an obstruction implies
existence of a trivial obstruction.
But if it is possible to get a trivial obstruction from a new obstruction
easily; i.e., if the asociated {\em decoding algorithm} works in polynomial
time, by  which we mean 
given specification of 
a new obstruction $O_{n,m}$ and a small $C$ of size $m$ it
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Note that if $O_{n,m}$ is short, i.e., $\bitlength{O_{n,m}}=\poly(n)$,
then this running time is $\poly(n,m)$.
Though we do not need the decoding algorithm to work in
polynomial time, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


It may be noticed that a final proof of the $P \not = NP$ conjecture 
is  an explicit obstruction for every $n$ and $m=\poly(n)$ 
as per Definition~\ref{defnobstexplicit} since it can be verified 
in $O(1)$ time. That is how it ought be since a final proof is 
the most explicit obstruction to the equality  of $NP$ with $P$ that one
can imagine. Similarly, an $O(1)$-size  program  for a one 
way function is an explicit obstruction for every $n$ and $m=\poly(n)$ 
after there is a final proof 
that it is indeed a one way function, i.e., when it is accompanied by
such a final proof  (without  it it is not even an 
obstruction, as already pointed out). 
But we are assuming here that the approach has not been
so lucky as to come with a final proof right in the first step. That is, 
the new obstruction in this first step is not a 
final proof or  accompanied by a final proof
but only a vehicle towards the final proof
as in the proofs of the earlier nonuniform lower bounds. 





\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing the specification of
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Formally, 

\begin{defn} 
We say that an explicit family of obstructions
(Definition~\ref{defnobstexplicit})
is {\em strongly explicit} if 
there is a discovery algorithm that given any $n$ and $m < 2^n$ 
decides in $\poly(n)$ time if ${\cal O}_{n,m}$ is nonempty
and, if so, produces in this much time specification $[O_{n,m}]$ of
an obstruction $O_{n,m} \in {\cal O}_{n,m}$.

We say that a strongly explicit family is {\em extremely explicit} 
if the obstructions are easy to decode; i.e., 
given the specifcation of a new obstruction $O_{n,m} \in {\cal O}_{n,m}$
and a small $C$ of size $m$ the associated decoding algorithm 
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$. 
\end{defn}

Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_{n,m} \in {\cal O}_{n,m}$. 

%We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs the specification of 
an obstruction $O_{n,m}$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
%If it is correct, we 
%call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture an {\em explicit proof},
based on the given notion of obstructions, if 
it is based on the flip and carries out the step I, a {\em strongly explicit
proof} if it carries out both steps I and II, and an 
{\em extremely explicit proof} if
in addition, the obstructions are easy to decode.




We  say that OH becomes {\em theoretically feasible}
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then become theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH, and 
however hard the task of proving OH may be mathematically,
the $P\not = NP$ conjecture  can be expected not to stand in the way
of its proof.
Hence, the name of this strategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both the barriers are 
crossed. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach   basically
means that the $P\not = NP$ conjecture should 
no longer stand in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.


Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{eqiohp}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_3$. We refer to this as the decision
problem associated with IOH and denote it by $DP(IOH)$.
When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
Let $DP(OH)$ be  the decision problem 
associated with OH, by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ and $m$ specified in unary. 
It belongs  to $NP$
after execution of the step I and to $P$ after the step II.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that  $DP(IOH) \in \Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH logically (both becoming tautologies),
and yet the decision problem for the 
new OH for general $m$ 
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH is also a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, such reduction
of a universal statement in $\Pi_3$ to another in $NP$ and then
to $P$ may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{},  it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.





For mathematical problems which are not universal, theoretical feasibility
can be meaningless. For example, consider 
a trivial  assertion $\forall A, B: A + B = B + A$ where $A$ and $B$ 
are $n\times n$ matrices.
The problem of brute force verification of this assertion 
belongs to $\Pi_1$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality and because 
those alternating quantifiers are intimately related to the 
the alternating quantifiers used to define the conjecturally 
noncollapsible  polynomial time hierarchy.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 


The  flip can also be formulated
in the theory of pseudorandom generators. For that we  fix 
an explicit $NP$-computable pseudorandom generator 
$g$ that conjecturally fools 
small  circuits (assuming which  $P \not = NP$). We  then express 
this property as an IOH for $g$ and associate a decision problem with it.
But it will be seen that this decision problem lies even higher in
the complexity hierarachy than the IOH for the $P$ vs. $NP$ problem; 
specifically it lies  in $\Pi_3^{BPP}$. Hence
the corresponding flip, which begins at this IOH  and runs towards FOH for $g$ 
through the complexity hierarchy, is harder.
In other words,  this says  that the theory
of pseudorandom generation (derandomization)
is in general  harder than the theory of lower bounds, and hence,
hardness should be proved first  and then transformed into
pseudorandom generation  as per the hardness vs. randomness 
principle \cite{}. This is why we focus on lower bounds in GCT at present.





The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
\ignore{It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.}
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. The same  for a local strongly explicit obstruction.
In this sense, the global flip is stronger than the local flip.
The global   flip also implies   the local  flip if there is a polynomial 
time decoding algorithm, since then 
from a  global  obstruction one can get 
a local  strongly  explicit  obstruction easily. 
The $P\not = NP$ conjecture does not stand in the way of this decoding.
Hence intuitively the global (strong) flip subsumes the local (strong) flip.
A local strong flip is used in the proof of the $P\not = NC$ result 
without bit operations described below. But for harder separation problems
it does not seem good enough to cross the feasibility barrier. 
We do not really understand why.






The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.



So far we have been assumming that the underlying field of 
computation is the boolean field. But the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems can also be defined over an arbitrary ring or
field, and we are  specifically  interested in 
the rings and fields of characteristic zero such as $Z$, $\Q$ and $\C$. 
Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
By the nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
we mean  the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
But we shall not worry about it here because all the basic ideas of GCT
are  illustrated in the $\#P$ vs. $NC$ problem in characteristic zero.
We  focuss  on characteristic zero  in this article  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

The flip can also be defined for the $P$ vs. $NP$ and $\#P$ vs. $NC$ 
problems over fields of characteristic zero such as $Q$ or $\C$ and for
algebraically closed fields of positive characteristic such as $\bar F_p$, 
the algebraic closure of the finite field $F_p$, $p$ prime.
All  definitions in the flip 
can be lifted to this setting in the obvious way. We  only give
one critical definition as an illustration assuming that the underlying 
field is $Q$. In this case we say that an
obstruction family is {\em easy to decode} 
if there is a decoding algorithm which given the specification of 
an obstruction $O=O_{n,m}$ and a small circuit $C$ over $\Q$ of size $m$ 
(i.e. whose whole description is of bitlength $m$)
produces in $\poly(n,m, \bitlength{O})$ time a counter example (local
obstruction) $X$ for 
$C$ whose description has  $\poly(n,\bitlength{O})$ bitlength, 
independent of $m$ as long as it is $\le n^{\log n}$ (say). If 
$\bitlength{O}$ is $\poly(n)$ the bitlength of $X$ is then $\poly(n)$
independent of $m$. In other words, smallness
of  obstructions is to be preserved in the process of decoding.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts are fine and also inevitable as long as 
the spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip also has the following disturbing   feature.
Namely,  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, as per the flip,  modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same.
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.

After all the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific  functions (generalized permanents) 
and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in this   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative.
After all, as pointed out in Section~\ref{sfeasibility}, 
any approach to the $P$ vs. $NP$ problem has 
to meet at least the criteria A, B, and C stated there.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{}) addresses (A).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{})   addresses (B).
The main result [GCT6] of GCT  (cf. Section~\ref{})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero;
[GCT11] does  the same for   any
field including the finite field (the usual case). This
addresses (C). 


But, at present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction.


We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.

\section{A: The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems. Hence, this lower bound meets 
the criterion B.
The proof technique of this result is  locally strongly
explicit, i.e.,  the   local strong form
of the flip (but a bit relaxed),  
in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$, or even 
$2^{\log^a N}$, for some positive constant $a$,
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.

Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit
(or in a relaxed sense, 
say $\log \log n$ depth circuit of $2^{\polylog(n)}$ size). 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally strongly) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas, 
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 


\noindent {\em Remark:} Assuming  a stronger lower bound result \cite{}  for 
constant depth circuits, it is easy to show that a counter example 
against a constant depth circuit can be found in $\polylog(N)$ time using
$2^{\polylog(N)}$ processors. And similarly assumming a stronger form
of the $P\not = NC$ result without bit operations, it is easy to show
that a counter example against a branching  circuit of $\polylog(N)$ depth
and $2^{\polylog(N)}$ size can be found by a branching circuit of
 $\polylog(N)$ depth and $2^{\polylog(N)}$ size. But what matters here is not 
how quickly obstructions can be constructed 
once  the lower bound result is proved, but rather how quickly the obstructions
that can be  used to prove the result can be constructed.


In view of the natural proof barrier, it should not be surprising 
that the proof of the  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).

Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar.%, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seem effective  for the harder separation problems.
So began a search for  a proof technique that can overcome the algebraic 
degree barrier and the locality limitation of local GCT. 


\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


\ignore{
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.}






\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS,
and to Janos Simon, Josh Grochow, and Hari Narayanan for 
the help in presentation. 









==> text1.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
The main barrier 
towards these problems is   the {\em   feasibility
barrier} described here (Section~\ref{})   and  the basic strategy
of GCT for crossing this barrier is called the flip [GCT6,GCTflip].
The main result of  GCT [GCT6,7,8,GCT11] is conjectural scheme for
the implementation of the flip.
Its  final goal
is to prove the {\em explicit proof conjecture} (Section~\ref{}),
which says that
the $P\not = NP$ conjecture has an {\em extremely explicit proof}, by 
which we mean a proof  
that shows existence of  proof certificates
of hardness for the $NP$-complete function under consideration 
that are short (of polynomial size), easy to verify, discover and decode 
(in polynomial time); cf. Section~\ref{}.
This  is supported by 
two concrete lower bounds of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] (Section~\ref{})
and a mathematical  form of the $\#P\not = NC$ conjecture in characteristic
zero (Section~\ref{}).
This introduction gives a short overview  of GCT outlining these developments.


The original lectures did not describe the 
the  feasiblity   barrier  and the explicit proof conjecture.
But all the mathematical effort in   GCT as described in these lectures 
goes towards crossing this barrier and  producing such an explicit proof.
Hence, we describe  them   here so that the root cause of 
all difficulties encountered in GCT and the need for nonelementary techniques
to cross this formidable barrier
becomes clear  at a high level before we get into any mathematics. 


The original IAS lectures did not state the first lower bound and
only stated   a special case of the second 
lower bound called  the weak form of the $\#P$ vs.
$NC$ problem. The article \cite{boris} showed that this weak form 
is too weak; i.e., it can be proved    by an elementary  technique
that  cannot cross the natural-proof barrier \cite{rudich}.
We cannot prove the full mathematical form by such
techniques for the reasons given in Sections~\ref{}.
Its  proof here 
is based on the results of GCT1,2 and geometric invariant theory 
\cite{mumford}. It crosses the relativization \cite{solovay}, 
natural proof \cite{rudich}, 
algebraic degree \cite{GCTlocal}, and algebrization \cite{aaronson} 
barriers simultaneously  and is (strongly) explicit. 
These two lower bound results  provide a concrete support  for 
the GCT approach.









\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 




\section{The  feasibility barrier} \label{sfeasibility}
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggest such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,razborov,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
of every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $\C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
deconding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or far that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results 
\cite{sipser,razborov,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonunifrom obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments, like the ones  based on uniform 
objects which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier 
relativization \cite{solovay}, natural-(probabilistic)-proof {rudich}, 
algebraic degree [GCTlocal], and 
algebrization \cite{aaronson} barriers simultaneously.
Here, in view of the fundamental nature of these barriers, we agree to
take them in spirit rather than letter. Because, though these barriers 
are defined only for the unrestricted $P$ vs. $NP$ problem, they make 
sense in  any reasonable restricted setting. Thus we assume that
the relativization barrier   applies to any technique that views 
computation abstractly without algebrizing it, algebraic degree or
algebrization barrier to any low degree technique,
and the natural proof barrier to any technique that works 
for most functions with the meaning of most as in \cite{rudich}. 
\item[C] A concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.



\section{The flip: going for explicit construction}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of a (nonuniform)
obstruction (cf. Definition~\ref{dobst})
that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}.
Formally:

\begin{defn} \label{defnobstexplicit}
We say that an obstruction family ${\cal O}$ (Definition~\ref{dobst}) 
is {\em explicit} if:
\begin{enumerate}
\item {\bf Shortness:}
For any $n$ and $m< 2^n$, if there exists  an 
obstruction in ${\cal O}_{n,m}$ 
to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction $O_{n,m}$ in ${\cal O}_{n,m}$, 
where by short we mean 
the bitlength $\bitlength{O_{n,m}}$ of its specification is
$\poly(n)$ (note the bound does not depend on $m$).
\item {\bf Easy-to-verify:} Given $n,m$ and a bit string $x$, whether 
it is the specification $[O_{n,m}]$ of an obstruction  
$O_{n,m} \in {\cal O}_{n,m}$ can be decided  in $\poly(n,\bitlength{x})$
time, where $\bitlength{x}$ denotes the bitlength of $x$.
\end{enumerate}
\end{defn} 

This means that the problem of verifying (recognizing)
an obstruction (or rather its specification) belongs to $P$, and hence,
is theoretically feasible (``easy''). Thus this notion 
of an obstruction is then fundamentally better than the theoretically
infeasible trivial obstruction as far as verification is concerned.





Now, to prove $P \not = NP$ it  suffices  to show that 
${\cal O}_{n,m}$ is nonempty if $m=\poly(n)$, $n \rightarrow \infty$.
In this step, the approach should also justify on the basis of
mathematical evidence why this should be
so assuming  $P \not = NP$ (nonuniform).
This circular reasoning at this stage is only meant to convince us 
before we  plunge ahead that such obstructions should exist, i.e., there 
is no loss of essential information,  
assuming $P \not = NP$, which we take on faith, and the goal
now is to prove the existence of these obstructions.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of 
the new  explicit 
obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time, but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction using
the associated decoding procedure to get an exponential
size trivial obstruction.
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way. That is,
the computational complexity of the associated decoding algorithm 
(which we are only assuming is decidable) could be extremely high. 
And for that matter, we do not even need such a decoding algorithm 
as long as there is a guarantee that existence of an obstruction implies
existence of a trivial obstruction.
But if it is possible to get a trivial obstruction from a new obstruction
easily; i.e., if the asociated {\em decoding algorithm} works in polynomial
time, by  which we mean 
given specification of 
a new obstruction $O_{n,m}$ and a small $C$ of size $m$ it
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Note that if $O_{n,m}$ is short, i.e., $\bitlength{O_{n,m}}=\poly(n)$,
then this running time is $\poly(n,m)$.
Though we do not need the decoding algorithm to work in
polynomial time, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


It may be noticed that a final proof of the $P \not = NP$ conjecture 
is  an explicit obstruction for every $n$ and $m=\poly(n)$ 
as per Definition~\ref{defnobstexplicit} since it can be verified 
in $O(1)$ time. That is how it ought be since a final proof is 
the most explicit obstruction to the equality  of $NP$ with $P$ that one
can imagine. Similarly, an $O(1)$-size  program  for a one 
way function is an explicit obstruction for every $n$ and $m=\poly(n)$ 
after there is a final proof 
that it is indeed a one way function, i.e., when it is accompanied by
such a final proof  (without  it it is not even an 
obstruction, as already pointed out). 
But we are assuming here that the approach has not been
so lucky as to come with a final proof right in the first step. That is, 
the new obstruction in this first step is not a 
final proof or  accompanied by a final proof
but only a vehicle towards the final proof
as in the proofs of the earlier nonuniform lower bounds. 





\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing the specification of
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Formally, 

\begin{defn} 
We say that an explicit family of obstructions
(Definition~\ref{defnobstexplicit})
is {\em strongly explicit} if 
there is a discovery algorithm that given any $n$ and $m < 2^n$ 
decides in $\poly(n)$ time if ${\cal O}_{n,m}$ is nonempty
and, if so, produces in this much time specification $[O_{n,m}]$ of
an obstruction $O_{n,m} \in {\cal O}_{n,m}$.

We say that a strongly explicit family is {\em extremely explicit} 
if the obstructions are easy to decode; i.e., 
given the specifcation of a new obstruction $O_{n,m} \in {\cal O}_{n,m}$
and a small $C$ of size $m$ the associated decoding algorithm 
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$. 
\end{defn}

Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_{n,m} \in {\cal O}_{n,m}$. 

%We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs the specification of 
an obstruction $O_{n,m}$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
%If it is correct, we 
%call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture an {\em explicit proof},
based on the given notion of obstructions, if 
it is based on the flip and carries out the step I, a {\em strongly explicit
proof} if it carries out both steps I and II, and an 
{\em extremely explicit proof} if
in addition, the obstructions are easy to decode.




We  say that OH becomes {\em theoretically feasible}
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then become theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH, and 
however hard the task of proving OH may be mathematically,
the $P\not = NP$ conjecture  can be expected not to stand in the way
of its proof.
Hence, the name of this strategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both the barriers are 
crossed. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach   basically
means that the $P\not = NP$ conjecture should 
no longer stand in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.


Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{eqiohp}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_3$. We refer to this as the decision
problem associated with IOH and denote it by $DP(IOH)$.
When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
Let $DP(OH)$ be  the decision problem 
associated with OH, by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ and $m$ specified in unary. 
It belongs  to $NP$
after execution of the step I and to $P$ after the step II.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that  $DP(IOH) \in \Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH logically (both becoming tautologies),
and yet the decision problem for the 
new OH for general $m$ 
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH is also a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, such reduction
of a universal statement in $\Pi_3$ to another in $NP$ and then
to $P$ may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{},  it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.





For mathematical problems which are not universal, theoretical feasibility
can be meaningless. For example, consider 
a trivial  assertion $\forall A, B: A + B = B + A$ where $A$ and $B$ 
are $n\times n$ matrices.
The problem of brute force verification of this assertion 
belongs to $\Pi_1$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality and because 
those alternating quantifiers are intimately related to the 
the alternating quantifiers used to define the conjecturally 
noncollapsible  polynomial time hierarchy.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 


The  flip can also be formulated
in the theory of pseudorandom generators. For that we  fix 
an explicit $NP$-computable pseudorandom generator 
$g$ that conjecturally fools 
small  circuits (assuming which  $P \not = NP$). We  then express 
this property as an IOH for $g$ and associate a decision problem with it.
But it will be seen that this decision problem lies even higher in
the complexity hierarachy than the IOH for the $P$ vs. $NP$ problem; 
specifically it lies  in $\Pi_3^{BPP}$. Hence
the corresponding flip, which begins at this IOH  and runs towards FOH for $g$ 
through the complexity hierarchy, is harder.
In other words,  this says  that the theory
of pseudorandom generation (derandomization)
is in general  harder than the theory of lower bounds, and hence,
hardness should be proved first  and then transformed into
pseudorandom generation  as per the hardness vs. randomness 
principle \cite{}. This is why we focus on lower bounds in GCT at present.





The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
\ignore{It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.}
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. The same  for a local strongly explicit obstruction.
In this sense, the global flip is stronger than the local flip.
The global   flip also implies   the local  flip if there is a polynomial 
time decoding algorithm, since then 
from a  global  obstruction one can get 
a local  strongly  explicit  obstruction easily. 
The $P\not = NP$ conjecture does not stand in the way of this decoding.
Hence intuitively the global (strong) flip subsumes the local (strong) flip.
A local strong flip is used in the proof of the $P\not = NC$ result 
without bit operations described below. But for harder separation problems
it does not seem good enough to cross the feasibility barrier. 
We do not really understand why.






The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.



So far we have been assumming that the underlying field of 
computation is the boolean field. But the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems can also be defined over an arbitrary ring or
field, and we are  specifically  interested in 
the rings and fields of characteristic zero such as $Z$, $\Q$ and $\C$. 
Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
By the nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
we mean  the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
But we shall not worry about it here because all the basic ideas of GCT
are  illustrated in the $\#P$ vs. $NC$ problem in characteristic zero.
We  focuss  on characteristic zero  in this article  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

The flip can also be defined for the $P$ vs. $NP$ and $\#P$ vs. $NC$ 
problems over fields of characteristic zero such as $Q$ or $\C$ and for
algebraically closed fields of positive characteristic such as $\bar F_p$, 
the algebraic closure of the finite field $F_p$, $p$ prime.
All  definitions in the flip 
can be lifted to this setting in the obvious way. We  only give
one critical definition as an illustration assuming that the underlying 
field is $Q$. In this case we say that an
obstruction family is {\em easy to decode} 
if there is a decoding algorithm which given the specification of 
an obstruction $O=O_{n,m}$ and a small circuit $C$ over $\Q$ of size $m$ 
(i.e. whose whole description is of bitlength $m$)
produces in $\poly(n,m, \bitlength{O})$ time a counter example (local
obstruction) $X$ for 
$C$ whose description has  $\poly(n,\bitlength{O})$ bitlength, 
independent of $m$ as long as it is $\le n^{\log n}$ (say). If 
$\bitlength{O}$ is $\poly(n)$ the bitlength of $X$ is then $\poly(n)$
independent of $m$. In other words, smallness
of  obstructions is to be preserved in the process of decoding.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts are fine and also inevitable as long as 
the spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip also has the following disturbing   feature.
Namely,  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, as per the flip,  modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same.
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.

After all the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific  functions (generalized permanents) 
and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in this   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative.
After all, as pointed out in Section~\ref{sfeasibility}, 
any approach to the $P$ vs. $NP$ problem has 
to meet at least the criteria A, B, and C stated there.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{}) addresses (A).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{})   addresses (B).
The main result [GCT6] of GCT  (cf. Section~\ref{})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero;
[GCT11] does  the same for   any
field including the finite field (the usual case). This
addresses (C). 


But, at present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction.


We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.

\section{A: The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems. Hence, this lower bound meets 
the criterion B.
The proof technique of this result is  locally strongly
explicit, i.e.,  the   local strong form
of the flip (but a bit relaxed),  
in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$, or even 
$2^{\log^a N}$, for some positive constant $a$,
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.

Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit
(or in a relaxed sense, 
say $\log \log n$ depth circuit of $2^{\polylog(n)}$ size). 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally strongly) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas, 
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 


\noindent {\em Remark:} Assuming  a stronger lower bound result \cite{}  for 
constant depth circuits, it is easy to show that a counter example 
against a constant depth circuit can be found in $\polylog(N)$ time using
$2^{\polylog(N)}$ processors. And similarly assumming a stronger form
of the $P\not = NC$ result without bit operations, it is easy to show
that a counter example against a branching  circuit of $\polylog(N)$ depth
and $2^{\polylog(N)}$ size can be found by a branching circuit of
 $\polylog(N)$ depth and $2^{\polylog(N)}$ size. But what matters here is not 
how quickly obstructions can be constructed 
once  the lower bound result is proved, but rather how quickly the obstructions
that can be  used to prove the result can be constructed.


In view of the natural proof barrier, it should not be surprising 
that the proof of the  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).

Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar.%, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seems good enough for the harder separation problems.
So began a search for  a proof technique that can overcome the algebraic 
degree barrier and the locality limitation of local GCT. 


\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


\ignore{
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.}






\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS,
and to Janos Simon, Josh Grochow, and Hari Narayanan for 
the help in presentation. 








